The Second Challenge on Cross-Domain Few-Shot Object Detection at NTIRE 2026: Methods and Results

Cross-domain few-shot object detection (CD-FSOD) remains a challenging problem for existing object detectors and few-shot learning approaches, particularly when generalizing across distinct domains. As part of NTIRE 2026, we hosted the second CD-FSOD Challenge to systematically evaluate and promote progress in detecting objects in unseen target domains under limited annotation conditions. The challenge received strong community interest, with 128 registered participants and a total of 696 submissions. Among them, 31 teams actively participated, and 19 teams submitted valid final results. Participants explored a wide range of strategies, introducing innovative methods that push the performance frontier under both open-source and closed-source tracks. This report presents a detailed overview of the NTIRE 2026 CD-FSOD Challenge, including a summary of the submitted approaches and an analysis of the final results across all participating teams. Challenge Codes: https://github.com/ohMargin/NTIRE2026_CDFSOD.

==> affiliation.tex <==
\subsection*{NTIRE 2026 team}
\noindent\textit{\textbf{Title: }} NTIRE 2026 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.\\
\noindent\textit{\textbf{Members: }} \\
Xingyu Qiu$^{1}$ (\href{mailto:xyqiu24@m.fudan.edu.cn}{xyqiu24@m.fudan.edu.cn}),\\
Yuqian Fu$^{2}$ (\href{mailto:yuqian.fu.ai@gmail.com}{yuqian.fu.ai@gmail.com}),\\
Jiawei Geng$^{1}$ (\href{mailto:jwgeng25@m.fudan.edu.cn}{jwgeng25@m.fudan.edu.cn}),\\
Bin Ren$^{3}$ (\href{mailto:bin.ren.mondo@gmail.com}{bin.ren.mondo@gmail.com}),\\
Jiancheng Pan$^{4}$ (\href{mailto:jiancheng.pan.plus@gmail.com}{jiancheng.pan.plus@gmail.com}),\\
Zongwei Wu$^{5}$ (\href{mailto:zongwei.wu@uni-wuerzburg.de}{zongwei.wu@uni-wuerzburg.de}),\\
Hao Tang$^{6}$ (\href{mailto:howard.haotang@gmail.com}{howard.haotang@gmail.com}),\\
Yanwei Fu$^{1}$ (\href{mailto:yanweifu@fudan.edu.cn}{yanweifu@fudan.edu.cn}),\\
Radu Timofte$^{5}$ (\href{mailto:radu.timofte@uni-wuerzburg.de}{radu.timofte@uni-wuerzburg.de}),\\
Nicu Sebe$^{7}$ (\href{mailto:niculae.sebe@unitn.it}{niculae.sebe@unitn.it}),\\
Mohamed Elhoseiny$^{2}$
(\href{mailto:mohamed.elhoseiny@kaust.edu.sa}{mohamed.elhoseiny@kaust.edu.sa})

\noindent\textit{\textbf{Affiliations: }}\\
$^1$ Fudan University, China\\
$^2$ KAUST, Saudi Arabia\\
$^3$ MBZUAI, United Arab Emirates\\
$^4$ Tsinghua University, China\\
$^5$ University of W\"urzburg, Germany\\
$^6$ The Hong Kong Polytechnic University, China\\
$^7$ University of Trento, Italy\\

==> main <==
\begin{thebibliography}{133}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Ancuti et~al.(2026{\natexlab{a}})Ancuti, Ancuti, Timofte, and Ancuti]{ntire26nthaze}
Radu Ancuti, Codruta Ancuti, Radu Timofte, and Cosmin Ancuti.
\newblock { NT-HAZE: A Benchmark Dataset for Realistic Night-time Image Dehazing }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Ancuti et~al.(2026{\natexlab{b}})Ancuti, Brateanu, Vasluianu, Balmez, Orhei, Ancuti, Timofte, Ancuti, et~al.]{ntire26nthaze_rep}
Radu Ancuti, Alexandru Brateanu, Florin Vasluianu, Raul Balmez, Ciprian Orhei, Codruta Ancuti, Radu Timofte, Cosmin Ancuti, et~al.
\newblock { NTIRE 2026 Nighttime Image Dehazing Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Bai et~al.(2025{\natexlab{a}})Bai, Cai, Chen, Chen, Chen, Cheng, Deng, Ding, Gao, Ge, Ge, Guo, Huang, Huang, Huang, Hui, Jiang, Li, Li, Li, Li, Lin, Lin, Liu, Liu, Liu, Liu, Liu, Liu, Lu, Luo, Lv, Men, Meng, Ren, Ren, Song, Sun, Tang, Tu, Wan, Wang, Wang, Wang, Wang, Xie, Xu, Xu, Xu, Yang, Yang, Yang, Yang, Yu, Zhang, Zhang, Zhang, Zheng, Zhong, Zhou, Zhou, Zhou, Zhu, and Zhu]{qwen3vl}
Shuai Bai, Yuxuan Cai, Ruizhe Chen, Keqin Chen, Xionghui Chen, Zesen Cheng, Lianghao Deng, Wei Ding, Chang Gao, Chunjiang Ge, Wenbin Ge, Zhifang Guo, Qidong Huang, Jie Huang, Fei Huang, Binyuan Hui, Shutong Jiang, Zhaohai Li, Mingsheng Li, Mei Li, Kaixin Li, Zicheng Lin, Junyang Lin, Xuejing Liu, Jiawei Liu, Chenglong Liu, Yang Liu, Dayiheng Liu, Shixuan Liu, Dunjie Lu, Ruilin Luo, Chenxu Lv, Rui Men, Lingchen Meng, Xuancheng Ren, Xingzhang Ren, Sibo Song, Yuchong Sun, Jun Tang, Jianhong Tu, Jianqiang Wan, Peng Wang, Pengfei Wang, Qiuyue Wang, Yuxuan Wang, Tianbao Xie, Yiheng Xu, Haiyang Xu, Jin Xu, Zhibo Yang, Mingkun Yang, Jianxin Yang, An Yang, Bowen Yu, Fei Zhang, Hang Zhang, Xi Zhang, Bo Zheng, Humen Zhong, Jingren Zhou, Fan Zhou, Jing Zhou, Yuanzhi Zhu, and Ke Zhu.
\newblock Qwen3-vl technical report.
\newblock \emph{arXiv preprint arXiv:2511.21631}, 2025{\natexlab{a}}.

\bibitem[Bai et~al.(2025{\natexlab{b}})Bai, Cai, Chen, Chen, Chen, Cheng, Deng, Ding, Gao, Ge, et~al.]{bai2025qwen3}
Shuai Bai, Yuxuan Cai, Ruizhe Chen, Keqin Chen, Xionghui Chen, Zesen Cheng, Lianghao Deng, Wei Ding, Chang Gao, Chunjiang Ge, et~al.
\newblock Qwen3-vl technical report.
\newblock \emph{arXiv preprint arXiv:2511.21631}, 2025{\natexlab{b}}.

\bibitem[Bochkovskiy et~al.(2020)Bochkovskiy, Wang, and Liao]{bochkovskiy2020yolov4}
Alexey Bochkovskiy, Chien-Yao Wang, and Hong-Yuan~Mark Liao.
\newblock Yolov4: Optimal speed and accuracy of object detection.
\newblock \emph{arXiv preprint arXiv:2004.10934}, 2020.

\bibitem[Cai et~al.(2026)Cai, Yang, Li, Vasluianu, Timofte, et~al.]{ntire26reflection}
Jie Cai, Kangning Yang, Zhiyuan Li, Florin Vasluianu, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Single Image Reflection Removal in the Wild: Datasets, Results, and Methods }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Carion et~al.(2020)Carion, Massa, Synnaeve, Usunier, Kirillov, and Zagoruyko]{carion2020end}
Nicolas Carion, Francisco Massa, Gabriel Synnaeve, Nicolas Usunier, Alexander Kirillov, and Sergey Zagoruyko.
\newblock End-to-end object detection with transformers.
\newblock In \emph{ECCV}, 2020.

\bibitem[Carion et~al.(2025{\natexlab{a}})Carion, Gustafson, Hu, Debnath, Hu, Suris, Ryali, Alwala, Khedr, Huang, Lei, Ma, Guo, Kalla, Marks, Greer, Wang, Sun, Rädle, Afouras, Mavroudi, Xu, Wu, Zhou, Momeni, Hazra, Ding, Vaze, Porcher, Li, Li, Kamath, Cheng, Dollár, Ravi, Saenko, Zhang, and Feichtenhofer]{sam3}
Nicolas Carion, Laura Gustafson, Yuan-Ting Hu, Shoubhik Debnath, Ronghang Hu, Didac Suris, Chaitanya Ryali, Kalyan~Vasudev Alwala, Haitham Khedr, Andrew Huang, Jie Lei, Tengyu Ma, Baishan Guo, Arpit Kalla, Markus Marks, Joseph Greer, Meng Wang, Peize Sun, Roman Rädle, Triantafyllos Afouras, Effrosyni Mavroudi, Katherine Xu, Tsung-Han Wu, Yu Zhou, Liliane Momeni, Rishi Hazra, Shuangrui Ding, Sagar Vaze, Francois Porcher, Feng Li, Siyuan Li, Aishwarya Kamath, Ho~Kei Cheng, Piotr Dollár, Nikhila Ravi, Kate Saenko, Pengchuan Zhang, and Christoph Feichtenhofer.
\newblock Sam 3: Segment anything with concepts, 2025{\natexlab{a}}.

\bibitem[Carion et~al.(2025{\natexlab{b}})Carion, Gustafson, Hu, Debnath, Hu, Suris, Ryali, Alwala, Khedr, Huang, et~al.]{carion2025sam}
Nicolas Carion, Laura Gustafson, Yuan-Ting Hu, Shoubhik Debnath, Ronghang Hu, Didac Suris, Chaitanya Ryali, Kalyan~Vasudev Alwala, Haitham Khedr, Andrew Huang, et~al.
\newblock Sam 3: Segment anything with concepts.
\newblock \emph{arXiv preprint arXiv:2511.16719}, 2025{\natexlab{b}}.

\bibitem[Carion et~al.(2026)Carion, Gustafson, Hu, Debnath, Hu, Coll-Vinent, Ryali, Alwala, Khedr, Huang, Lei, Ma, Guo, Kalla, Marks, Greer, Wang, Sun, R{\"a}dle, Afouras, Mavroudi, Xu, Wu, Zhou, Momeni, HAZRA, Ding, Vaze, Porcher, Li, Li, Kamath, Cheng, Dollar, Ravi, Saenko, Zhang, and Feichtenhofer]{carion2026sam}
Nicolas Carion, Laura Gustafson, Yuan-Ting Hu, Shoubhik Debnath, Ronghang Hu, Didac~Suris Coll-Vinent, Chaitanya Ryali, Kalyan~Vasudev Alwala, Haitham Khedr, Andrew Huang, Jie Lei, Tengyu Ma, Baishan Guo, Arpit Kalla, Markus Marks, Joseph Greer, Meng Wang, Peize Sun, Roman R{\"a}dle, Triantafyllos Afouras, Effrosyni Mavroudi, Katherine Xu, Tsung-Han Wu, Yu Zhou, Liliane Momeni, RISHI HAZRA, Shuangrui Ding, Sagar Vaze, Francois Porcher, Feng Li, Siyuan Li, Aishwarya Kamath, Ho~Kei Cheng, Piotr Dollar, Nikhila Ravi, Kate Saenko, Pengchuan Zhang, and Christoph Feichtenhofer.
\newblock {SAM} 3: Segment anything with concepts.
\newblock In \emph{The Fourteenth International Conference on Learning Representations}, 2026.

\bibitem[Chen et~al.(2019)Chen, Wang, Pang, Cao, Xiong, Li, Sun, Feng, Liu, Xu, Zhang, Cheng, Zhu, Cheng, Zhao, Li, Lu, Zhu, Wu, Dai, Wang, Shi, Ouyang, Loy, and Lin]{mmdetection}
Kai Chen, Jiaqi Wang, Jiangmiao Pang, Yuhang Cao, Yu Xiong, Xiaoxiao Li, Shuyang Sun, Wansen Feng, Ziwei Liu, Jiarui Xu, Zheng Zhang, Dazhi Cheng, Chenchen Zhu, Tianheng Cheng, Qijie Zhao, Buyu Li, Xin Lu, Rui Zhu, Yue Wu, Jifeng Dai, Jingdong Wang, Jianping Shi, Wanli Ouyang, Chen~Change Loy, and Dahua Lin.
\newblock {MMDetection}: Open mmlab detection toolbox and benchmark.
\newblock \emph{arXiv preprint arXiv:1906.07155}, 2019.

\bibitem[Chen et~al.(2026)Chen, Liu, Wang, Yan, Li, Zhang, Gong, Li, Sun, Liu, Timofte, Zhang, et~al.]{ntire26srx4}
Zheng Chen, Kai Liu, Jingkai Wang, Xianglong Yan, Jianze Li, Ziqing Zhang, Jue Gong, Jiatong Li, Lei Sun, Xiaoyang Liu, Radu Timofte, Yulun Zhang, et~al.
\newblock { The Fourth Challenge on Image Super-Resolution (×4) at NTIRE 2026: Benchmark Results and Method Overview }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[{Chenping Fu, Risheng Liu, Xin Fan, Puyang Chen, Hao Fu, Wanqi Yuan, Ming Zhu, Zhongxuan Luo}()]{RUOD23}
{Chenping Fu, Risheng Liu, Xin Fan, Puyang Chen, Hao Fu, Wanqi Yuan, Ming Zhu, Zhongxuan Luo}.
\newblock {Rethinking general underwater object detection: Datasets, challenges, and solutions}.
\newblock \emph{{Neurocomputing}}.

\bibitem[Choi et~al.(2025)Choi, Go, and Jang]{spbaizero}
Sangbum Choi, Kyeongryeol Go, and Taewoong Jang.
\newblock Zero: Industry-ready vision foundation model with multi-modal prompts, 2025.

\bibitem[Ciubotariu et~al.(2026{\natexlab{a}})Ciubotariu, S~M~A, Rehman, Ali, Naqvi, Conde, Timofte, et~al.]{ntire26llie}
George Ciubotariu, Sharif S~M~A, Abdur Rehman, Fayaz Ali, Rizwan~Ali Naqvi, Marcos Conde, Radu Timofte, et~al.
\newblock { Low Light Image Enhancement Challenge at NTIRE 2026 }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Ciubotariu et~al.(2026{\natexlab{b}})Ciubotariu, Zhou, Jin, Wu, Timofte, et~al.]{ntire26highfps}
George Ciubotariu, Zhuyun Zhou, Yeying Jin, Zongwei Wu, Radu Timofte, et~al.
\newblock { High FPS Video Frame Interpolation Challenge at NTIRE 2026 }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Devlin et~al.(2019)Devlin, Chang, Lee, and Toutanova]{devlin2019bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language understanding.
\newblock In \emph{Proceedings of the 2019 conference of the North American chapter of the association for computational linguistics: human language technologies, volume 1 (long and short papers)}, 2019.

\bibitem[Drange(2019)]{GeirArTaxOr}
Geir Drange.
\newblock Arthropod taxonomy orders object detection dataset.
\newblock In \emph{https://doi.org/10.34740/kaggle/dsv/1240192}, 2019.

\bibitem[Dumitriu et~al.(2026)Dumitriu, Ralhan, Miron, Tatui, Ionescu, Timofte, et~al.]{ntire26ripdetseg}
Andrei Dumitriu, Aakash Ralhan, Florin Miron, Florin Tatui, Radu~Tudor Ionescu, Radu Timofte, et~al.
\newblock { NTIRE 2026 Rip Current Detection and Segmentation (RipDetSeg) Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Elezabi et~al.(2026)Elezabi, V.~Conde, Wu, Jin, Timofte, et~al.]{ntire26retouching}
Omar Elezabi, Marcos V.~Conde, Zongwei Wu, Yeying Jin, Radu Timofte, et~al.
\newblock { Photography Retouching Transfer, NTIRE 2026 Challenge: Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Feng et~al.(2026{\natexlab{a}})Feng, Sha, Liu, Yu, Vong, Yu, and Shen]{feng2025fsodvfm}
Chen-Bin Feng, Youyang Sha, Longfei Liu, Yongjun Yu, Chi~Man Vong, Xuanlong Yu, and Xi Shen.
\newblock Few-shot object detection with vision foundation models and graph diffusion.
\newblock In \emph{The Fourteenth International Conference on Learning Representations}, 2026{\natexlab{a}}.

\bibitem[Feng et~al.(2026{\natexlab{b}})Feng, Sha, Liu, Yu, Vong, Yu, and Shen]{feng2026fsodvfm}
Chen-Bin Feng, Youyang Sha, Longfei Liu, Yongjun Yu, Chi~Man Vong, Xuanlong Yu, and Xi Shen.
\newblock {FSOD-VFM}: Few-shot object detection with vision foundation models and graph diffusion.
\newblock In \emph{ICLR}, 2026{\natexlab{b}}.

\bibitem[Fu et~al.(2025{\natexlab{a}})Fu, Su, Rao, Lyu, Xie, and Zheng]{fu2025wedetect}
Shenghao Fu, Yukun Su, Fengyun Rao, Jing Lyu, Xiaohua Xie, and Wei-Shi Zheng.
\newblock Wedetect: Fast open-vocabulary object detection as retrieval.
\newblock \emph{arXiv preprint arXiv:2512.12309}, 2025{\natexlab{a}}.

\bibitem[Fu et~al.(2021)Fu, Fu, and Jiang]{fu2021meta}
Yuqian Fu, Yanwei Fu, and Yu-Gang Jiang.
\newblock Meta-fdmixup: Cross-domain few-shot learning guided by labeled target data.
\newblock In \emph{ACM multimedia}, 2021.

\bibitem[Fu et~al.(2022)Fu, Xie, Fu, Chen, and Jiang]{fu2022me}
Yuqian Fu, Yu Xie, Yanwei Fu, Jingjing Chen, and Yu-Gang Jiang.
\newblock Me-d2n: Multi-expert domain decompositional network for cross-domain few-shot learning.
\newblock In \emph{ACM multimedia}, 2022.

\bibitem[Fu et~al.(2023)Fu, Xie, Fu, and Jiang]{fu2023styleadv}
Yuqian Fu, Yu Xie, Yanwei Fu, and Yu-Gang Jiang.
\newblock Styleadv: Meta style adversarial training for cross-domain few-shot learning.
\newblock In \emph{CVPR}, 2023.

\bibitem[Fu et~al.(2024)Fu, Wang, Pan, Huai, Qiu, Shangguan, Liu, Fu, Van~Gool, and Jiang]{fu2024cross}
Yuqian Fu, Yu Wang, Yixuan Pan, Lian Huai, Xingyu Qiu, Zeyu Shangguan, Tong Liu, Yanwei Fu, Luc Van~Gool, and Xingqun Jiang.
\newblock Cross-domain few-shot object detection via enhanced open-set object detector.
\newblock In \emph{European Conference on Computer Vision}, 2024.

\bibitem[Fu et~al.(2025{\natexlab{b}})Fu, Qiu, Ren, Fu, Timofte, Sebe, Yang, Van~Gool, Zhang, Nong, et~al.]{fu2025ntire}
Yuqian Fu, Xingyu Qiu, Bin Ren, Yanwei Fu, Radu Timofte, Nicu Sebe, Ming-Hsuan Yang, Luc Van~Gool, Kaijin Zhang, Qingpeng Nong, et~al.
\newblock Ntire 2025 challenge on cross-domain few-shot object detection: Methods and results.
\newblock In \emph{Proceedings of the Computer Vision and Pattern Recognition Conference}, 2025{\natexlab{b}}.

\bibitem[Guan et~al.(2026{\natexlab{a}})Guan, Li, Yang, Ke, Cai, Vasluianu, Timofte, et~al.]{ntire26finrec}
Bochen Guan, Jinlong Li, Kangning Yang, Chuang Ke, Jie Cai, Florin Vasluianu, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on End-to-End Financial Receipt Restoration and Reasoning from Degraded Images: Datasets, Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Guan et~al.(2026{\natexlab{b}})Guan, Zhang, Guo, Wang, Fan, Liang, Zeng, Qin, Qu, Dai, Xia, Zhang, Timofte, et~al.]{ntire26raim_portrait}
Ya-nan Guan, Shaonan Zhang, Hang Guo, Yawen Wang, Xinying Fan, Jie Liang, Hui Zeng, Guanyi Qin, Lishen Qu, Tao Dai, Shu-Tao Xia, Lei Zhang, Radu Timofte, et~al.
\newblock { NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: AI Flash Portrait (Track 3) }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Gui et~al.(2024)Gui, Song, Qin, and Tang]{gui2024remote}
Shengxi Gui, Shuang Song, Rongjun Qin, and Yang Tang.
\newblock Remote sensing object detection in the deep learning era—a review.
\newblock \emph{Remote Sensing}, 16\penalty0 (2):\penalty0 327, 2024.

\bibitem[Guo et~al.(2022)Guo, Mu, Chen, Wang, Yu, and Luo]{guo2022scale}
Qiushan Guo, Yao Mu, Jianyu Chen, Tianqi Wang, Yizhou Yu, and Ping Luo.
\newblock Scale-equivalent distillation for semi-supervised object detection.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2022.

\bibitem[Guo et~al.(2020)Guo, Codella, Karlinsky, Codella, Smith, Saenko, Rosing, and Feris]{guo2020broader}
Yunhui Guo, Noel~C Codella, Leonid Karlinsky, James~V Codella, John~R Smith, Kate Saenko, Tajana Rosing, and Rogerio Feris.
\newblock A broader study of cross-domain few-shot learning.
\newblock In \emph{ECCV}, 2020.

\bibitem[Gushchin et~al.(2026)Gushchin, Abud, Shumitskaya, Filippov, Bychkov, Lavrushkin, Erofeev, Antsiferova, Chen, Tan, Timofte, Vatolin, et~al.]{ntire26aigendet}
Aleksandr Gushchin, Khaled Abud, Ekaterina Shumitskaya, Artem Filippov, Georgii Bychkov, Sergey Lavrushkin, Mikhail Erofeev, Anastasia Antsiferova, Changsheng Chen, Shunquan Tan, Radu Timofte, Dmitriy Vatolin, et~al.
\newblock { NTIRE 2026 Challenge on Robust AI-Generated Image Detection in the Wild }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Hopf et~al.(2026)Hopf, Timofte, et~al.]{ntire26deepfake}
Benedikt Hopf, Radu Timofte, et~al.
\newblock { Robust Deepfake Detection, NTIRE 2026 Challenge: Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Hsieh et~al.(2017)Hsieh, Lin, and Hsu]{hsieh2017drone}
Meng-Ru Hsieh, Yen-Liang Lin, and Winston~H Hsu.
\newblock Drone-based object counting by spatially regularized regional proposal network.
\newblock In \emph{Proceedings of the IEEE international conference on computer vision}, 2017.

\bibitem[Hu et~al.(2022)Hu, Shen, Wallis, Allen-Zhu, Li, Wang, Wang, and Chen]{lora}
Edward~J. Hu, Yelong Shen, Phillip Wallis, Zeyuan Allen-Zhu, Yuanzhi Li, Shean Wang, Lu Wang, and Weizhu Chen.
\newblock Lora: Low-rank adaptation of large language models.
\newblock In \emph{ICLR}. OpenReview.net, 2022.

\bibitem[Inoue et~al.(2018)Inoue, Furuta, Yamasaki, and Aizawa]{inoue2018cross}
Naoto Inoue, Ryosuke Furuta, Toshihiko Yamasaki, and Kiyoharu Aizawa.
\newblock Cross-domain weakly-supervised object detection through progressive domain adaptation.
\newblock In \emph{CVPR}, 2018.

\bibitem[Jiang et~al.(2021)Jiang, Wang, Jia, Xu, Liu, Fan, Li, Liu, Xue, and Wang]{jiang2021underwater}
Lihao Jiang, Yi Wang, Qi Jia, Shengwei Xu, Yu Liu, Xin Fan, Haojie Li, Risheng Liu, Xinwei Xue, and Ruili Wang.
\newblock Underwater species detection using channel sharpening attention.
\newblock In \emph{ACM MM}, 2021.

\bibitem[Jiang et~al.(2024)Jiang, luo, Yang, Xiong, Chen, Zeng, Ren, and Zhang]{jiang2024chatrextamingmultimodalllm}
Qing Jiang, Gen luo, Yuqin Yang, Yuda Xiong, Yihao Chen, Zhaoyang Zeng, Tianhe Ren, and Lei Zhang.
\newblock Chatrex: Taming multimodal llm for joint perception and understanding, 2024.

\bibitem[Kamath et~al.(2021)Kamath, Singh, LeCun, Synnaeve, Misra, and Carion]{kamath2021mdetr}
Aishwarya Kamath, Mannat Singh, Yann LeCun, Gabriel Synnaeve, Ishan Misra, and Nicolas Carion.
\newblock Mdetr-modulated detection for end-to-end multi-modal understanding.
\newblock In \emph{ICCV}, 2021.

\bibitem[Khalin et~al.(2026)Khalin, Ershov, Panshin, Korchagin, Lobarev, Terekhin, Dorogova, Shamsutdinov, Mamedov, Khalfin, Sheludko, Zilyaev, Banić, Perevozchikov, Timofte, et~al.]{ntire26twilight}
Aleksei Khalin, Egor Ershov, Artem Panshin, Sergey Korchagin, Georgiy Lobarev, Arseniy Terekhin, Sofiia Dorogova, Amir Shamsutdinov, Yasin Mamedov, Bakhtiyar Khalfin, Bogdan Sheludko, Emil Zilyaev, Nikola Banić, Georgy Perevozchikov, Radu Timofte, et~al.
\newblock { NTIRE 2026 Low-light Enhancement: Twilight Cowboy Challenge }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[K{\"o}hler et~al.(2023)K{\"o}hler, Eisenbach, and Gross]{kohler2023few}
Mona K{\"o}hler, Markus Eisenbach, and Horst-Michael Gross.
\newblock Few-shot object detection: A comprehensive survey.
\newblock \emph{IEEE Transactions on Neural Networks and Learning Systems}, 2023.

\bibitem[Krishna et~al.(2017{\natexlab{a}})Krishna, Zhu, Groth, Johnson, Hata, Kravitz, Chen, Kalantidis, Li, Shamma, et~al.]{krishna2017visual}
Ranjay Krishna, Yuke Zhu, Oliver Groth, Justin Johnson, Kenji Hata, Joshua Kravitz, Stephanie Chen, Yannis Kalantidis, Li-Jia Li, David~A Shamma, et~al.
\newblock Visual genome: Connecting language and vision using crowdsourced dense image annotations.
\newblock \emph{International journal of computer vision}, 2017{\natexlab{a}}.

\bibitem[Krishna et~al.(2017{\natexlab{b}})]{krishna2017vg}
Ranjay Krishna et~al.
\newblock Visual genome.
\newblock In \emph{IJCV}, 2017{\natexlab{b}}.

\bibitem[Krizhevsky et~al.(2012)Krizhevsky, Sutskever, and Hinton]{krizhevsky2012imagenet}
Alex Krizhevsky, Ilya Sutskever, and Geoffrey~E Hinton.
\newblock Imagenet classification with deep convolutional neural networks.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2012.

\bibitem[Kuznetsova et~al.(2020)Kuznetsova, Rom, Alldrin, Uijlings, Krasin, Pont-Tuset, Kamali, Popov, Malloci, Kolesnikov, et~al.]{kuznetsova2020open}
Alina Kuznetsova, Hassan Rom, Neil Alldrin, Jasper Uijlings, Ivan Krasin, Jordi Pont-Tuset, Shahab Kamali, Stefan Popov, Matteo Malloci, Alexander Kolesnikov, et~al.
\newblock The open images dataset v4: Unified image classification, object detection, and visual relationship detection at scale.
\newblock \emph{International journal of computer vision}, 2020.

\bibitem[Li et~al.(2025{\natexlab{a}})Li, Wang, Zhang, Zhao, Gao, and Li]{li2025maris}
Bingyu Li, Feiyu Wang, Da Zhang, Zhiyuan Zhao, Junyu Gao, and Xuelong Li.
\newblock Maris: Marine open-vocabulary instance segmentation with geometric enhancement and semantic alignment.
\newblock \emph{arXiv preprint arXiv:2510.15398}, 2025{\natexlab{a}}.

\bibitem[Li et~al.(2022{\natexlab{a}})Li, Liu, Li, Zhang, Aneja, Yang, Jin, Hu, Liu, Lee, et~al.]{li2022elevater}
Chunyuan Li, Haotian Liu, Liunian Li, Pengchuan Zhang, Jyoti Aneja, Jianwei Yang, Ping Jin, Houdong Hu, Zicheng Liu, Yong~Jae Lee, et~al.
\newblock Elevater: A benchmark and toolkit for evaluating language-augmented visual models.
\newblock \emph{Advances in Neural Information Processing Systems}, 2022{\natexlab{a}}.

\bibitem[Li et~al.(2025{\natexlab{b}})Li, Pan, Sun, and Huang]{li2025semantic}
Jiahao Li, Jiancheng Pan, Yuze Sun, and Xiaomeng Huang.
\newblock Semantic-aware ship detection with vision-language integration.
\newblock In \emph{IGARSS 2025-2025 IEEE International Geoscience and Remote Sensing Symposium}, 2025{\natexlab{b}}.

\bibitem[Li et~al.(2026{\natexlab{a}})Li, Chen, Liu, Wang, Zhou, Liu, Zhu, Timofte, Zhang, et~al.]{ntire26rwsr}
Jiatong Li, Zheng Chen, Kai Liu, Jingkai Wang, Zihan Zhou, Xiaoyang Liu, Libo Zhu, Radu Timofte, Yulun Zhang, et~al.
\newblock { The First Challenge on Mobile Real-World Image Super-Resolution at NTIRE 2026: Benchmark Results and Method Overview }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Li et~al.(2020)Li, Wan, Cheng, Meng, and Han]{li2020object}
Ke Li, Gang Wan, Gong Cheng, Liqiu Meng, and Junwei Han.
\newblock Object detection in optical remote sensing images: A survey and a new benchmark.
\newblock \emph{ISPRS}, 2020.

\bibitem[Li et~al.(2022{\natexlab{b}})]{li2022glip}
Liunian Li et~al.
\newblock Grounded language-image pre-training.
\newblock In \emph{CVPR}, 2022{\natexlab{b}}.

\bibitem[Li et~al.(2022{\natexlab{c}})Li, Zhang, Zhang, Yang, Li, Zhong, Wang, Yuan, Zhang, Hwang, et~al.]{li2022grounded}
Liunian~Harold Li, Pengchuan Zhang, Haotian Zhang, Jianwei Yang, Chunyuan Li, Yiwu Zhong, Lijuan Wang, Lu Yuan, Lei Zhang, Jenq-Neng Hwang, et~al.
\newblock Grounded language-image pre-training.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2022{\natexlab{c}}.

\bibitem[Li et~al.(2022{\natexlab{d}})Li, Liu, and Bilen]{li2022cross}
Wei-Hong Li, Xialei Liu, and Hakan Bilen.
\newblock Cross-domain few-shot learning with task-specific adapters.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2022{\natexlab{d}}.

\bibitem[Li et~al.(2026{\natexlab{b}})Li, Gong, Wang, Xiong, Li, Yao, Zhou, Chen, Timofte, et~al.]{ntire26ugcvideo}
Xin Li, Jiachao Gong, Xijun Wang, Shiyao Xiong, Bingchen Li, Suhang Yao, Chao Zhou, Zhibo Chen, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Short-form UGC Video Restoration in the Wild with Generative Models: Datasets, Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Li et~al.(2026{\natexlab{c}})Li, Jin, Yao, Lin, Fan, Yan, Jin, Wu, Li, Shi, Yang, Li, Chen, Wen, Tan, Timofte, et~al.]{ntire26dual_focus}
Xin Li, Yeying Jin, Suhang Yao, Beibei Lin, Zhaoxin Fan, Wending Yan, Xin Jin, Zongwei Wu, Bingchen Li, Peishu Shi, Yufei Yang, Yu Li, Zhibo Chen, Bihan Wen, Robby Tan, Radu Timofte, et~al.
\newblock { NTIRE 2026 The Second Challenge on Day and Night Raindrop Removal for Dual-Focused Images: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{c}}.

\bibitem[Li et~al.(2025{\natexlab{c}})Li, Qiu, Fu, Chen, Qian, Zheng, Paudel, Fu, Huang, Van~Gool, et~al.]{li2025domain}
Yu Li, Xingyu Qiu, Yuqian Fu, Jie Chen, Tianwen Qian, Xu Zheng, Danda~Pani Paudel, Yanwei Fu, Xuanjing Huang, Luc Van~Gool, et~al.
\newblock Domain-rag: Retrieval-guided compositional image generation for cross-domain few-shot object detection.
\newblock \emph{arXiv preprint arXiv:2506.05872}, 2025{\natexlab{c}}.

\bibitem[Lin et~al.(2014{\natexlab{a}})Lin, Maire, Belongie, Hays, Perona, Ramanan, Doll{\'a}r, and Zitnick]{lin2014microsoft}
Tsung-Yi Lin, Michael Maire, Serge Belongie, James Hays, Pietro Perona, Deva Ramanan, Piotr Doll{\'a}r, and C~Lawrence Zitnick.
\newblock Microsoft coco: Common objects in context.
\newblock In \emph{ECCV}, 2014{\natexlab{a}}.

\bibitem[Lin et~al.(2014{\natexlab{b}})]{lin2014coco}
Tsung-Yi Lin et~al.
\newblock Microsoft coco.
\newblock In \emph{ECCV}, 2014{\natexlab{b}}.

\bibitem[Lin et~al.(2017)]{lin2017focal}
Tsung-Yi Lin et~al.
\newblock Focal loss.
\newblock In \emph{ICCV}, 2017.

\bibitem[Liu et~al.(2026{\natexlab{a}})Liu, Yue, Lin, Chen, Wang, Gong, Timofte, Zhang, et~al.]{ntire26rsirsr}
Kai Liu, Haoyang Yue, Zeli Lin, Zheng Chen, Jingkai Wang, Jue Gong, Radu Timofte, Yulun Zhang, et~al.
\newblock { The First Challenge on Remote Sensing Infrared Image Super-Resolution at NTIRE 2026: Benchmark Results and Method Overview }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Liu et~al.(2023)Liu, Zeng, Ren, Li, Zhang, Yang, Li, Yang, Su, Zhu, et~al.]{groundingdino}
Shilong Liu, Zhaoyang Zeng, Tianhe Ren, Feng Li, Hao Zhang, Jie Yang, Chunyuan Li, Jianwei Yang, Hang Su, Jun Zhu, et~al.
\newblock Grounding dino: Marrying dino with grounded pre-training for open-set object detection.
\newblock \emph{arXiv preprint arXiv:2303.05499}, 2023.

\bibitem[Liu et~al.(2024)Liu, Zeng, Ren, Li, Zhang, Yang, Jiang, Li, Yang, Su, et~al.]{liu2024grounding}
Shilong Liu, Zhaoyang Zeng, Tianhe Ren, Feng Li, Hao Zhang, Jie Yang, Qing Jiang, Chunyuan Li, Jianwei Yang, Hang Su, et~al.
\newblock Grounding dino: Marrying dino with grounded pre-training for open-set object detection.
\newblock In \emph{European Conference on Computer Vision}, 2024.

\bibitem[Liu et~al.(2026{\natexlab{b}})Liu, Cui, Bao, Chu, Gu, Ren, Timofte, Conde, et~al.]{ntire26realx3d}
Shuhong Liu, Ziteng Cui, Chenyu Bao, Xuangeng Chu, Lin Gu, Bin Ren, Radu Timofte, Marcos~V. Conde, et~al.
\newblock { 3D Restoration and Reconstruction in Adverse Conditions: RealX3D Challenge Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Liu et~al.(2026{\natexlab{c}})Liu, Min, Zhai, Hu, Cao, Zhou, Sun, Wen, Xu, Zhou, Duan, Liu, Wang, Luo, Li, Xu, Zhang, Shi, Wang, Zhang, Guo, Hu, Chen, Wu, Ma, Lv, Xue, Wang, Sha, Timofte, et~al.]{ntire26XAIGCqa}
Xiaohong Liu, Xiongkuo Min, Guangtao Zhai, Qiang Hu, Jiezhang Cao, Yu Zhou, Wei Sun, Farong Wen, Zitong Xu, Yingjie Zhou, Huiyu Duan, Lu Liu, Jiarui Wang, Siqi Luo, Chunyi Li, Li Xu, Zicheng Zhang, Yue Shi, Yubo Wang, Minghong Zhang, Chunchao Guo, Zhichao Hu, Mingtao Chen, Xiele Wu, Xin Ma, Zhaohe Lv, Yuanhao Xue, Jiaqi Wang, Xinxing Sha, Radu Timofte, et~al.
\newblock { NTIRE 2026 X-AIGC Quality Assessment Challenge: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{c}}.

\bibitem[Liu et~al.(2025)Liu, Pan, Yang, Chen, Zhou, and Zhang]{liu2025diverse}
Yanxing Liu, Jiancheng Pan, Jianwei Yang, Tiancheng Chen, Peiling Zhou, and Bingchen Zhang.
\newblock Diverse instance generation via diffusion models for enhanced few-shot object detection in remote sensing images.
\newblock \emph{IEEE Geoscience and Remote Sensing Letters}, 2025.

\bibitem[Liu et~al.(2021)Liu, Lin, Cao, Hu, Wei, Zhang, Lin, and Guo]{liu2021swin}
Ze Liu, Yutong Lin, Yue Cao, Han Hu, Yixuan Wei, Zheng Zhang, Stephen Lin, and Baining Guo.
\newblock Swin transformer: Hierarchical vision transformer using shifted windows.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, 2021.

\bibitem[Meng et~al.(2025)Meng, Zhang, Li, Wu, Li, Zhao, Yu, and Shen]{meng2025cdformer}
Boyuan Meng, Xiaohan Zhang, Peilin Li, Zhe Wu, Yiming Li, Wenkai Zhao, Beinan Yu, and Hui-Liang Shen.
\newblock Cdformer: Cross-domain few-shot object detection transformer against feature confusion.
\newblock In \emph{ICME}, 2025.

\bibitem[Moskalenko et~al.(2026)Moskalenko, Bryncev, Kosmynin, Shilovskaya, Erofeev, Vatolin, Timofte, et~al.]{ntire26videosal}
Andrey Moskalenko, Alexey Bryncev, Ivan Kosmynin, Kira Shilovskaya, Mikhail Erofeev, Dmitry Vatolin, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Video Saliency Prediction: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Oquab et~al.(2024)Oquab, Darcet, Moutakanni, Vo, Szafraniec, Khalidov, Fernandez, Haziza, Massa, El-Nouby, et~al.]{oquab2024dinov2}
Maxime Oquab, Timoth{\'e}e Darcet, Th{\'e}o Moutakanni, Huy~V. Vo, Marc Szafraniec, Vasil Khalidov, Pierre Fernandez, Daniel Haziza, Francisco Massa, Alaaeldin El-Nouby, et~al.
\newblock {DINOv2}: Learning robust visual features without supervision.
\newblock \emph{Transactions on Machine Learning Research}, 2024.

\bibitem[Ordonez et~al.(2011)Ordonez, Kulkarni, and Berg]{ordonez2011im2text}
Vicente Ordonez, Girish Kulkarni, and Tamara Berg.
\newblock Im2text: Describing images using 1 million captioned photographs.
\newblock \emph{Advances in neural information processing systems}, 24, 2011.

\bibitem[Pan et~al.(2025{\natexlab{a}})Pan, Liu, Fu, Ma, Li, Paudel, Van~Gool, and Huang]{pan2025locate}
Jiancheng Pan, Yanxing Liu, Yuqian Fu, Muyuan Ma, Jiahao Li, Danda~Pani Paudel, Luc Van~Gool, and Xiaomeng Huang.
\newblock Locate anything on earth: Advancing open-vocabulary object detection for remote sensing community.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, 2025{\natexlab{a}}.

\bibitem[Pan et~al.(2025{\natexlab{b}})Pan, Liu, He, Peng, Li, Sun, and Huang]{pan2025enhance}
Jiancheng Pan, Yanxing Liu, Xiao He, Long Peng, Jiahao Li, Yuze Sun, and Xiaomeng Huang.
\newblock Enhance then search: An augmentation-search strategy with foundation models for cross-domain few-shot object detection.
\newblock In \emph{Proceedings of the Computer Vision and Pattern Recognition Conference}, 2025{\natexlab{b}}.

\bibitem[Park et~al.(2026)Park, Park, Lee, Timofte, et~al.]{ntire26bursthdr}
Hyunhee Park, Eunpil Park, Sangmin Lee, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Efficient Burst HDR and Restoration: Datasets, Methods, and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Perevozchikov et~al.(2026)Perevozchikov, Vladimirov, Timofte, et~al.]{ntire26isp}
Georgy Perevozchikov, Daniil Vladimirov, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Learned Smartphone ISP with Unpaired Data: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Qiao et~al.(2021)Qiao, Zhao, Li, Qiu, Wu, and Zhang]{qiao2021defrcn}
Limeng Qiao, Yuxuan Zhao, Zhiyuan Li, Xi Qiu, Jianan Wu, and Chi Zhang.
\newblock Defrcn: Decoupled faster r-cnn for few-shot object detection.
\newblock In \emph{ICCV}, 2021.

\bibitem[Qin et~al.(2026)Qin, Liang, Zhang, Qu, Guan, Zeng, Zhang, Timofte, et~al.]{ntire26raim_piqa}
Guanyi Qin, Jie Liang, Bingbing Zhang, Lishen Qu, Ya-nan Guan, Hui Zeng, Lei Zhang, Radu Timofte, et~al.
\newblock { NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: Professional Image Quality Assessment (Track 1) }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Qiu et~al.(2026)Qiu, Fu, Geng, Ren, Pan, Wu, Tang, Fu, Timofte, Sebe, Elhoseiny, et~al.]{ntire26cdfsod}
Xingyu Qiu, Yuqian Fu, Jiawei Geng, Bin Ren, Jiancheng Pan, Zongwei Wu, Hao Tang, Yanwei Fu, Radu Timofte, Nicu Sebe, Mohamed Elhoseiny, et~al.
\newblock { The Second Challenge on Cross-Domain Few-Shot Object Detection at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Qu et~al.(2026)Qu, Liu, Liang, Zeng, Dai, Guan, Qin, Zhou, Yang, Zhang, Timofte, et~al.]{ntire26raim_fusion}
Lishen Qu, Yao Liu, Jie Liang, Hui Zeng, Wen Dai, Ya-nan Guan, Guanyi Qin, Shihao Zhou, Jufeng Yang, Lei Zhang, Radu Timofte, et~al.
\newblock { NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: Multi-Exposure Image Fusion in Dynamic Scenes (Track2) }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[{Qwen Team}(2026)]{qwen3.5}
{Qwen Team}.
\newblock {Qwen3.5}: Towards native multimodal agents, 2026.

\bibitem[Radford et~al.(2021)Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin, Clark, Krueger, and Sutskever]{clip}
Alec Radford, Jong~Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, Gretchen Krueger, and Ilya Sutskever.
\newblock Learning transferable visual models from natural language supervision.
\newblock In \emph{ICML}, 2021.

\bibitem[Ravi et~al.(2024)Ravi, Gabeur, Hu, Hu, Ryali, Ma, Khedr, R{\"a}dle, Rolland, Gustafson, et~al.]{ravi2024sam2}
Nikhila Ravi, Valentin Gabeur, Yuan-Ting Hu, Ronghang Hu, Chaitanya Ryali, Tengyu Ma, Haitham Khedr, Roman R{\"a}dle, Chloe Rolland, Laura Gustafson, et~al.
\newblock {SAM} 2: Segment anything in images and videos.
\newblock \emph{arXiv preprint arXiv:2408.00714}, 2024.

\bibitem[Ren et~al.(2024)Ren, Li, Liang, Ranjan, Liu, Cucchiara, Gool, Yang, and Sebe]{ren2024sharing}
Bin Ren, Yawei Li, Jingyun Liang, Rakesh Ranjan, Mengyuan Liu, Rita Cucchiara, Luc~V Gool, Ming-Hsuan Yang, and Nicu Sebe.
\newblock Sharing key semantics in transformer makes efficient image restoration.
\newblock \emph{Advances in Neural Information Processing Systems}, 37:\penalty0 7427--7463, 2024.

\bibitem[Ren et~al.(2026)Ren, Guo, Shu, Ma, Cui, Liu, Mei, Sun, Wu, Khan, Khan, Timofte, Li, et~al.]{ntire26effsr}
Bin Ren, Hang Guo, Yan Shu, Jiaqi Ma, Ziteng Cui, Shuhong Liu, Guofeng Mei, Lei Sun, Zongwei Wu, Fahad~Shahbaz Khan, Salman Khan, Radu Timofte, Yawei Li, et~al.
\newblock { The Eleventh NTIRE 2026 Efficient Super-Resolution Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Ren et~al.(2015)Ren, He, Girshick, and Sun]{ren2015faster}
Shaoqing Ren, Kaiming He, Ross Girshick, and Jian Sun.
\newblock Faster {R-CNN}: Towards real-time object detection with region proposal networks.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2015.

\bibitem[Ren et~al.(2016)Ren, He, Girshick, and Sun]{fasterrcnn}
Shaoqing Ren, Kaiming He, Ross Girshick, and Jian Sun.
\newblock Faster r-cnn: Towards real-time object detection with region proposal networks.
\newblock \emph{IEEE transactions on pattern analysis and machine intelligence}, 2016.

\bibitem[Rezatofighi et~al.(2019)]{rezatofighi2019giou}
Hamid Rezatofighi et~al.
\newblock Generalized intersection over union.
\newblock In \emph{CVPR}, 2019.

\bibitem[Saleh et~al.(2020)Saleh, Laradji, Konovalov, Bradley, Vazquez, and Sheaves]{saleh2020realistic}
Alzayat Saleh, Issam~H Laradji, Dmitry~A Konovalov, Michael Bradley, David Vazquez, and Marcus Sheaves.
\newblock A realistic fish-habitat dataset to evaluate algorithms for underwater visual analysis.
\newblock \emph{Scientific Reports}, 2020.

\bibitem[Seizinger et~al.(2026)Seizinger, Vasluianu, Conde, Chen, Zhou, Wu, Timofte, et~al.]{ntire26bokeh}
Tim Seizinger, Florin-Alexandru Vasluianu, Marcos~V. Conde, Jeffrey Chen, Zhuyun Zhou, Zongwei Wu, Radu Timofte, et~al.
\newblock { The First Controllable Bokeh Rendering Challenge at NTIRE 2026 }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Shangguan and Rostami(2023)]{shangguan2023identification}
Zeyu Shangguan and Mohammad Rostami.
\newblock Identification of novel classes for improving few-shot object detection.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, 2023.

\bibitem[Shangguan and Rostami(2024)]{shangguan2024improved}
Zeyu Shangguan and Mohammad Rostami.
\newblock Improved region proposal network for enhanced few-shot object detection.
\newblock \emph{Neural Networks}, 180:\penalty0 106699, 2024.

\bibitem[Shao et~al.(2019{\natexlab{a}})Shao, Li, Zhang, Peng, Yu, Zhang, Li, and Sun]{object365}
Shuai Shao, Zeming Li, Tianyuan Zhang, Chao Peng, Gang Yu, Xiangyu Zhang, Jing Li, and Jian Sun.
\newblock Objects365: A large-scale, high-quality dataset for object detection.
\newblock In \emph{ICCV}, 2019{\natexlab{a}}.

\bibitem[Shao et~al.(2019{\natexlab{b}})Shao, Li, Zhang, Peng, Yu, Zhang, Li, and Sun]{shao2019objects365}
Shuai Shao, Zeming Li, Tianyuan Zhang, Chao Peng, Gang Yu, Xiangyu Zhang, Jing Li, and Jian Sun.
\newblock Objects365: A large-scale, high-quality dataset for object detection.
\newblock In \emph{ICCV}, 2019{\natexlab{b}}.

\bibitem[Sim{\'e}oni et~al.(2025)Sim{\'e}oni, Vo, Seitzer, Baldassarre, Oquab, Jose, Khalidov, Szafraniec, Yi, Ramamonjisoa, et~al.]{simeoni2025dinov3}
Oriane Sim{\'e}oni, Huy~V Vo, Maximilian Seitzer, Federico Baldassarre, Maxime Oquab, Cijo Jose, Vasil Khalidov, Marc Szafraniec, Seungeun Yi, Micha{\"e}l Ramamonjisoa, et~al.
\newblock Dinov3.
\newblock \emph{arXiv preprint arXiv:2508.10104}, 2025.

\bibitem[Solovyev et~al.(2021)Solovyev, Wang, and Gabruseva]{solovyev2021weighted}
Roman Solovyev, Weimin Wang, and Tatiana Gabruseva.
\newblock Weighted boxes fusion: Ensembling boxes from different object detection models.
\newblock \emph{Image and Vision Computing}, 2021.

\bibitem[Song and Yan(2013)]{song2013noise}
Kechen Song and Yunhui Yan.
\newblock A noise robust method based on completed local binary patterns for hot-rolled steel strip surface defects.
\newblock \emph{Applied Surface Science}, 2013.

\bibitem[Sun et~al.(2021)Sun, Li, Cai, Yuan, and Zhang]{sun2021fsce}
Bo Sun, Banghuai Li, Shengcai Cai, Ye Yuan, and Chi Zhang.
\newblock Fsce: Few-shot object detection via contrastive proposal encoding.
\newblock In \emph{CVPR}, 2021.

\bibitem[Sun et~al.(2026{\natexlab{a}})Sun, Guo, Ren, Su, Wang, Pani~Paudel, Van~Gool, Timofte, Li, et~al.]{ntire26denoising}
Lei Sun, Hang Guo, Bin Ren, Shaolin Su, Xian Wang, Danda Pani~Paudel, Luc Van~Gool, Radu Timofte, Yawei Li, et~al.
\newblock { The Third Challenge on Image Denoising at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Sun et~al.(2026{\natexlab{b}})Sun, Li, Wang, Li, Shi, Xu, Zhang, Hu, Guo, Su, Timofte, Pani~Paudel, Van~Gool, et~al.]{ntire26eventblurr}
Lei Sun, Weilun Li, Xian Wang, Zhendong Li, Letian Shi, Dannong Xu, Deheng Zhang, Mengshun Hu, Shuang Guo, Shaolin Su, Radu Timofte, Danda Pani~Paudel, Luc Van~Gool, et~al.
\newblock { The Second Challenge on Event-Based Image Deblurring at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Sun et~al.(2026{\natexlab{c}})Sun, Qian, Jiang, Wang, Gao, Yang, Wang, Timofte, Pani~Paudel, Van~Gool, et~al.]{ntire26aberration}
Lei Sun, Xiaolong Qian, Qi Jiang, Xian Wang, Yao Gao, Kailun Yang, Kaiwei Wang, Radu Timofte, Danda Pani~Paudel, Luc Van~Gool, et~al.
\newblock { NTIRE 2026 The First Challenge on Blind Computational Aberration Correction: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{c}}.

\bibitem[Tang et~al.(2022)Tang, Yuan, Li, and Tang]{tang2022learning}
Hao Tang, Chengcheng Yuan, Zechao Li, and Jinhui Tang.
\newblock Learning attention-guided pyramidal features for few-shot fine-grained recognition.
\newblock \emph{Pattern Recognition}, 130:\penalty0 108792, 2022.

\bibitem[Team(2024)]{diffsynth2024}
DiffSynth Team.
\newblock Diffsynth studio: Enjoy the magic of diffusion models!
\newblock \emph{GitHub Repository}, 2024.
\newblock \url{https://github.com/modelscope/DiffSynth-Studio}.

\bibitem[Tschannen et~al.(2023)Tschannen, Kumar, Steiner, Zhai, Houlsby, and Beyer]{cappa}
Michael Tschannen, Manoj Kumar, Andreas Steiner, Xiaohua Zhai, Neil Houlsby, and Lucas Beyer.
\newblock Image captioners are scalable vision learners too.
\newblock In \emph{Proceedings of the 37th International Conference on Neural Information Processing Systems}, 2023.

\bibitem[Tseng et~al.(2020)Tseng, Lee, Huang, and Yang]{tseng2020cross}
Hung-Yu Tseng, Hsin-Ying Lee, Jia-Bin Huang, and Ming-Hsuan Yang.
\newblock Cross-domain few-shot classification via learned feature-wise transformation.
\newblock \emph{arXiv preprint arXiv:2001.08735}, 2020.

\bibitem[Vasluianu et~al.(2026{\natexlab{a}})Vasluianu, Seizinger, Chen, Zhou, Wu, Timofte, et~al.]{ntire26lightnorm}
Florin-Alexandru Vasluianu, Tim Seizinger, Jeffrey Chen, Zhuyun Zhou, Zongwei Wu, Radu Timofte, et~al.
\newblock { Learning-Based Ambient Lighting Normalization: NTIRE 2026 Challenge Results and Findings }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Vasluianu et~al.(2026{\natexlab{b}})Vasluianu, Seizinger, Zhou, Wu, Timofte, et~al.]{ntire26shadow}
Florin-Alexandru Vasluianu, Tim Seizinger, Zhuyun Zhou, Zongwei Wu, Radu Timofte, et~al.
\newblock { Advances in Single-Image Shadow Removal: Results from the NTIRE 2026 Challenge }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Wang et~al.(2025)Wang, Liu, Chen, Lin, Han, and Ding]{yoloe}
Ao Wang, Lihao Liu, Hui Chen, Zijia Lin, Jungong Han, and Guiguang Ding.
\newblock Yoloe: Real-time seeing anything, 2025.

\bibitem[Wang et~al.(2026{\natexlab{a}})Wang, Gong, Chen, Liu, Li, Zhang, Timofte, et~al.]{ntire26faceres}
Jingkai Wang, Jue Gong, Zheng Chen, Kai Liu, Jiatong Li, Yulun Zhang, Radu Timofte, et~al.
\newblock { The Second Challenge on Real-World Face Restoration at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Wang et~al.(2026{\natexlab{b}})Wang, Guo, Wang, Li, Peng, Zhang, Timofte, Chen, Wang, Hu, Lei, et~al.]{ntire263dsr}
Longguang Wang, Yulan Guo, Yingqian Wang, Juncheng Li, Sida Peng, Ye Zhang, Radu Timofte, Minglin Chen, Yi Wang, Qibin Hu, Wenjie Lei, et~al.
\newblock { NTIRE 2026 Challenge on 3D Content Super-Resolution: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Wang et~al.(2024)Wang, Bai, Tan, Wang, Fan, Bai, Chen, Liu, Wang, Ge, et~al.]{wang2024qwen2}
Peng Wang, Shuai Bai, Sinan Tan, Shijie Wang, Zhihao Fan, Jinze Bai, Keqin Chen, Xuejing Liu, Jialin Wang, Wenbin Ge, et~al.
\newblock Qwen2-vl: Enhancing vision-language model's perception of the world at any resolution.
\newblock \emph{arXiv preprint arXiv:2409.12191}, 2024.

\bibitem[Wang et~al.(2026{\natexlab{c}})Wang, Guo, Cai, and Chen]{wang2026learning}
Wanqi Wang, Jingcai Guo, Yuxiang Cai, and Zhi Chen.
\newblock Learning multi-modal prototypes for cross-domain few-shot object detection.
\newblock \emph{arXiv preprint arXiv:2602.18811}, 2026{\natexlab{c}}.

\bibitem[Wang et~al.(2020)Wang, Huang, Darrell, Gonzalez, and Yu]{wang2020frustratingly}
Xin Wang, Thomas~E Huang, Trevor Darrell, Joseph~E Gonzalez, and Fisher Yu.
\newblock Frustratingly simple few-shot object detection.
\newblock \emph{arXiv preprint arXiv:2003.06957}, 2020.

\bibitem[Wang et~al.(2023)Wang, Li, and Wu]{wang2023cardd}
Xinkuang Wang, Wenjing Li, and Zhongcheng Wu.
\newblock Cardd: A new dataset for vision-based car damage detection.
\newblock \emph{IEEE Transactions on Intelligent Transportation Systems}, 2023.

\bibitem[Wang et~al.(2026{\natexlab{d}})Wang, Liang, Zhang, Zhao, Wang, Li, Yang, Timofte, Guo, et~al.]{ntire26lightsr}
Yingqian Wang, Zhengyu Liang, Fengyuan Zhang, Wending Zhao, Longguang Wang, Juncheng Li, Jungang Yang, Radu Timofte, Yulan Guo, et~al.
\newblock { NTIRE 2026 Challenge on Light Field Image Super-Resolution: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{d}}.

\bibitem[Wolf et~al.(2020)Wolf, Debut, Sanh, Chaumond, Delangue, Moi, Cistac, Rault, Louf, Funtowicz, Davison, Shleifer, von Platen, Ma, Jernite, Plu, Xu, Scao, Gugger, Drame, Lhoest, and Rush]{transformers}
Thomas Wolf, Lysandre Debut, Victor Sanh, Julien Chaumond, Clement Delangue, Anthony Moi, Pierric Cistac, Tim Rault, Rémi Louf, Morgan Funtowicz, Joe Davison, Sam Shleifer, Patrick von Platen, Clara Ma, Yacine Jernite, Julien Plu, Canwen Xu, Teven~Le Scao, Sylvain Gugger, Mariama Drame, Quentin Lhoest, and Alexander~M. Rush.
\newblock Transformers: State-of-the-art natural language processing.
\newblock 2020.

\bibitem[Wu et~al.(2025{\natexlab{a}})Wu, Li, Zhou, Lin, Gao, Yan, ming Yin, Bai, Xu, Chen, Chen, Tang, Zhang, Wang, Yang, Yu, Cheng, Liu, Li, Zhang, Meng, Wei, Ni, Chen, Cao, Peng, Qu, Wu, Wang, Yu, Wen, Feng, Xu, Wang, Zhang, Zhu, Wu, Cai, and Liu]{qwenimage}
Chenfei Wu, Jiahao Li, Jingren Zhou, Junyang Lin, Kaiyuan Gao, Kun Yan, Sheng ming Yin, Shuai Bai, Xiao Xu, Yilei Chen, Yuxiang Chen, Zecheng Tang, Zekai Zhang, Zhengyi Wang, An Yang, Bowen Yu, Chen Cheng, Dayiheng Liu, Deqing Li, Hang Zhang, Hao Meng, Hu Wei, Jingyuan Ni, Kai Chen, Kuan Cao, Liang Peng, Lin Qu, Minggang Wu, Peng Wang, Shuting Yu, Tingkun Wen, Wensen Feng, Xiaoxiao Xu, Yi Wang, Yichang Zhang, Yongqiang Zhu, Yujia Wu, Yuxuan Cai, and Zenan Liu.
\newblock Qwen-image technical report, 2025{\natexlab{a}}.

\bibitem[Wu et~al.(2025{\natexlab{b}})Wu, Li, Zhou, Lin, Gao, Yan, Yin, Bai, Xu, Chen, et~al.]{wu2025qwen}
Chenfei Wu, Jiahao Li, Jingren Zhou, Junyang Lin, Kaiyuan Gao, Kun Yan, Sheng-ming Yin, Shuai Bai, Xiao Xu, Yilei Chen, et~al.
\newblock Qwen-image technical report.
\newblock \emph{arXiv preprint arXiv:2508.02324}, 2025{\natexlab{b}}.

\bibitem[Yan et~al.(2026)Yan, Tu, Lin, WU, Zhang, Wang, Cao, Fang, Liu, Zhou, Timofte, et~al.]{ntire26effllie}
Jiebin Yan, Chenyu Tu, Qinghua Lin, Zongwei WU, Weixia Zhang, Zhihua Wang, Peibei Cao, Yuming Fang, Xiaoning Liu, Zhuyun Zhou, Radu Timofte, et~al.
\newblock { Efficient Low Light Image Enhancement: NTIRE 2026 Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Yang and Xie(2026)]{yang2026styleproto}
Xi Yang and Quantao Xie.
\newblock Styleproto: Style-augmented prototype learning for cross-domain few-shot object detection.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, 2026.

\bibitem[Yu et~al.(2026)Yu, Sha, Liu, Shen, and Yang]{yu2026acloser}
Xuanlong Yu, Youyang Sha, Longfei Liu, Xi Shen, and Di Yang.
\newblock A closer look at cross-domain few-shot object detection: Fine-tuning matters and parallel decoder helps.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 2026.

\bibitem[Zama~Ramirez et~al.(2026)Zama~Ramirez, Tosi, Di~Stefano, Timofte, Costanzino, Poggi, Salti, Mattoccia, et~al.]{ntire26hrdepth}
Pierluigi Zama~Ramirez, Fabio Tosi, Luigi Di~Stefano, Radu Timofte, Alex Costanzino, Matteo Poggi, Samuele Salti, Stefano Mattoccia, et~al.
\newblock { NTIRE 2026 Challenge on High-Resolution Depth of non-Lambertian Surfaces }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Zha et~al.(2023)Zha, Tang, Sun, and Tang]{zha2023boosting}
Zican Zha, Hao Tang, Yunlian Sun, and Jinhui Tang.
\newblock Boosting few-shot fine-grained recognition with background suppression and foreground alignment.
\newblock \emph{IEEE TCSVT}, 2023.

\bibitem[Zhang et~al.(2022)Zhang, Song, Gao, and Shen]{zhang2022free}
Ji Zhang, Jingkuan Song, Lianli Gao, and Hengtao Shen.
\newblock Free-lunch for cross-domain few-shot learning: Style-aware episodic training with robust contrastive learning.
\newblock In \emph{ACM multimedia}, 2022.

\bibitem[Zhang et~al.(2023)Zhang, Liu, Wang, and Boularias]{zhang2023detect}
Xinyu Zhang, Yuhan Liu, Yuting Wang, and Abdeslam Boularias.
\newblock Detect everything with few examples.
\newblock \emph{arXiv preprint arXiv:2309.12969}, 2023.

\bibitem[Zhao et~al.(2024{\natexlab{a}})]{zhao2024upn}
Hengyue Zhao et~al.
\newblock Universal proposal network for multi-domain visual context understanding.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 2024{\natexlab{a}}.

\bibitem[Zhao et~al.(2024{\natexlab{b}})Zhao, Chen, Xu, Li, Wang, Li, and Huang]{zhao2024open}
Xiangyu Zhao, Yicheng Chen, Shilin Xu, Xiangtai Li, Xinjiang Wang, Yining Li, and Haian Huang.
\newblock An open and comprehensive pipeline for unified object grounding and detection.
\newblock \emph{arXiv preprint arXiv:2401.02361}, 2024{\natexlab{b}}.

\bibitem[Zhong et~al.(2026)Zhong, Ma, Wang, Jiang, Timofte, et~al.]{ntire26anomalydet}
Yan Zhong, Qiufang Ma, Zhen Wang, Tingting Jiang, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge Report on Anomaly Detection of Face Enhancement for UGC Images }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Zhuo et~al.(2022)Zhuo, Fu, Chen, Cao, and Jiang]{zhuo2022tgdm}
Linhai Zhuo, Yuqian Fu, Jingjing Chen, Yixin Cao, and Yu-Gang Jiang.
\newblock Tgdm: Target guided dynamic mixup for cross-domain few-shot learning.
\newblock In \emph{ACM Multimedia}, 2022.

\bibitem[Zhuo et~al.(2024)Zhuo, Fu, Chen, Cao, and Jiang]{zhuo2024unified}
Linhai Zhuo, Yuqian Fu, Jingjing Chen, Yixin Cao, and Yu-Gang Jiang.
\newblock Unified view empirical study for large pretrained model on cross-domain few-shot learning.
\newblock \emph{ACM Transactions on Multimedia Computing, Communications and Applications}, 2024.

\bibitem[Zhuo et~al.(2026)Zhuo, Wang, Qian, and Fu]{zhuo2026segdp}
Linhai Zhuo, Zheng Wang, Tianwen Qian, and Yuqian Fu.
\newblock Segdp: Source-free cross-domain few-shot learning via semantic guided diversity prompting.
\newblock \emph{ACM Transactions on Multimedia Computing, Communications and Applications}, 2026.

\bibitem[Zong et~al.(2023)Zong, Song, and Liu]{codetr}
Zhuofan Zong, Guanglu Song, and Yu Liu.
\newblock Detrs with collaborative hybrid assignments training.
\newblock In \emph{ICCV}, 2023.

\bibitem[Zou et~al.(2026)Zou, Liu, Wu, Zhuang, Wu, Zhou, Timofte, et~al.]{ntire26videores}
Wenbin Zou, Tianyi Liu, Kejun Wu, Huiping Zhuang, Zongwei Wu, Zhuyun Zhou, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Bitstream-Corrupted Video Restoration: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\end{thebibliography}


==> ntire26/affiliation.tex <==
\subsection*{NTIRE 2026 team}
\noindent\textit{\textbf{Title: }} NTIRE 2026 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.\\
\noindent\textit{\textbf{Members: }} \\
Xingyu Qiu$^{1}$ (\href{mailto:xyqiu24@m.fudan.edu.cn}{xyqiu24@m.fudan.edu.cn}),\\
Yuqian Fu$^{2}$ (\href{mailto:yuqian.fu.ai@gmail.com}{yuqian.fu.ai@gmail.com}),\\
Jiawei Geng$^{1}$ (\href{mailto:jwgeng25@m.fudan.edu.cn}{jwgeng25@m.fudan.edu.cn}),\\
Bin Ren$^{3}$ (\href{mailto:bin.ren.mondo@gmail.com}{bin.ren.mondo@gmail.com}),\\
Jiancheng Pan$^{4}$ (\href{mailto:jiancheng.pan.plus@gmail.com}{jiancheng.pan.plus@gmail.com}),\\
Zongwei Wu$^{5}$ (\href{mailto:zongwei.wu@uni-wuerzburg.de}{zongwei.wu@uni-wuerzburg.de}),\\
Hao Tang$^{6}$ (\href{mailto:howard.haotang@gmail.com}{howard.haotang@gmail.com}),\\
Yanwei Fu$^{1}$ (\href{mailto:yanweifu@fudan.edu.cn}{yanweifu@fudan.edu.cn}),\\
Radu Timofte$^{5}$ (\href{mailto:radu.timofte@uni-wuerzburg.de}{radu.timofte@uni-wuerzburg.de}),\\
Nicu Sebe$^{7}$ (\href{mailto:niculae.sebe@unitn.it}{niculae.sebe@unitn.it}),\\
Mohamed Elhoseiny$^{2}$
(\href{mailto:mohamed.elhoseiny@kaust.edu.sa}{mohamed.elhoseiny@kaust.edu.sa})

\noindent\textit{\textbf{Affiliations: }}\\
$^1$ Fudan University, China\\
$^2$ KAUST, Saudi Arabia\\
$^3$ MBZUAI, United Arab Emirates\\
$^4$ Tsinghua University, China\\
$^5$ University of W\"urzburg, Germany\\
$^6$ The Hong Kong Polytechnic University, China\\
$^7$ University of Trento, Italy\\

==> ntire26/main <==
\begin{thebibliography}{133}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Ancuti et~al.(2026{\natexlab{a}})Ancuti, Ancuti, Timofte, and Ancuti]{ntire26nthaze}
Radu Ancuti, Codruta Ancuti, Radu Timofte, and Cosmin Ancuti.
\newblock { NT-HAZE: A Benchmark Dataset for Realistic Night-time Image Dehazing }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Ancuti et~al.(2026{\natexlab{b}})Ancuti, Brateanu, Vasluianu, Balmez, Orhei, Ancuti, Timofte, Ancuti, et~al.]{ntire26nthaze_rep}
Radu Ancuti, Alexandru Brateanu, Florin Vasluianu, Raul Balmez, Ciprian Orhei, Codruta Ancuti, Radu Timofte, Cosmin Ancuti, et~al.
\newblock { NTIRE 2026 Nighttime Image Dehazing Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Bai et~al.(2025{\natexlab{a}})Bai, Cai, Chen, Chen, Chen, Cheng, Deng, Ding, Gao, Ge, Ge, Guo, Huang, Huang, Huang, Hui, Jiang, Li, Li, Li, Li, Lin, Lin, Liu, Liu, Liu, Liu, Liu, Liu, Lu, Luo, Lv, Men, Meng, Ren, Ren, Song, Sun, Tang, Tu, Wan, Wang, Wang, Wang, Wang, Xie, Xu, Xu, Xu, Yang, Yang, Yang, Yang, Yu, Zhang, Zhang, Zhang, Zheng, Zhong, Zhou, Zhou, Zhou, Zhu, and Zhu]{qwen3vl}
Shuai Bai, Yuxuan Cai, Ruizhe Chen, Keqin Chen, Xionghui Chen, Zesen Cheng, Lianghao Deng, Wei Ding, Chang Gao, Chunjiang Ge, Wenbin Ge, Zhifang Guo, Qidong Huang, Jie Huang, Fei Huang, Binyuan Hui, Shutong Jiang, Zhaohai Li, Mingsheng Li, Mei Li, Kaixin Li, Zicheng Lin, Junyang Lin, Xuejing Liu, Jiawei Liu, Chenglong Liu, Yang Liu, Dayiheng Liu, Shixuan Liu, Dunjie Lu, Ruilin Luo, Chenxu Lv, Rui Men, Lingchen Meng, Xuancheng Ren, Xingzhang Ren, Sibo Song, Yuchong Sun, Jun Tang, Jianhong Tu, Jianqiang Wan, Peng Wang, Pengfei Wang, Qiuyue Wang, Yuxuan Wang, Tianbao Xie, Yiheng Xu, Haiyang Xu, Jin Xu, Zhibo Yang, Mingkun Yang, Jianxin Yang, An Yang, Bowen Yu, Fei Zhang, Hang Zhang, Xi Zhang, Bo Zheng, Humen Zhong, Jingren Zhou, Fan Zhou, Jing Zhou, Yuanzhi Zhu, and Ke Zhu.
\newblock Qwen3-vl technical report.
\newblock \emph{arXiv preprint arXiv:2511.21631}, 2025{\natexlab{a}}.

\bibitem[Bai et~al.(2025{\natexlab{b}})Bai, Cai, Chen, Chen, Chen, Cheng, Deng, Ding, Gao, Ge, et~al.]{bai2025qwen3}
Shuai Bai, Yuxuan Cai, Ruizhe Chen, Keqin Chen, Xionghui Chen, Zesen Cheng, Lianghao Deng, Wei Ding, Chang Gao, Chunjiang Ge, et~al.
\newblock Qwen3-vl technical report.
\newblock \emph{arXiv preprint arXiv:2511.21631}, 2025{\natexlab{b}}.

\bibitem[Bochkovskiy et~al.(2020)Bochkovskiy, Wang, and Liao]{bochkovskiy2020yolov4}
Alexey Bochkovskiy, Chien-Yao Wang, and Hong-Yuan~Mark Liao.
\newblock Yolov4: Optimal speed and accuracy of object detection.
\newblock \emph{arXiv preprint arXiv:2004.10934}, 2020.

\bibitem[Cai et~al.(2026)Cai, Yang, Li, Vasluianu, Timofte, et~al.]{ntire26reflection}
Jie Cai, Kangning Yang, Zhiyuan Li, Florin Vasluianu, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Single Image Reflection Removal in the Wild: Datasets, Results, and Methods }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Carion et~al.(2020)Carion, Massa, Synnaeve, Usunier, Kirillov, and Zagoruyko]{carion2020end}
Nicolas Carion, Francisco Massa, Gabriel Synnaeve, Nicolas Usunier, Alexander Kirillov, and Sergey Zagoruyko.
\newblock End-to-end object detection with transformers.
\newblock In \emph{ECCV}, 2020.

\bibitem[Carion et~al.(2025{\natexlab{a}})Carion, Gustafson, Hu, Debnath, Hu, Suris, Ryali, Alwala, Khedr, Huang, Lei, Ma, Guo, Kalla, Marks, Greer, Wang, Sun, Rädle, Afouras, Mavroudi, Xu, Wu, Zhou, Momeni, Hazra, Ding, Vaze, Porcher, Li, Li, Kamath, Cheng, Dollár, Ravi, Saenko, Zhang, and Feichtenhofer]{sam3}
Nicolas Carion, Laura Gustafson, Yuan-Ting Hu, Shoubhik Debnath, Ronghang Hu, Didac Suris, Chaitanya Ryali, Kalyan~Vasudev Alwala, Haitham Khedr, Andrew Huang, Jie Lei, Tengyu Ma, Baishan Guo, Arpit Kalla, Markus Marks, Joseph Greer, Meng Wang, Peize Sun, Roman Rädle, Triantafyllos Afouras, Effrosyni Mavroudi, Katherine Xu, Tsung-Han Wu, Yu Zhou, Liliane Momeni, Rishi Hazra, Shuangrui Ding, Sagar Vaze, Francois Porcher, Feng Li, Siyuan Li, Aishwarya Kamath, Ho~Kei Cheng, Piotr Dollár, Nikhila Ravi, Kate Saenko, Pengchuan Zhang, and Christoph Feichtenhofer.
\newblock Sam 3: Segment anything with concepts, 2025{\natexlab{a}}.

\bibitem[Carion et~al.(2025{\natexlab{b}})Carion, Gustafson, Hu, Debnath, Hu, Suris, Ryali, Alwala, Khedr, Huang, et~al.]{carion2025sam}
Nicolas Carion, Laura Gustafson, Yuan-Ting Hu, Shoubhik Debnath, Ronghang Hu, Didac Suris, Chaitanya Ryali, Kalyan~Vasudev Alwala, Haitham Khedr, Andrew Huang, et~al.
\newblock Sam 3: Segment anything with concepts.
\newblock \emph{arXiv preprint arXiv:2511.16719}, 2025{\natexlab{b}}.

\bibitem[Carion et~al.(2026)Carion, Gustafson, Hu, Debnath, Hu, Coll-Vinent, Ryali, Alwala, Khedr, Huang, Lei, Ma, Guo, Kalla, Marks, Greer, Wang, Sun, R{\"a}dle, Afouras, Mavroudi, Xu, Wu, Zhou, Momeni, HAZRA, Ding, Vaze, Porcher, Li, Li, Kamath, Cheng, Dollar, Ravi, Saenko, Zhang, and Feichtenhofer]{carion2026sam}
Nicolas Carion, Laura Gustafson, Yuan-Ting Hu, Shoubhik Debnath, Ronghang Hu, Didac~Suris Coll-Vinent, Chaitanya Ryali, Kalyan~Vasudev Alwala, Haitham Khedr, Andrew Huang, Jie Lei, Tengyu Ma, Baishan Guo, Arpit Kalla, Markus Marks, Joseph Greer, Meng Wang, Peize Sun, Roman R{\"a}dle, Triantafyllos Afouras, Effrosyni Mavroudi, Katherine Xu, Tsung-Han Wu, Yu Zhou, Liliane Momeni, RISHI HAZRA, Shuangrui Ding, Sagar Vaze, Francois Porcher, Feng Li, Siyuan Li, Aishwarya Kamath, Ho~Kei Cheng, Piotr Dollar, Nikhila Ravi, Kate Saenko, Pengchuan Zhang, and Christoph Feichtenhofer.
\newblock {SAM} 3: Segment anything with concepts.
\newblock In \emph{The Fourteenth International Conference on Learning Representations}, 2026.

\bibitem[Chen et~al.(2019)Chen, Wang, Pang, Cao, Xiong, Li, Sun, Feng, Liu, Xu, Zhang, Cheng, Zhu, Cheng, Zhao, Li, Lu, Zhu, Wu, Dai, Wang, Shi, Ouyang, Loy, and Lin]{mmdetection}
Kai Chen, Jiaqi Wang, Jiangmiao Pang, Yuhang Cao, Yu Xiong, Xiaoxiao Li, Shuyang Sun, Wansen Feng, Ziwei Liu, Jiarui Xu, Zheng Zhang, Dazhi Cheng, Chenchen Zhu, Tianheng Cheng, Qijie Zhao, Buyu Li, Xin Lu, Rui Zhu, Yue Wu, Jifeng Dai, Jingdong Wang, Jianping Shi, Wanli Ouyang, Chen~Change Loy, and Dahua Lin.
\newblock {MMDetection}: Open mmlab detection toolbox and benchmark.
\newblock \emph{arXiv preprint arXiv:1906.07155}, 2019.

\bibitem[Chen et~al.(2026)Chen, Liu, Wang, Yan, Li, Zhang, Gong, Li, Sun, Liu, Timofte, Zhang, et~al.]{ntire26srx4}
Zheng Chen, Kai Liu, Jingkai Wang, Xianglong Yan, Jianze Li, Ziqing Zhang, Jue Gong, Jiatong Li, Lei Sun, Xiaoyang Liu, Radu Timofte, Yulun Zhang, et~al.
\newblock { The Fourth Challenge on Image Super-Resolution (×4) at NTIRE 2026: Benchmark Results and Method Overview }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[{Chenping Fu, Risheng Liu, Xin Fan, Puyang Chen, Hao Fu, Wanqi Yuan, Ming Zhu, Zhongxuan Luo}()]{RUOD23}
{Chenping Fu, Risheng Liu, Xin Fan, Puyang Chen, Hao Fu, Wanqi Yuan, Ming Zhu, Zhongxuan Luo}.
\newblock {Rethinking general underwater object detection: Datasets, challenges, and solutions}.
\newblock \emph{{Neurocomputing}}.

\bibitem[Choi et~al.(2025)Choi, Go, and Jang]{spbaizero}
Sangbum Choi, Kyeongryeol Go, and Taewoong Jang.
\newblock Zero: Industry-ready vision foundation model with multi-modal prompts, 2025.

\bibitem[Ciubotariu et~al.(2026{\natexlab{a}})Ciubotariu, S~M~A, Rehman, Ali, Naqvi, Conde, Timofte, et~al.]{ntire26llie}
George Ciubotariu, Sharif S~M~A, Abdur Rehman, Fayaz Ali, Rizwan~Ali Naqvi, Marcos Conde, Radu Timofte, et~al.
\newblock { Low Light Image Enhancement Challenge at NTIRE 2026 }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Ciubotariu et~al.(2026{\natexlab{b}})Ciubotariu, Zhou, Jin, Wu, Timofte, et~al.]{ntire26highfps}
George Ciubotariu, Zhuyun Zhou, Yeying Jin, Zongwei Wu, Radu Timofte, et~al.
\newblock { High FPS Video Frame Interpolation Challenge at NTIRE 2026 }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Devlin et~al.(2019)Devlin, Chang, Lee, and Toutanova]{devlin2019bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language understanding.
\newblock In \emph{Proceedings of the 2019 conference of the North American chapter of the association for computational linguistics: human language technologies, volume 1 (long and short papers)}, 2019.

\bibitem[Drange(2019)]{GeirArTaxOr}
Geir Drange.
\newblock Arthropod taxonomy orders object detection dataset.
\newblock In \emph{https://doi.org/10.34740/kaggle/dsv/1240192}, 2019.

\bibitem[Dumitriu et~al.(2026)Dumitriu, Ralhan, Miron, Tatui, Ionescu, Timofte, et~al.]{ntire26ripdetseg}
Andrei Dumitriu, Aakash Ralhan, Florin Miron, Florin Tatui, Radu~Tudor Ionescu, Radu Timofte, et~al.
\newblock { NTIRE 2026 Rip Current Detection and Segmentation (RipDetSeg) Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Elezabi et~al.(2026)Elezabi, V.~Conde, Wu, Jin, Timofte, et~al.]{ntire26retouching}
Omar Elezabi, Marcos V.~Conde, Zongwei Wu, Yeying Jin, Radu Timofte, et~al.
\newblock { Photography Retouching Transfer, NTIRE 2026 Challenge: Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Feng et~al.(2026{\natexlab{a}})Feng, Sha, Liu, Yu, Vong, Yu, and Shen]{feng2025fsodvfm}
Chen-Bin Feng, Youyang Sha, Longfei Liu, Yongjun Yu, Chi~Man Vong, Xuanlong Yu, and Xi Shen.
\newblock Few-shot object detection with vision foundation models and graph diffusion.
\newblock In \emph{The Fourteenth International Conference on Learning Representations}, 2026{\natexlab{a}}.

\bibitem[Feng et~al.(2026{\natexlab{b}})Feng, Sha, Liu, Yu, Vong, Yu, and Shen]{feng2026fsodvfm}
Chen-Bin Feng, Youyang Sha, Longfei Liu, Yongjun Yu, Chi~Man Vong, Xuanlong Yu, and Xi Shen.
\newblock {FSOD-VFM}: Few-shot object detection with vision foundation models and graph diffusion.
\newblock In \emph{ICLR}, 2026{\natexlab{b}}.

\bibitem[Fu et~al.(2025{\natexlab{a}})Fu, Su, Rao, Lyu, Xie, and Zheng]{fu2025wedetect}
Shenghao Fu, Yukun Su, Fengyun Rao, Jing Lyu, Xiaohua Xie, and Wei-Shi Zheng.
\newblock Wedetect: Fast open-vocabulary object detection as retrieval.
\newblock \emph{arXiv preprint arXiv:2512.12309}, 2025{\natexlab{a}}.

\bibitem[Fu et~al.(2021)Fu, Fu, and Jiang]{fu2021meta}
Yuqian Fu, Yanwei Fu, and Yu-Gang Jiang.
\newblock Meta-fdmixup: Cross-domain few-shot learning guided by labeled target data.
\newblock In \emph{ACM multimedia}, 2021.

\bibitem[Fu et~al.(2022)Fu, Xie, Fu, Chen, and Jiang]{fu2022me}
Yuqian Fu, Yu Xie, Yanwei Fu, Jingjing Chen, and Yu-Gang Jiang.
\newblock Me-d2n: Multi-expert domain decompositional network for cross-domain few-shot learning.
\newblock In \emph{ACM multimedia}, 2022.

\bibitem[Fu et~al.(2023)Fu, Xie, Fu, and Jiang]{fu2023styleadv}
Yuqian Fu, Yu Xie, Yanwei Fu, and Yu-Gang Jiang.
\newblock Styleadv: Meta style adversarial training for cross-domain few-shot learning.
\newblock In \emph{CVPR}, 2023.

\bibitem[Fu et~al.(2024)Fu, Wang, Pan, Huai, Qiu, Shangguan, Liu, Fu, Van~Gool, and Jiang]{fu2024cross}
Yuqian Fu, Yu Wang, Yixuan Pan, Lian Huai, Xingyu Qiu, Zeyu Shangguan, Tong Liu, Yanwei Fu, Luc Van~Gool, and Xingqun Jiang.
\newblock Cross-domain few-shot object detection via enhanced open-set object detector.
\newblock In \emph{European Conference on Computer Vision}, 2024.

\bibitem[Fu et~al.(2025{\natexlab{b}})Fu, Qiu, Ren, Fu, Timofte, Sebe, Yang, Van~Gool, Zhang, Nong, et~al.]{fu2025ntire}
Yuqian Fu, Xingyu Qiu, Bin Ren, Yanwei Fu, Radu Timofte, Nicu Sebe, Ming-Hsuan Yang, Luc Van~Gool, Kaijin Zhang, Qingpeng Nong, et~al.
\newblock Ntire 2025 challenge on cross-domain few-shot object detection: Methods and results.
\newblock In \emph{Proceedings of the Computer Vision and Pattern Recognition Conference}, 2025{\natexlab{b}}.

\bibitem[Guan et~al.(2026{\natexlab{a}})Guan, Li, Yang, Ke, Cai, Vasluianu, Timofte, et~al.]{ntire26finrec}
Bochen Guan, Jinlong Li, Kangning Yang, Chuang Ke, Jie Cai, Florin Vasluianu, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on End-to-End Financial Receipt Restoration and Reasoning from Degraded Images: Datasets, Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Guan et~al.(2026{\natexlab{b}})Guan, Zhang, Guo, Wang, Fan, Liang, Zeng, Qin, Qu, Dai, Xia, Zhang, Timofte, et~al.]{ntire26raim_portrait}
Ya-nan Guan, Shaonan Zhang, Hang Guo, Yawen Wang, Xinying Fan, Jie Liang, Hui Zeng, Guanyi Qin, Lishen Qu, Tao Dai, Shu-Tao Xia, Lei Zhang, Radu Timofte, et~al.
\newblock { NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: AI Flash Portrait (Track 3) }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Gui et~al.(2024)Gui, Song, Qin, and Tang]{gui2024remote}
Shengxi Gui, Shuang Song, Rongjun Qin, and Yang Tang.
\newblock Remote sensing object detection in the deep learning era—a review.
\newblock \emph{Remote Sensing}, 16\penalty0 (2):\penalty0 327, 2024.

\bibitem[Guo et~al.(2022)Guo, Mu, Chen, Wang, Yu, and Luo]{guo2022scale}
Qiushan Guo, Yao Mu, Jianyu Chen, Tianqi Wang, Yizhou Yu, and Ping Luo.
\newblock Scale-equivalent distillation for semi-supervised object detection.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2022.

\bibitem[Guo et~al.(2020)Guo, Codella, Karlinsky, Codella, Smith, Saenko, Rosing, and Feris]{guo2020broader}
Yunhui Guo, Noel~C Codella, Leonid Karlinsky, James~V Codella, John~R Smith, Kate Saenko, Tajana Rosing, and Rogerio Feris.
\newblock A broader study of cross-domain few-shot learning.
\newblock In \emph{ECCV}, 2020.

\bibitem[Gushchin et~al.(2026)Gushchin, Abud, Shumitskaya, Filippov, Bychkov, Lavrushkin, Erofeev, Antsiferova, Chen, Tan, Timofte, Vatolin, et~al.]{ntire26aigendet}
Aleksandr Gushchin, Khaled Abud, Ekaterina Shumitskaya, Artem Filippov, Georgii Bychkov, Sergey Lavrushkin, Mikhail Erofeev, Anastasia Antsiferova, Changsheng Chen, Shunquan Tan, Radu Timofte, Dmitriy Vatolin, et~al.
\newblock { NTIRE 2026 Challenge on Robust AI-Generated Image Detection in the Wild }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Hopf et~al.(2026)Hopf, Timofte, et~al.]{ntire26deepfake}
Benedikt Hopf, Radu Timofte, et~al.
\newblock { Robust Deepfake Detection, NTIRE 2026 Challenge: Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Hsieh et~al.(2017)Hsieh, Lin, and Hsu]{hsieh2017drone}
Meng-Ru Hsieh, Yen-Liang Lin, and Winston~H Hsu.
\newblock Drone-based object counting by spatially regularized regional proposal network.
\newblock In \emph{Proceedings of the IEEE international conference on computer vision}, 2017.

\bibitem[Hu et~al.(2022)Hu, Shen, Wallis, Allen-Zhu, Li, Wang, Wang, and Chen]{lora}
Edward~J. Hu, Yelong Shen, Phillip Wallis, Zeyuan Allen-Zhu, Yuanzhi Li, Shean Wang, Lu Wang, and Weizhu Chen.
\newblock Lora: Low-rank adaptation of large language models.
\newblock In \emph{ICLR}. OpenReview.net, 2022.

\bibitem[Inoue et~al.(2018)Inoue, Furuta, Yamasaki, and Aizawa]{inoue2018cross}
Naoto Inoue, Ryosuke Furuta, Toshihiko Yamasaki, and Kiyoharu Aizawa.
\newblock Cross-domain weakly-supervised object detection through progressive domain adaptation.
\newblock In \emph{CVPR}, 2018.

\bibitem[Jiang et~al.(2021)Jiang, Wang, Jia, Xu, Liu, Fan, Li, Liu, Xue, and Wang]{jiang2021underwater}
Lihao Jiang, Yi Wang, Qi Jia, Shengwei Xu, Yu Liu, Xin Fan, Haojie Li, Risheng Liu, Xinwei Xue, and Ruili Wang.
\newblock Underwater species detection using channel sharpening attention.
\newblock In \emph{ACM MM}, 2021.

\bibitem[Jiang et~al.(2024)Jiang, luo, Yang, Xiong, Chen, Zeng, Ren, and Zhang]{jiang2024chatrextamingmultimodalllm}
Qing Jiang, Gen luo, Yuqin Yang, Yuda Xiong, Yihao Chen, Zhaoyang Zeng, Tianhe Ren, and Lei Zhang.
\newblock Chatrex: Taming multimodal llm for joint perception and understanding, 2024.

\bibitem[Kamath et~al.(2021)Kamath, Singh, LeCun, Synnaeve, Misra, and Carion]{kamath2021mdetr}
Aishwarya Kamath, Mannat Singh, Yann LeCun, Gabriel Synnaeve, Ishan Misra, and Nicolas Carion.
\newblock Mdetr-modulated detection for end-to-end multi-modal understanding.
\newblock In \emph{ICCV}, 2021.

\bibitem[Khalin et~al.(2026)Khalin, Ershov, Panshin, Korchagin, Lobarev, Terekhin, Dorogova, Shamsutdinov, Mamedov, Khalfin, Sheludko, Zilyaev, Banić, Perevozchikov, Timofte, et~al.]{ntire26twilight}
Aleksei Khalin, Egor Ershov, Artem Panshin, Sergey Korchagin, Georgiy Lobarev, Arseniy Terekhin, Sofiia Dorogova, Amir Shamsutdinov, Yasin Mamedov, Bakhtiyar Khalfin, Bogdan Sheludko, Emil Zilyaev, Nikola Banić, Georgy Perevozchikov, Radu Timofte, et~al.
\newblock { NTIRE 2026 Low-light Enhancement: Twilight Cowboy Challenge }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[K{\"o}hler et~al.(2023)K{\"o}hler, Eisenbach, and Gross]{kohler2023few}
Mona K{\"o}hler, Markus Eisenbach, and Horst-Michael Gross.
\newblock Few-shot object detection: A comprehensive survey.
\newblock \emph{IEEE Transactions on Neural Networks and Learning Systems}, 2023.

\bibitem[Krishna et~al.(2017{\natexlab{a}})Krishna, Zhu, Groth, Johnson, Hata, Kravitz, Chen, Kalantidis, Li, Shamma, et~al.]{krishna2017visual}
Ranjay Krishna, Yuke Zhu, Oliver Groth, Justin Johnson, Kenji Hata, Joshua Kravitz, Stephanie Chen, Yannis Kalantidis, Li-Jia Li, David~A Shamma, et~al.
\newblock Visual genome: Connecting language and vision using crowdsourced dense image annotations.
\newblock \emph{International journal of computer vision}, 2017{\natexlab{a}}.

\bibitem[Krishna et~al.(2017{\natexlab{b}})]{krishna2017vg}
Ranjay Krishna et~al.
\newblock Visual genome.
\newblock In \emph{IJCV}, 2017{\natexlab{b}}.

\bibitem[Krizhevsky et~al.(2012)Krizhevsky, Sutskever, and Hinton]{krizhevsky2012imagenet}
Alex Krizhevsky, Ilya Sutskever, and Geoffrey~E Hinton.
\newblock Imagenet classification with deep convolutional neural networks.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2012.

\bibitem[Kuznetsova et~al.(2020)Kuznetsova, Rom, Alldrin, Uijlings, Krasin, Pont-Tuset, Kamali, Popov, Malloci, Kolesnikov, et~al.]{kuznetsova2020open}
Alina Kuznetsova, Hassan Rom, Neil Alldrin, Jasper Uijlings, Ivan Krasin, Jordi Pont-Tuset, Shahab Kamali, Stefan Popov, Matteo Malloci, Alexander Kolesnikov, et~al.
\newblock The open images dataset v4: Unified image classification, object detection, and visual relationship detection at scale.
\newblock \emph{International journal of computer vision}, 2020.

\bibitem[Li et~al.(2025{\natexlab{a}})Li, Wang, Zhang, Zhao, Gao, and Li]{li2025maris}
Bingyu Li, Feiyu Wang, Da Zhang, Zhiyuan Zhao, Junyu Gao, and Xuelong Li.
\newblock Maris: Marine open-vocabulary instance segmentation with geometric enhancement and semantic alignment.
\newblock \emph{arXiv preprint arXiv:2510.15398}, 2025{\natexlab{a}}.

\bibitem[Li et~al.(2022{\natexlab{a}})Li, Liu, Li, Zhang, Aneja, Yang, Jin, Hu, Liu, Lee, et~al.]{li2022elevater}
Chunyuan Li, Haotian Liu, Liunian Li, Pengchuan Zhang, Jyoti Aneja, Jianwei Yang, Ping Jin, Houdong Hu, Zicheng Liu, Yong~Jae Lee, et~al.
\newblock Elevater: A benchmark and toolkit for evaluating language-augmented visual models.
\newblock \emph{Advances in Neural Information Processing Systems}, 2022{\natexlab{a}}.

\bibitem[Li et~al.(2025{\natexlab{b}})Li, Pan, Sun, and Huang]{li2025semantic}
Jiahao Li, Jiancheng Pan, Yuze Sun, and Xiaomeng Huang.
\newblock Semantic-aware ship detection with vision-language integration.
\newblock In \emph{IGARSS 2025-2025 IEEE International Geoscience and Remote Sensing Symposium}, 2025{\natexlab{b}}.

\bibitem[Li et~al.(2026{\natexlab{a}})Li, Chen, Liu, Wang, Zhou, Liu, Zhu, Timofte, Zhang, et~al.]{ntire26rwsr}
Jiatong Li, Zheng Chen, Kai Liu, Jingkai Wang, Zihan Zhou, Xiaoyang Liu, Libo Zhu, Radu Timofte, Yulun Zhang, et~al.
\newblock { The First Challenge on Mobile Real-World Image Super-Resolution at NTIRE 2026: Benchmark Results and Method Overview }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Li et~al.(2020)Li, Wan, Cheng, Meng, and Han]{li2020object}
Ke Li, Gang Wan, Gong Cheng, Liqiu Meng, and Junwei Han.
\newblock Object detection in optical remote sensing images: A survey and a new benchmark.
\newblock \emph{ISPRS}, 2020.

\bibitem[Li et~al.(2022{\natexlab{b}})]{li2022glip}
Liunian Li et~al.
\newblock Grounded language-image pre-training.
\newblock In \emph{CVPR}, 2022{\natexlab{b}}.

\bibitem[Li et~al.(2022{\natexlab{c}})Li, Zhang, Zhang, Yang, Li, Zhong, Wang, Yuan, Zhang, Hwang, et~al.]{li2022grounded}
Liunian~Harold Li, Pengchuan Zhang, Haotian Zhang, Jianwei Yang, Chunyuan Li, Yiwu Zhong, Lijuan Wang, Lu Yuan, Lei Zhang, Jenq-Neng Hwang, et~al.
\newblock Grounded language-image pre-training.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2022{\natexlab{c}}.

\bibitem[Li et~al.(2022{\natexlab{d}})Li, Liu, and Bilen]{li2022cross}
Wei-Hong Li, Xialei Liu, and Hakan Bilen.
\newblock Cross-domain few-shot learning with task-specific adapters.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, 2022{\natexlab{d}}.

\bibitem[Li et~al.(2026{\natexlab{b}})Li, Gong, Wang, Xiong, Li, Yao, Zhou, Chen, Timofte, et~al.]{ntire26ugcvideo}
Xin Li, Jiachao Gong, Xijun Wang, Shiyao Xiong, Bingchen Li, Suhang Yao, Chao Zhou, Zhibo Chen, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Short-form UGC Video Restoration in the Wild with Generative Models: Datasets, Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Li et~al.(2026{\natexlab{c}})Li, Jin, Yao, Lin, Fan, Yan, Jin, Wu, Li, Shi, Yang, Li, Chen, Wen, Tan, Timofte, et~al.]{ntire26dual_focus}
Xin Li, Yeying Jin, Suhang Yao, Beibei Lin, Zhaoxin Fan, Wending Yan, Xin Jin, Zongwei Wu, Bingchen Li, Peishu Shi, Yufei Yang, Yu Li, Zhibo Chen, Bihan Wen, Robby Tan, Radu Timofte, et~al.
\newblock { NTIRE 2026 The Second Challenge on Day and Night Raindrop Removal for Dual-Focused Images: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{c}}.

\bibitem[Li et~al.(2025{\natexlab{c}})Li, Qiu, Fu, Chen, Qian, Zheng, Paudel, Fu, Huang, Van~Gool, et~al.]{li2025domain}
Yu Li, Xingyu Qiu, Yuqian Fu, Jie Chen, Tianwen Qian, Xu Zheng, Danda~Pani Paudel, Yanwei Fu, Xuanjing Huang, Luc Van~Gool, et~al.
\newblock Domain-rag: Retrieval-guided compositional image generation for cross-domain few-shot object detection.
\newblock \emph{arXiv preprint arXiv:2506.05872}, 2025{\natexlab{c}}.

\bibitem[Lin et~al.(2014{\natexlab{a}})Lin, Maire, Belongie, Hays, Perona, Ramanan, Doll{\'a}r, and Zitnick]{lin2014microsoft}
Tsung-Yi Lin, Michael Maire, Serge Belongie, James Hays, Pietro Perona, Deva Ramanan, Piotr Doll{\'a}r, and C~Lawrence Zitnick.
\newblock Microsoft coco: Common objects in context.
\newblock In \emph{ECCV}, 2014{\natexlab{a}}.

\bibitem[Lin et~al.(2014{\natexlab{b}})]{lin2014coco}
Tsung-Yi Lin et~al.
\newblock Microsoft coco.
\newblock In \emph{ECCV}, 2014{\natexlab{b}}.

\bibitem[Lin et~al.(2017)]{lin2017focal}
Tsung-Yi Lin et~al.
\newblock Focal loss.
\newblock In \emph{ICCV}, 2017.

\bibitem[Liu et~al.(2026{\natexlab{a}})Liu, Yue, Lin, Chen, Wang, Gong, Timofte, Zhang, et~al.]{ntire26rsirsr}
Kai Liu, Haoyang Yue, Zeli Lin, Zheng Chen, Jingkai Wang, Jue Gong, Radu Timofte, Yulun Zhang, et~al.
\newblock { The First Challenge on Remote Sensing Infrared Image Super-Resolution at NTIRE 2026: Benchmark Results and Method Overview }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Liu et~al.(2023)Liu, Zeng, Ren, Li, Zhang, Yang, Li, Yang, Su, Zhu, et~al.]{groundingdino}
Shilong Liu, Zhaoyang Zeng, Tianhe Ren, Feng Li, Hao Zhang, Jie Yang, Chunyuan Li, Jianwei Yang, Hang Su, Jun Zhu, et~al.
\newblock Grounding dino: Marrying dino with grounded pre-training for open-set object detection.
\newblock \emph{arXiv preprint arXiv:2303.05499}, 2023.

\bibitem[Liu et~al.(2024)Liu, Zeng, Ren, Li, Zhang, Yang, Jiang, Li, Yang, Su, et~al.]{liu2024grounding}
Shilong Liu, Zhaoyang Zeng, Tianhe Ren, Feng Li, Hao Zhang, Jie Yang, Qing Jiang, Chunyuan Li, Jianwei Yang, Hang Su, et~al.
\newblock Grounding dino: Marrying dino with grounded pre-training for open-set object detection.
\newblock In \emph{European Conference on Computer Vision}, 2024.

\bibitem[Liu et~al.(2026{\natexlab{b}})Liu, Cui, Bao, Chu, Gu, Ren, Timofte, Conde, et~al.]{ntire26realx3d}
Shuhong Liu, Ziteng Cui, Chenyu Bao, Xuangeng Chu, Lin Gu, Bin Ren, Radu Timofte, Marcos~V. Conde, et~al.
\newblock { 3D Restoration and Reconstruction in Adverse Conditions: RealX3D Challenge Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Liu et~al.(2026{\natexlab{c}})Liu, Min, Zhai, Hu, Cao, Zhou, Sun, Wen, Xu, Zhou, Duan, Liu, Wang, Luo, Li, Xu, Zhang, Shi, Wang, Zhang, Guo, Hu, Chen, Wu, Ma, Lv, Xue, Wang, Sha, Timofte, et~al.]{ntire26XAIGCqa}
Xiaohong Liu, Xiongkuo Min, Guangtao Zhai, Qiang Hu, Jiezhang Cao, Yu Zhou, Wei Sun, Farong Wen, Zitong Xu, Yingjie Zhou, Huiyu Duan, Lu Liu, Jiarui Wang, Siqi Luo, Chunyi Li, Li Xu, Zicheng Zhang, Yue Shi, Yubo Wang, Minghong Zhang, Chunchao Guo, Zhichao Hu, Mingtao Chen, Xiele Wu, Xin Ma, Zhaohe Lv, Yuanhao Xue, Jiaqi Wang, Xinxing Sha, Radu Timofte, et~al.
\newblock { NTIRE 2026 X-AIGC Quality Assessment Challenge: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{c}}.

\bibitem[Liu et~al.(2025)Liu, Pan, Yang, Chen, Zhou, and Zhang]{liu2025diverse}
Yanxing Liu, Jiancheng Pan, Jianwei Yang, Tiancheng Chen, Peiling Zhou, and Bingchen Zhang.
\newblock Diverse instance generation via diffusion models for enhanced few-shot object detection in remote sensing images.
\newblock \emph{IEEE Geoscience and Remote Sensing Letters}, 2025.

\bibitem[Liu et~al.(2021)Liu, Lin, Cao, Hu, Wei, Zhang, Lin, and Guo]{liu2021swin}
Ze Liu, Yutong Lin, Yue Cao, Han Hu, Yixuan Wei, Zheng Zhang, Stephen Lin, and Baining Guo.
\newblock Swin transformer: Hierarchical vision transformer using shifted windows.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, 2021.

\bibitem[Meng et~al.(2025)Meng, Zhang, Li, Wu, Li, Zhao, Yu, and Shen]{meng2025cdformer}
Boyuan Meng, Xiaohan Zhang, Peilin Li, Zhe Wu, Yiming Li, Wenkai Zhao, Beinan Yu, and Hui-Liang Shen.
\newblock Cdformer: Cross-domain few-shot object detection transformer against feature confusion.
\newblock In \emph{ICME}, 2025.

\bibitem[Moskalenko et~al.(2026)Moskalenko, Bryncev, Kosmynin, Shilovskaya, Erofeev, Vatolin, Timofte, et~al.]{ntire26videosal}
Andrey Moskalenko, Alexey Bryncev, Ivan Kosmynin, Kira Shilovskaya, Mikhail Erofeev, Dmitry Vatolin, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Video Saliency Prediction: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Oquab et~al.(2024)Oquab, Darcet, Moutakanni, Vo, Szafraniec, Khalidov, Fernandez, Haziza, Massa, El-Nouby, et~al.]{oquab2024dinov2}
Maxime Oquab, Timoth{\'e}e Darcet, Th{\'e}o Moutakanni, Huy~V. Vo, Marc Szafraniec, Vasil Khalidov, Pierre Fernandez, Daniel Haziza, Francisco Massa, Alaaeldin El-Nouby, et~al.
\newblock {DINOv2}: Learning robust visual features without supervision.
\newblock \emph{Transactions on Machine Learning Research}, 2024.

\bibitem[Ordonez et~al.(2011)Ordonez, Kulkarni, and Berg]{ordonez2011im2text}
Vicente Ordonez, Girish Kulkarni, and Tamara Berg.
\newblock Im2text: Describing images using 1 million captioned photographs.
\newblock \emph{Advances in neural information processing systems}, 24, 2011.

\bibitem[Pan et~al.(2025{\natexlab{a}})Pan, Liu, Fu, Ma, Li, Paudel, Van~Gool, and Huang]{pan2025locate}
Jiancheng Pan, Yanxing Liu, Yuqian Fu, Muyuan Ma, Jiahao Li, Danda~Pani Paudel, Luc Van~Gool, and Xiaomeng Huang.
\newblock Locate anything on earth: Advancing open-vocabulary object detection for remote sensing community.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, 2025{\natexlab{a}}.

\bibitem[Pan et~al.(2025{\natexlab{b}})Pan, Liu, He, Peng, Li, Sun, and Huang]{pan2025enhance}
Jiancheng Pan, Yanxing Liu, Xiao He, Long Peng, Jiahao Li, Yuze Sun, and Xiaomeng Huang.
\newblock Enhance then search: An augmentation-search strategy with foundation models for cross-domain few-shot object detection.
\newblock In \emph{Proceedings of the Computer Vision and Pattern Recognition Conference}, 2025{\natexlab{b}}.

\bibitem[Park et~al.(2026)Park, Park, Lee, Timofte, et~al.]{ntire26bursthdr}
Hyunhee Park, Eunpil Park, Sangmin Lee, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Efficient Burst HDR and Restoration: Datasets, Methods, and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Perevozchikov et~al.(2026)Perevozchikov, Vladimirov, Timofte, et~al.]{ntire26isp}
Georgy Perevozchikov, Daniil Vladimirov, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Learned Smartphone ISP with Unpaired Data: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Qiao et~al.(2021)Qiao, Zhao, Li, Qiu, Wu, and Zhang]{qiao2021defrcn}
Limeng Qiao, Yuxuan Zhao, Zhiyuan Li, Xi Qiu, Jianan Wu, and Chi Zhang.
\newblock Defrcn: Decoupled faster r-cnn for few-shot object detection.
\newblock In \emph{ICCV}, 2021.

\bibitem[Qin et~al.(2026)Qin, Liang, Zhang, Qu, Guan, Zeng, Zhang, Timofte, et~al.]{ntire26raim_piqa}
Guanyi Qin, Jie Liang, Bingbing Zhang, Lishen Qu, Ya-nan Guan, Hui Zeng, Lei Zhang, Radu Timofte, et~al.
\newblock { NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: Professional Image Quality Assessment (Track 1) }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Qiu et~al.(2026)Qiu, Fu, Geng, Ren, Pan, Wu, Tang, Fu, Timofte, Sebe, Elhoseiny, et~al.]{ntire26cdfsod}
Xingyu Qiu, Yuqian Fu, Jiawei Geng, Bin Ren, Jiancheng Pan, Zongwei Wu, Hao Tang, Yanwei Fu, Radu Timofte, Nicu Sebe, Mohamed Elhoseiny, et~al.
\newblock { The Second Challenge on Cross-Domain Few-Shot Object Detection at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Qu et~al.(2026)Qu, Liu, Liang, Zeng, Dai, Guan, Qin, Zhou, Yang, Zhang, Timofte, et~al.]{ntire26raim_fusion}
Lishen Qu, Yao Liu, Jie Liang, Hui Zeng, Wen Dai, Ya-nan Guan, Guanyi Qin, Shihao Zhou, Jufeng Yang, Lei Zhang, Radu Timofte, et~al.
\newblock { NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: Multi-Exposure Image Fusion in Dynamic Scenes (Track2) }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[{Qwen Team}(2026)]{qwen3.5}
{Qwen Team}.
\newblock {Qwen3.5}: Towards native multimodal agents, 2026.

\bibitem[Radford et~al.(2021)Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin, Clark, Krueger, and Sutskever]{clip}
Alec Radford, Jong~Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, Gretchen Krueger, and Ilya Sutskever.
\newblock Learning transferable visual models from natural language supervision.
\newblock In \emph{ICML}, 2021.

\bibitem[Ravi et~al.(2024)Ravi, Gabeur, Hu, Hu, Ryali, Ma, Khedr, R{\"a}dle, Rolland, Gustafson, et~al.]{ravi2024sam2}
Nikhila Ravi, Valentin Gabeur, Yuan-Ting Hu, Ronghang Hu, Chaitanya Ryali, Tengyu Ma, Haitham Khedr, Roman R{\"a}dle, Chloe Rolland, Laura Gustafson, et~al.
\newblock {SAM} 2: Segment anything in images and videos.
\newblock \emph{arXiv preprint arXiv:2408.00714}, 2024.

\bibitem[Ren et~al.(2024)Ren, Li, Liang, Ranjan, Liu, Cucchiara, Gool, Yang, and Sebe]{ren2024sharing}
Bin Ren, Yawei Li, Jingyun Liang, Rakesh Ranjan, Mengyuan Liu, Rita Cucchiara, Luc~V Gool, Ming-Hsuan Yang, and Nicu Sebe.
\newblock Sharing key semantics in transformer makes efficient image restoration.
\newblock \emph{Advances in Neural Information Processing Systems}, 37:\penalty0 7427--7463, 2024.

\bibitem[Ren et~al.(2026)Ren, Guo, Shu, Ma, Cui, Liu, Mei, Sun, Wu, Khan, Khan, Timofte, Li, et~al.]{ntire26effsr}
Bin Ren, Hang Guo, Yan Shu, Jiaqi Ma, Ziteng Cui, Shuhong Liu, Guofeng Mei, Lei Sun, Zongwei Wu, Fahad~Shahbaz Khan, Salman Khan, Radu Timofte, Yawei Li, et~al.
\newblock { The Eleventh NTIRE 2026 Efficient Super-Resolution Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Ren et~al.(2015)Ren, He, Girshick, and Sun]{ren2015faster}
Shaoqing Ren, Kaiming He, Ross Girshick, and Jian Sun.
\newblock Faster {R-CNN}: Towards real-time object detection with region proposal networks.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2015.

\bibitem[Ren et~al.(2016)Ren, He, Girshick, and Sun]{fasterrcnn}
Shaoqing Ren, Kaiming He, Ross Girshick, and Jian Sun.
\newblock Faster r-cnn: Towards real-time object detection with region proposal networks.
\newblock \emph{IEEE transactions on pattern analysis and machine intelligence}, 2016.

\bibitem[Rezatofighi et~al.(2019)]{rezatofighi2019giou}
Hamid Rezatofighi et~al.
\newblock Generalized intersection over union.
\newblock In \emph{CVPR}, 2019.

\bibitem[Saleh et~al.(2020)Saleh, Laradji, Konovalov, Bradley, Vazquez, and Sheaves]{saleh2020realistic}
Alzayat Saleh, Issam~H Laradji, Dmitry~A Konovalov, Michael Bradley, David Vazquez, and Marcus Sheaves.
\newblock A realistic fish-habitat dataset to evaluate algorithms for underwater visual analysis.
\newblock \emph{Scientific Reports}, 2020.

\bibitem[Seizinger et~al.(2026)Seizinger, Vasluianu, Conde, Chen, Zhou, Wu, Timofte, et~al.]{ntire26bokeh}
Tim Seizinger, Florin-Alexandru Vasluianu, Marcos~V. Conde, Jeffrey Chen, Zhuyun Zhou, Zongwei Wu, Radu Timofte, et~al.
\newblock { The First Controllable Bokeh Rendering Challenge at NTIRE 2026 }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Shangguan and Rostami(2023)]{shangguan2023identification}
Zeyu Shangguan and Mohammad Rostami.
\newblock Identification of novel classes for improving few-shot object detection.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, 2023.

\bibitem[Shangguan and Rostami(2024)]{shangguan2024improved}
Zeyu Shangguan and Mohammad Rostami.
\newblock Improved region proposal network for enhanced few-shot object detection.
\newblock \emph{Neural Networks}, 180:\penalty0 106699, 2024.

\bibitem[Shao et~al.(2019{\natexlab{a}})Shao, Li, Zhang, Peng, Yu, Zhang, Li, and Sun]{object365}
Shuai Shao, Zeming Li, Tianyuan Zhang, Chao Peng, Gang Yu, Xiangyu Zhang, Jing Li, and Jian Sun.
\newblock Objects365: A large-scale, high-quality dataset for object detection.
\newblock In \emph{ICCV}, 2019{\natexlab{a}}.

\bibitem[Shao et~al.(2019{\natexlab{b}})Shao, Li, Zhang, Peng, Yu, Zhang, Li, and Sun]{shao2019objects365}
Shuai Shao, Zeming Li, Tianyuan Zhang, Chao Peng, Gang Yu, Xiangyu Zhang, Jing Li, and Jian Sun.
\newblock Objects365: A large-scale, high-quality dataset for object detection.
\newblock In \emph{ICCV}, 2019{\natexlab{b}}.

\bibitem[Sim{\'e}oni et~al.(2025)Sim{\'e}oni, Vo, Seitzer, Baldassarre, Oquab, Jose, Khalidov, Szafraniec, Yi, Ramamonjisoa, et~al.]{simeoni2025dinov3}
Oriane Sim{\'e}oni, Huy~V Vo, Maximilian Seitzer, Federico Baldassarre, Maxime Oquab, Cijo Jose, Vasil Khalidov, Marc Szafraniec, Seungeun Yi, Micha{\"e}l Ramamonjisoa, et~al.
\newblock Dinov3.
\newblock \emph{arXiv preprint arXiv:2508.10104}, 2025.

\bibitem[Solovyev et~al.(2021)Solovyev, Wang, and Gabruseva]{solovyev2021weighted}
Roman Solovyev, Weimin Wang, and Tatiana Gabruseva.
\newblock Weighted boxes fusion: Ensembling boxes from different object detection models.
\newblock \emph{Image and Vision Computing}, 2021.

\bibitem[Song and Yan(2013)]{song2013noise}
Kechen Song and Yunhui Yan.
\newblock A noise robust method based on completed local binary patterns for hot-rolled steel strip surface defects.
\newblock \emph{Applied Surface Science}, 2013.

\bibitem[Sun et~al.(2021)Sun, Li, Cai, Yuan, and Zhang]{sun2021fsce}
Bo Sun, Banghuai Li, Shengcai Cai, Ye Yuan, and Chi Zhang.
\newblock Fsce: Few-shot object detection via contrastive proposal encoding.
\newblock In \emph{CVPR}, 2021.

\bibitem[Sun et~al.(2026{\natexlab{a}})Sun, Guo, Ren, Su, Wang, Pani~Paudel, Van~Gool, Timofte, Li, et~al.]{ntire26denoising}
Lei Sun, Hang Guo, Bin Ren, Shaolin Su, Xian Wang, Danda Pani~Paudel, Luc Van~Gool, Radu Timofte, Yawei Li, et~al.
\newblock { The Third Challenge on Image Denoising at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Sun et~al.(2026{\natexlab{b}})Sun, Li, Wang, Li, Shi, Xu, Zhang, Hu, Guo, Su, Timofte, Pani~Paudel, Van~Gool, et~al.]{ntire26eventblurr}
Lei Sun, Weilun Li, Xian Wang, Zhendong Li, Letian Shi, Dannong Xu, Deheng Zhang, Mengshun Hu, Shuang Guo, Shaolin Su, Radu Timofte, Danda Pani~Paudel, Luc Van~Gool, et~al.
\newblock { The Second Challenge on Event-Based Image Deblurring at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Sun et~al.(2026{\natexlab{c}})Sun, Qian, Jiang, Wang, Gao, Yang, Wang, Timofte, Pani~Paudel, Van~Gool, et~al.]{ntire26aberration}
Lei Sun, Xiaolong Qian, Qi Jiang, Xian Wang, Yao Gao, Kailun Yang, Kaiwei Wang, Radu Timofte, Danda Pani~Paudel, Luc Van~Gool, et~al.
\newblock { NTIRE 2026 The First Challenge on Blind Computational Aberration Correction: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{c}}.

\bibitem[Tang et~al.(2022)Tang, Yuan, Li, and Tang]{tang2022learning}
Hao Tang, Chengcheng Yuan, Zechao Li, and Jinhui Tang.
\newblock Learning attention-guided pyramidal features for few-shot fine-grained recognition.
\newblock \emph{Pattern Recognition}, 130:\penalty0 108792, 2022.

\bibitem[Team(2024)]{diffsynth2024}
DiffSynth Team.
\newblock Diffsynth studio: Enjoy the magic of diffusion models!
\newblock \emph{GitHub Repository}, 2024.
\newblock \url{https://github.com/modelscope/DiffSynth-Studio}.

\bibitem[Tschannen et~al.(2023)Tschannen, Kumar, Steiner, Zhai, Houlsby, and Beyer]{cappa}
Michael Tschannen, Manoj Kumar, Andreas Steiner, Xiaohua Zhai, Neil Houlsby, and Lucas Beyer.
\newblock Image captioners are scalable vision learners too.
\newblock In \emph{Proceedings of the 37th International Conference on Neural Information Processing Systems}, 2023.

\bibitem[Tseng et~al.(2020)Tseng, Lee, Huang, and Yang]{tseng2020cross}
Hung-Yu Tseng, Hsin-Ying Lee, Jia-Bin Huang, and Ming-Hsuan Yang.
\newblock Cross-domain few-shot classification via learned feature-wise transformation.
\newblock \emph{arXiv preprint arXiv:2001.08735}, 2020.

\bibitem[Vasluianu et~al.(2026{\natexlab{a}})Vasluianu, Seizinger, Chen, Zhou, Wu, Timofte, et~al.]{ntire26lightnorm}
Florin-Alexandru Vasluianu, Tim Seizinger, Jeffrey Chen, Zhuyun Zhou, Zongwei Wu, Radu Timofte, et~al.
\newblock { Learning-Based Ambient Lighting Normalization: NTIRE 2026 Challenge Results and Findings }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Vasluianu et~al.(2026{\natexlab{b}})Vasluianu, Seizinger, Zhou, Wu, Timofte, et~al.]{ntire26shadow}
Florin-Alexandru Vasluianu, Tim Seizinger, Zhuyun Zhou, Zongwei Wu, Radu Timofte, et~al.
\newblock { Advances in Single-Image Shadow Removal: Results from the NTIRE 2026 Challenge }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Wang et~al.(2025)Wang, Liu, Chen, Lin, Han, and Ding]{yoloe}
Ao Wang, Lihao Liu, Hui Chen, Zijia Lin, Jungong Han, and Guiguang Ding.
\newblock Yoloe: Real-time seeing anything, 2025.

\bibitem[Wang et~al.(2026{\natexlab{a}})Wang, Gong, Chen, Liu, Li, Zhang, Timofte, et~al.]{ntire26faceres}
Jingkai Wang, Jue Gong, Zheng Chen, Kai Liu, Jiatong Li, Yulun Zhang, Radu Timofte, et~al.
\newblock { The Second Challenge on Real-World Face Restoration at NTIRE 2026: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{a}}.

\bibitem[Wang et~al.(2026{\natexlab{b}})Wang, Guo, Wang, Li, Peng, Zhang, Timofte, Chen, Wang, Hu, Lei, et~al.]{ntire263dsr}
Longguang Wang, Yulan Guo, Yingqian Wang, Juncheng Li, Sida Peng, Ye Zhang, Radu Timofte, Minglin Chen, Yi Wang, Qibin Hu, Wenjie Lei, et~al.
\newblock { NTIRE 2026 Challenge on 3D Content Super-Resolution: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{b}}.

\bibitem[Wang et~al.(2024)Wang, Bai, Tan, Wang, Fan, Bai, Chen, Liu, Wang, Ge, et~al.]{wang2024qwen2}
Peng Wang, Shuai Bai, Sinan Tan, Shijie Wang, Zhihao Fan, Jinze Bai, Keqin Chen, Xuejing Liu, Jialin Wang, Wenbin Ge, et~al.
\newblock Qwen2-vl: Enhancing vision-language model's perception of the world at any resolution.
\newblock \emph{arXiv preprint arXiv:2409.12191}, 2024.

\bibitem[Wang et~al.(2026{\natexlab{c}})Wang, Guo, Cai, and Chen]{wang2026learning}
Wanqi Wang, Jingcai Guo, Yuxiang Cai, and Zhi Chen.
\newblock Learning multi-modal prototypes for cross-domain few-shot object detection.
\newblock \emph{arXiv preprint arXiv:2602.18811}, 2026{\natexlab{c}}.

\bibitem[Wang et~al.(2020)Wang, Huang, Darrell, Gonzalez, and Yu]{wang2020frustratingly}
Xin Wang, Thomas~E Huang, Trevor Darrell, Joseph~E Gonzalez, and Fisher Yu.
\newblock Frustratingly simple few-shot object detection.
\newblock \emph{arXiv preprint arXiv:2003.06957}, 2020.

\bibitem[Wang et~al.(2023)Wang, Li, and Wu]{wang2023cardd}
Xinkuang Wang, Wenjing Li, and Zhongcheng Wu.
\newblock Cardd: A new dataset for vision-based car damage detection.
\newblock \emph{IEEE Transactions on Intelligent Transportation Systems}, 2023.

\bibitem[Wang et~al.(2026{\natexlab{d}})Wang, Liang, Zhang, Zhao, Wang, Li, Yang, Timofte, Guo, et~al.]{ntire26lightsr}
Yingqian Wang, Zhengyu Liang, Fengyuan Zhang, Wending Zhao, Longguang Wang, Juncheng Li, Jungang Yang, Radu Timofte, Yulan Guo, et~al.
\newblock { NTIRE 2026 Challenge on Light Field Image Super-Resolution: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026{\natexlab{d}}.

\bibitem[Wolf et~al.(2020)Wolf, Debut, Sanh, Chaumond, Delangue, Moi, Cistac, Rault, Louf, Funtowicz, Davison, Shleifer, von Platen, Ma, Jernite, Plu, Xu, Scao, Gugger, Drame, Lhoest, and Rush]{transformers}
Thomas Wolf, Lysandre Debut, Victor Sanh, Julien Chaumond, Clement Delangue, Anthony Moi, Pierric Cistac, Tim Rault, Rémi Louf, Morgan Funtowicz, Joe Davison, Sam Shleifer, Patrick von Platen, Clara Ma, Yacine Jernite, Julien Plu, Canwen Xu, Teven~Le Scao, Sylvain Gugger, Mariama Drame, Quentin Lhoest, and Alexander~M. Rush.
\newblock Transformers: State-of-the-art natural language processing.
\newblock 2020.

\bibitem[Wu et~al.(2025{\natexlab{a}})Wu, Li, Zhou, Lin, Gao, Yan, ming Yin, Bai, Xu, Chen, Chen, Tang, Zhang, Wang, Yang, Yu, Cheng, Liu, Li, Zhang, Meng, Wei, Ni, Chen, Cao, Peng, Qu, Wu, Wang, Yu, Wen, Feng, Xu, Wang, Zhang, Zhu, Wu, Cai, and Liu]{qwenimage}
Chenfei Wu, Jiahao Li, Jingren Zhou, Junyang Lin, Kaiyuan Gao, Kun Yan, Sheng ming Yin, Shuai Bai, Xiao Xu, Yilei Chen, Yuxiang Chen, Zecheng Tang, Zekai Zhang, Zhengyi Wang, An Yang, Bowen Yu, Chen Cheng, Dayiheng Liu, Deqing Li, Hang Zhang, Hao Meng, Hu Wei, Jingyuan Ni, Kai Chen, Kuan Cao, Liang Peng, Lin Qu, Minggang Wu, Peng Wang, Shuting Yu, Tingkun Wen, Wensen Feng, Xiaoxiao Xu, Yi Wang, Yichang Zhang, Yongqiang Zhu, Yujia Wu, Yuxuan Cai, and Zenan Liu.
\newblock Qwen-image technical report, 2025{\natexlab{a}}.

\bibitem[Wu et~al.(2025{\natexlab{b}})Wu, Li, Zhou, Lin, Gao, Yan, Yin, Bai, Xu, Chen, et~al.]{wu2025qwen}
Chenfei Wu, Jiahao Li, Jingren Zhou, Junyang Lin, Kaiyuan Gao, Kun Yan, Sheng-ming Yin, Shuai Bai, Xiao Xu, Yilei Chen, et~al.
\newblock Qwen-image technical report.
\newblock \emph{arXiv preprint arXiv:2508.02324}, 2025{\natexlab{b}}.

\bibitem[Yan et~al.(2026)Yan, Tu, Lin, WU, Zhang, Wang, Cao, Fang, Liu, Zhou, Timofte, et~al.]{ntire26effllie}
Jiebin Yan, Chenyu Tu, Qinghua Lin, Zongwei WU, Weixia Zhang, Zhihua Wang, Peibei Cao, Yuming Fang, Xiaoning Liu, Zhuyun Zhou, Radu Timofte, et~al.
\newblock { Efficient Low Light Image Enhancement: NTIRE 2026 Challenge Report }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Yang and Xie(2026)]{yang2026styleproto}
Xi Yang and Quantao Xie.
\newblock Styleproto: Style-augmented prototype learning for cross-domain few-shot object detection.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, 2026.

\bibitem[Yu et~al.(2026)Yu, Sha, Liu, Shen, and Yang]{yu2026acloser}
Xuanlong Yu, Youyang Sha, Longfei Liu, Xi Shen, and Di Yang.
\newblock A closer look at cross-domain few-shot object detection: Fine-tuning matters and parallel decoder helps.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 2026.

\bibitem[Zama~Ramirez et~al.(2026)Zama~Ramirez, Tosi, Di~Stefano, Timofte, Costanzino, Poggi, Salti, Mattoccia, et~al.]{ntire26hrdepth}
Pierluigi Zama~Ramirez, Fabio Tosi, Luigi Di~Stefano, Radu Timofte, Alex Costanzino, Matteo Poggi, Samuele Salti, Stefano Mattoccia, et~al.
\newblock { NTIRE 2026 Challenge on High-Resolution Depth of non-Lambertian Surfaces }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Zha et~al.(2023)Zha, Tang, Sun, and Tang]{zha2023boosting}
Zican Zha, Hao Tang, Yunlian Sun, and Jinhui Tang.
\newblock Boosting few-shot fine-grained recognition with background suppression and foreground alignment.
\newblock \emph{IEEE TCSVT}, 2023.

\bibitem[Zhang et~al.(2022)Zhang, Song, Gao, and Shen]{zhang2022free}
Ji Zhang, Jingkuan Song, Lianli Gao, and Hengtao Shen.
\newblock Free-lunch for cross-domain few-shot learning: Style-aware episodic training with robust contrastive learning.
\newblock In \emph{ACM multimedia}, 2022.

\bibitem[Zhang et~al.(2023)Zhang, Liu, Wang, and Boularias]{zhang2023detect}
Xinyu Zhang, Yuhan Liu, Yuting Wang, and Abdeslam Boularias.
\newblock Detect everything with few examples.
\newblock \emph{arXiv preprint arXiv:2309.12969}, 2023.

\bibitem[Zhao et~al.(2024{\natexlab{a}})]{zhao2024upn}
Hengyue Zhao et~al.
\newblock Universal proposal network for multi-domain visual context understanding.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 2024{\natexlab{a}}.

\bibitem[Zhao et~al.(2024{\natexlab{b}})Zhao, Chen, Xu, Li, Wang, Li, and Huang]{zhao2024open}
Xiangyu Zhao, Yicheng Chen, Shilin Xu, Xiangtai Li, Xinjiang Wang, Yining Li, and Haian Huang.
\newblock An open and comprehensive pipeline for unified object grounding and detection.
\newblock \emph{arXiv preprint arXiv:2401.02361}, 2024{\natexlab{b}}.

\bibitem[Zhong et~al.(2026)Zhong, Ma, Wang, Jiang, Timofte, et~al.]{ntire26anomalydet}
Yan Zhong, Qiufang Ma, Zhen Wang, Tingting Jiang, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge Report on Anomaly Detection of Face Enhancement for UGC Images }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\bibitem[Zhuo et~al.(2022)Zhuo, Fu, Chen, Cao, and Jiang]{zhuo2022tgdm}
Linhai Zhuo, Yuqian Fu, Jingjing Chen, Yixin Cao, and Yu-Gang Jiang.
\newblock Tgdm: Target guided dynamic mixup for cross-domain few-shot learning.
\newblock In \emph{ACM Multimedia}, 2022.

\bibitem[Zhuo et~al.(2024)Zhuo, Fu, Chen, Cao, and Jiang]{zhuo2024unified}
Linhai Zhuo, Yuqian Fu, Jingjing Chen, Yixin Cao, and Yu-Gang Jiang.
\newblock Unified view empirical study for large pretrained model on cross-domain few-shot learning.
\newblock \emph{ACM Transactions on Multimedia Computing, Communications and Applications}, 2024.

\bibitem[Zhuo et~al.(2026)Zhuo, Wang, Qian, and Fu]{zhuo2026segdp}
Linhai Zhuo, Zheng Wang, Tianwen Qian, and Yuqian Fu.
\newblock Segdp: Source-free cross-domain few-shot learning via semantic guided diversity prompting.
\newblock \emph{ACM Transactions on Multimedia Computing, Communications and Applications}, 2026.

\bibitem[Zong et~al.(2023)Zong, Song, and Liu]{codetr}
Zhuofan Zong, Guanglu Song, and Yu Liu.
\newblock Detrs with collaborative hybrid assignments training.
\newblock In \emph{ICCV}, 2023.

\bibitem[Zou et~al.(2026)Zou, Liu, Wu, Zhuang, Wu, Zhou, Timofte, et~al.]{ntire26videores}
Wenbin Zou, Tianyi Liu, Kejun Wu, Huiping Zhuang, Zongwei Wu, Zhuyun Zhou, Radu Timofte, et~al.
\newblock { NTIRE 2026 Challenge on Bitstream-Corrupted Video Restoration: Methods and Results }.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, 2026.

\end{thebibliography}


==> ntire26/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> ntire26/teams/team00_Example/affiliation.tex <==
\subsection*{Example}
\noindent\textit{\textbf{Title: }}Cross-Domain Few-Shot Object Detection via Enhanced Open-Set Object Detector\\
\noindent\textit{\textbf{Members: }} \\
Yuqian Fu$^1$ (\href{mailto:yuqian.fu@insait.ai}{yuqian.fu@insait.ai}),\\
Yu Wang$^2$, \\
Yixuan Pan$^3$, \\
Xingyu Qiu$^2$, \\
$^1$ INSAIT \\
$^2$ Fudan University  \\
$^3$ Southeast University\\



==> ntire26/teams/team00_Example/main.tex <==
\subsection{Example}
\subsubsection{Proposed Method}
We propsose a novel CD-ViTO method for the CD-FSOD, under the close-set setting, which only takes COCO as source data and transfer the model to novel target. 
As in Fig.~\ref{fig:framework}, we build our CD-ViTO upon one open-set detector (DE-ViT) and finetune our method using few labeled instances of target domain. Modules in blue are inherited from DE-ViT while modules in orange are proposed by us. New improvements include learnable instance features, instance reweighting, domain prompter, and finetuning;  

\begin{figure}[h]
\vspace{-0.1in}
\centering	{\includegraphics[width=1.\linewidth]{teams/team00_Example/framework.jpg}}
\vspace{-0.1in}
\caption{(a) Overall framework of CD-ViTO. \label{fig:framework} 
}
\vspace{-0.15in}
\end{figure}

Specifically, given $S$ and $q$ as input, we perform the same steps as DE-ViT to obtain instance features $F_{ins} =\{F_{ins}^{ob}, F_{ins}^{bg}\}$, region proposals $R_{q}$, visual features $F_{q}$, and ROI features $F_{q_{roi}}$.
But different from directly averaging $F_{ins}^{ob}$ to obtain class prototypes $F_{pro}^{ob}$ for objects, we first utilize our $M_{LIF}$ to make the precalculated $F_{ins}$ learnable and adapt them by performing the disentangled detection tasks i.e., the localization task supervised by $\mathcal{L}_{loc}$ and the classification task supervised by $\mathcal{L}_{cls}$. 
we apply our $M_{LR}$ to reweight the weights of object instances features $F_{ins}^{ob}$. Generally, $M_{LR}$ is expected to assign higher values to the high-quality instances with slight IB. In this way, the high-quality instances could contribute more to its class prototype. The $M_{LR}$ is inserted after the $M_{LIF}$ and is optimized use the same $\mathcal{L}_{loc}$, $\mathcal{L}_{cls}$.
In addition, to make the model more robust to the changing styles, our proposed $M_{DP}$ is applied to synthesize several virtual "domains" $F_{domain}$. The goal of the $M_{DP}$ is to introduce such domain perturbations and force our features to be consistent with different domains. To ensure the diversity of the introduced domains and constrain the domains would not affect the semantics of features, an extra loss $\mathcal{L}_{dp}$ is introduced. The $M_{DP}$ is build upon the object prototypes $F_{pro}^{ob}$ and the $\mathcal{L}_{dp}$ works with the $\mathcal{L}_{loc}$ and $\mathcal{L}_{cls}$ together.

As for finetuning, we finetune the top two modules i.e., the $M_{DET}$ and $M_{CLS}$. 
via the object function $\mathcal{L}$ as:
\begin{equation}\label{eq:loss}
\mathcal{L}  = \mathcal{L}_{loc} + \mathcal{L}_{cls} + \mathcal{L}_{dp}.
\end{equation}


\noindent \textbf{Learnable Instance Features $M_{LIF}$.}
% The implementation of our learnable instance features $M_{LIF}$ is quiet easy and efficient. 
Given the precalculated instance features $F_{ins} \in \mathcal{R}^{(N \times K + N_{bg}) \times D}$, where $N$, $K$, $N_{bg}$, $D$ represents the number of object classes, the number of shots, the number of background instances, and the dimension of visual features, $M_{LIF}$ defines a new learnable matrix $F_{ins}^{lea}$ with the same size of $F_{ins}$ and use the $F_{ins}$ for initialization. 

\noindent \textbf{Instance Reweighting Module $M_{IR}$.}
Our $M_{IR}$ is proposed to reweight the instances enabling high-quality object instances e.g., objects with slight IB contribute more to the class prototype. 
% The architecture of $M_{IR}$ is shown in Fig.~\ref{fig:framework}(b). 
Given the learnable instance features $F_{ins}^{lea}$ from $M_{LIF}$, we first obtain the object instance features from  $F_{ins}^{lea}$ and denote it as $F_{ins}^{0} \in \mathcal{R}^{N \times K \times D}$. Our $M_{IR}$ has two paths connected in a residual way. 
More specifically, the lower path feeds the $F_{ins}^{0}$ into an MLP module to get the weighted score which is further used to perform the weighted sum on the initial $F_{ins}^{0}$ resulting in the deformed prototypes $F_{ins}^{att} \in \mathcal{R}^{N \times D}$. The upper path performs the average operation on $F_{ins}^{0}$ getting $F_{ins}^{avg} \in \mathcal{R}^{N \times D}$. The final object prototypes $F_{pro}^{ob}$ are represented as $\alpha fc(F_{ins}^{att}) + (1-\alpha)F_{ins}^{avg}$, where the $fc(\cdot)$ denotes a fully connected layer and $\alpha$ is a hyperparameter.  



\noindent \textbf{Domain Prompter $M_{DP}$.}

Given $F_{domain}$ and $F_{pro}^{ob}$, we first propose the domain diversity loss $\mathcal{L}_{domain}$ to force the different domains e.g., $f^{d_{i}}$ and $f^{d_j}$ to be far from each other. Secondly, for a prototype $f_{p_{i}}$ in $F_{pro}^{ob}$, we randomly perturbs it with two various domains $f^{d_{k}}$ and $f^{d_{m}}$ sampled from $F_{domain}$ forming two perturbed prototypes $f_{p_{i}}^{d_{k}}, f_{p_{i}}^{d_{m}}$. The perturbation is done by adding the features e.g., $f_{p_{i}}^{d_{k}} = f_{p_{i}} +f^{d_{k}}$. 
The domain $f^{d_{m}}$ is also added to other object prototypes forming $f_{p_{j}}^{d_{m}}$, where $j = 1, \ldots, N$. 
We constrain that $f_{p_{i}}^{d_{k}}$ and $f_{p_{i}}^{d_{m}}$ should be close to each other while being distant from perturbed prototypes generated from different class prototypes.
This constitutes our prototype consistency loss $\mathcal{L}_{proto}$.  Both the $\mathcal{L}_{domain}$ and $\mathcal{L}_{proto}$ are implemented by the InfoNCE loss.

\subsubsection{Training Details}
we adopt the "pretrain, finetune, and test" pipeline. 
In the case of our CD-ViTO, the base DE-ViT model pretrained on COCO is taken, then the $M_{DET}$, $M_{CLS}$, $M_{LIF}$, $M_{IR}$, and $M_{DP}$ are tuned on novel support images $S$ using the loss as in Eq.~\ref{eq:loss}.
The hyperparameter $N_{bg}$, $\alpha$ ratio of instance reweighting module, $\tau$ temperature for $\mathcal{L}_{proto}$, $\tau$ temperature for $\mathcal{L}_{domain}$  are set as 530, 0.7, 2, 0.1 for all the target datasets. While the value $N_{dom}$ means the number of virtual domains depending on the number of target classes $N$, specifically, we have $N_{dom} = 2*N$.  The hyperparameter Top-K ($K$) in DE-ViT is set as 5. For datasets with number of classes $N$ less than 5, we have $K=N$. We tune the trainable parameters on 1-shot around 80 epochs, and on 5/10-shot around 40 epochs. The SGD with the learning rate as 0.002 is used as the optimizer. Experiments are performed on four RTX3090 GPUs.



==> ntire26/teams/team10_NTR/affiliation.tex <==
\subsection*{NTR}
\noindent\textit{\textbf{Title: }} NTR\\
\noindent\textit{\textbf{Members: }} \\
Jiachen Tu (\href{mailto:jtu9@illinois.edu}{jtu9@illinois.edu}),\\
Yaokun Shi (\href{mailto:yaokuns2@illinois.edu}{yaokuns2@illinois.edu}),\\
Guoyi Xu (\href{mailto:ericx3@illinois.edu}{ericx3@illinois.edu}),\\
Yaoxin Jiang (\href{mailto:yaoxinj2@illinois.edu}{yaoxinj2@illinois.edu}),\\
Jiajia Liu (\href{mailto:ciciliu2@illinois.edu}{ciciliu2@illinois.edu})\\
\noindent\textit{\textbf{Affiliations: }} \\
University of Illinois Urbana-Champaign

==> ntire26/teams/team10_NTR/main.tex <==
% % NTIRE 2026 CD-FSOD Factsheet
% % Team NTR, University of Illinois Urbana-Champaign

% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{cvpr}

% \usepackage{graphicx}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{bm}
% \usepackage{color}
% \usepackage{xcolor}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% % =========================================================================
% \begin{document}

% \title{NTIRE 2026 Challenge on Cross-Domain Few-Shot Object Detection Factsheet\\
% Team: NTR -- Username: miketjc}

% \author{Jiachen Tu$^{*}$ \quad Guoyi Xu \quad Yaoxin Jiang \quad Jiajia Liu \quad Yaokun Shi\\
% University of Illinois Urbana-Champaign\\
% Champaign, IL 61820, USA\\
% {\tt\small \{jtu9, ericx3, yaoxinj2, ciciliu2, yaokuns2\}@illinois.edu}\\[2pt]
% \small $^{*}$Corresponding author: jtu9@illinois.edu
% }
% \maketitle

% % -------------------------------------------------------------------------
% \section{Team Details}

% \begin{itemize}[noitemsep]
% \item \textbf{Team name:} NTR
% \item \textbf{Team leader:} Jiachen Tu
% \item \textbf{Address:} University of Illinois Urbana-Champaign, Champaign, IL 61820, USA
% \item \textbf{Email:} jtu9@illinois.edu
% \item \textbf{Team members:} Jiachen Tu, Guoyi Xu, Yaoxin Jiang, Jiajia Liu, Yaokun Shi
% \item \textbf{Affiliation:} University of Illinois Urbana-Champaign
% \item \textbf{CodaBench username:} \texttt{miketjc} (jtu9@illinois.edu)
% \end{itemize}

% \noindent\textbf{Testing phase (final):}
% \begin{itemize}[noitemsep,topsep=2pt]
% \item \textbf{Final Score:} 149.7586
% \item D1 (marine fauna): 1-shot = 26.89\%, 5-shot = 38.23\%, 10-shot = 35.03\%
% \item D2 (car detection): 1-shot = 58.84\%, 5-shot = 58.71\%, 10-shot = 58.23\%
% \item D3 (car damage): 1-shot = 17.29\%, 5-shot = 25.82\%, 10-shot = 27.22\%
% \end{itemize}

% % -------------------------------------------------------------------------
% \section{Method}
\subsection{NTR}
\subsubsection{Proposed Method}

\noindent \textbf{Problem Formulation.} Cross-Domain Few-Shot Object Detection (CD-FSOD) aims to detect novel object categories in a target domain given only $K$ annotated support examples per category, where the target domain differs significantly from the source domain.

Formally, let $\mathcal{S} = \{(I_i^s, B_i^s, c_i)\}_{i=1}^{NK}$ denote the support set of $N$ categories with $K$ shots each, where $I_i^s$ is a support image, $B_i^s$ is its bounding box annotation, and $c_i$ is the category label. Given a query image $I^q$ and support set $\mathcal{S}$, the model must predict a set of bounding boxes $\hat{B} = \{(b_j, c_j, s_j)\}$ on $I^q$, where $b_j$, $c_j$, and $s_j$ denote the box coordinates, predicted category, and confidence score, respectively.

The challenge evaluates models under $K \in \{1, 5, 10\}$ shots across three novel test domains (marine fauna, car detection, and car damage detection) using mean Average Precision (mAP). The final ranking score weights 1-shot performance more heavily:
\begin{equation}
\text{Score} = 2 \cdot \overline{\text{mAP}}_{1\text{-shot}} + \overline{\text{mAP}}_{5\text{-shot}} + \overline{\text{mAP}}_{10\text{-shot}},
\end{equation}
where $\overline{\text{mAP}}_{K\text{-shot}}$ is the mean mAP across the three datasets under $K$-shot setting.


\noindent \textbf{Overview: Training-Free FSOD-VFM}

Theyadopt \textbf{FSOD-VFM}~\cite{feng2026fsodvfm}, a training-free few-shot object detection framework that integrates three vision foundation models:

\begin{enumerate}[noitemsep]
    \item \textbf{UPN}~\cite{zhao2024upn} --- Universal Proposal Network for category-agnostic proposal generation;
    \item \textbf{SAM2}~\cite{ravi2024sam2} --- Segment Anything Model 2 for precise mask extraction;
    \item \textbf{DINOv2}~\cite{oquab2024dinov2} ViT-L/14 --- for discriminative feature extraction.
\end{enumerate}

No fine-tuning is performed on the target domain. The method uses only the provided $K$-shot support set at test time.


\noindent \textbf{Method Details}

The FSOD-VFM pipeline proceeds in three stages:

\paragraph{Stage 1: Proposal Generation.}
Given a query image $I^q$, UPN generates a set of category-agnostic bounding box proposals $\mathcal{P} = \{p_1, \ldots, p_M\}$. UPN is pretrained on large-scale data and generalizes to novel domains without retraining.

\paragraph{Stage 2: Feature Matching.}
DINOv2 ViT-L/14 extracts patch-level features from both the support crops and the query proposals. For each support example $(I_i^s, B_i^s)$, the region within $B_i^s$ is cropped and encoded. Query proposal features are matched against support features via cosine similarity to assign category scores.

To address over-fragmentation in UPN proposals (many small, redundant boxes), FSOD-VFM introduces a \textbf{graph-based confidence reweighting} strategy. A graph $G = (V, E)$ is constructed over proposals, where edges connect spatially overlapping proposals. Confidence scores are diffused along the graph to propagate information from high-confidence to neighboring proposals, suppressing spurious detections while preserving true positives.

\paragraph{Stage 3: SAM2 Mask Refinement.}
SAM2 refines proposal boundaries by predicting instance masks for top-scored proposals. The tighter mask-derived bounding boxes improve localization accuracy.

Final detections are produced by non-maximum suppression over the refined, reweighted proposals.

\paragraph{Hyperparameters.}
Theyuse the default FSOD-VFM hyperparameters: diffusion steps $= 30$, graph diffusion weight $\alpha = 0.3$, NMS threshold $\lambda = 0.5$, minimum confidence threshold $= 0.01$.

\noindent \textbf{Foundation Models Used}

Per competition rules, theyuse exactly three foundation models:
\begin{enumerate}[noitemsep]
    \item DINOv2 ViT-L/14~\cite{oquab2024dinov2} (pretrained on LVD-142M, publicly available)
    \item SAM2.1 large~\cite{ravi2024sam2} (pretrained by Meta AI, publicly available)
    \item UPN large~\cite{zhao2024upn} (pretrained for universal proposal generation, publicly available)
\end{enumerate}

\noindent No additional datasets or training data beyond the provided $K$-shot support sets are used.

% -------------------------------------------------------------------------
% \section{Results}

% \begin{table}[ht]
% \centering
% \small
% \caption{Per-dataset mAP (\%) on the final test phase.}
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \textbf{Dataset} & \textbf{Domain} & \textbf{1-shot} & \textbf{5-shot} & \textbf{10-shot} \\
% \midrule
% D1 & Marine fauna (10 cats) & 26.89 & 38.23 & 35.03 \\
% D2 & Car detection (1 cat) & 58.84 & 58.71 & 58.23 \\
% D3 & Car damage (6 cats) & 17.29 & 25.82 & 27.22 \\
% \midrule
% \textbf{Mean} & & \textbf{34.34} & \textbf{40.92} & \textbf{40.16} \\
% \midrule
% \multicolumn{4}{l}{\textbf{Final Score}} & \textbf{149.76} \\
% \bottomrule
% \end{tabular}
% \label{tab:results}
% \end{table}

% \begin{table}[ht]
% \centering
% \small
% \caption{Development phase CodaBench score (validation datasets).}
% \begin{tabular}{@{}lcc@{}}
% \toprule
% \textbf{Phase} & \textbf{Method} & \textbf{Score} \\
% \midrule
% Validation & FSOD-VFM (3 val datasets) & 175.79 \\
% \textbf{Test} & \textbf{FSOD-VFM (3 test datasets)} & \textbf{149.76} \\
% \bottomrule
% \end{tabular}
% \label{tab:phases}
% \end{table}

% \noindent The validation score (175.79) was obtained on three known validation domains (ArTaxOr, Clipart1k, FISH). The test score reflects performance on three previously unseen target domains, demonstrating the method's generalizability.

% -------------------------------------------------------------------------
\subsubsection{Training Details}

\textbf{Platform:} NVIDIA H100 (80 GB) GPU. PyTorch 2.6.0, Python 3.10, CUDA 12.4.

\textbf{Inference runtime:} Approximately 30--90 minutes per dataset/shot case on a single NVIDIA H100 GPU, depending on the number of query images. Total runtime for all 9 cases: approximately 8 hours.

\textbf{Extra training data:} None. This is a training-free method. No additional datasets beyond the provided $K$-shot support sets are used at any stage.

\textbf{Pretrained models:} DINOv2 ViT-L/14, SAM2.1 large, and UPN large (all publicly available). No fine-tuning is applied to any foundation model.

\textbf{Code:} Available in the accompanying code submission (\texttt{NTR\_code.zip}). The code is based on the publicly available FSOD-VFM repository~\cite{feng2026fsodvfm}. Setup requires compiling the UPN CUDA extension (MultiScaleDeformableAttention) and installing SAM2.

\textbf{Challenge impressions:} The CD-FSOD challenge is a well-designed benchmark that highlights a critical limitation of standard FSOD methods --- they often overfit to the source domain and fail when the target domain introduces significant visual style or class distribution shifts. They found that training-free vision foundation models generalize surprisingly well across diverse unseen domains (marine fauna, vehicles, damage detection), outperforming a fine-tuned GroundingDINO baseline on test domains despite the fine-tuned model performing better on validation domains. This suggests that over-parameterized few-shot adaptation can hurt cross-domain generalization. The challenge's emphasis on 1-shot performance (2$\times$ weight) correctly prioritizes the most challenging and practically relevant setting.

% -------------------------------------------------------------------------
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team11_AIRCAS_MILab/affiliation.tex <==
\subsection*{AIRCAS MILab}
\noindent\textit{\textbf{Title: }} Semantic-Filtered Domain-RAG and Auto-Tuned GroundingDINO\\
\noindent\textit{\textbf{Members: }} \\
Zhenzhao Xing (\href{mailto:xingzhenzhao25@mails.ucas.ac.cn}{xingzhenzhao25@mails.ucas.ac.cn}),\\
Dandan Zhao (\href{mailto:zhaodandan@aitech.edu.cn}{zhaodandan@aitech.edu.cn}),\\
Hanzhe Xia (\href{mailto:xiahanzhe25@163.com}{xiahanzhe25@163.com}),\\
Dongdong Lu (\href{mailto:ludd@aircas.ac.cn}{ludd@aircas.ac.cn}),\\
Zhe Zhang (\href{mailto:zhangzhe01@aircas.ac.cn}{zhangzhe01@aircas.ac.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\
AIRCAS MILab

==> ntire26/teams/team11_AIRCAS_MILab/main.tex <==
\subsection{AIRCAS MILab}

\subsubsection{Proposed Method}
The AIRCAS MILab team addresses the cross-domain few-shot object detection challenge by treating it as nine independent few-shot tasks (three target datasets under 1-shot, 5-shot, and 10-shot settings), with the overall pipeline illustrated in Fig.~\ref{fig:method11}.

\begin{figure}[!htbp]
\centering
\def\figPath{teams/team11_AIRCAS_MILab/method_figure.pdf}
\IfFileExists{\figPath}{
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{1.\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put the method figure file (e.g., .pdf/.png/.jpg) in \texttt{teams/team11_AIRCAS MILab/} folder and check filename.
  }}
}
\caption{Overall pipeline of the AIRCAS MILab team's method. Each dataset-shot pair is treated as an independent few-shot task. Support annotations are expanded with semantically filtered Domain-RAG generated samples, used to build task-specific GroundingDINO configurations, and detector outputs are filtered with dataset-specific post-processing for submission.}
\label{fig:method11}
\end{figure}

The AIRCAS MILab team adopts GroundingDINO with a Swin-B visual backbone as the base detector, and fine-tunes it separately for each dataset-shot pair instead of merging all tasks into a single training set. To mitigate the lack of supervision in few-shot scenarios, the team expands original support annotations with Domain-RAG generated samples, and introduces a lightweight semantic filtering step to retain only generated backgrounds semantically compatible with foreground objects, reducing augmentation noise.

Additionally, the team develops an automatic configuration generation and parameter tuning pipeline for GroundingDINO, enabling consistent and reproducible management of all nine task-specific settings (including data paths, class reconstruction, training hyperparameters, checkpoint handling, and inference settings). During inference, dataset-specific post-processing (confidence filtering, NMS, top-$k$ control) is applied to generate final submission files.

The model architecture remains largely consistent with the original GroundingDINO, initialized from official pre-trained checkpoints with no heavy architectural modifications. The focus is on optimizing the data pipeline and task adaptation process: class definitions are automatically reconstructed from target few-shot COCO annotations, and the detector head is adapted to each specific task to ensure stable and robust adaptation to the challenge setting.

The key contributions of the AIRCAS MILab team are as follows:
\begin{itemize}[leftmargin=1.2em]
    \item Semantic filtering is introduced for Domain-RAG generated backgrounds, reducing semantically mismatched augmentation noise before few-shot detector training.
    \item An automatic GroundingDINO configuration generation and parameter tuning pipeline is developed for all nine dataset-shot tasks, covering data paths, class reconstruction, training hyperparameters, checkpoint handling, and inference settings.
    \item Fully task-specific training and dataset-specific inference post-processing are employed (instead of a unified setting), improving stability under cross-domain and extremely low-shot conditions.
\end{itemize}

\subsubsection{Training Details}
The AIRCAS MILab team organizes training around nine independent tasks: dataset1, dataset2, and dataset3 under 1-shot, 5-shot, and 10-shot settings, with no mixing of different datasets or shot settings in a single training set. Each task uses its own task-specific COCO annotation file and GroundingDINO configuration to avoid cross-dataset contamination and preserve the integrity of the few-shot setting.

Original support annotations are converted to task-specific COCO training files and expanded with Domain-RAG generated samples (after semantic filtering to remove semantically inconsistent backgrounds). GroundingDINO is fine-tuned with the AdamW optimizer, and the learning rate and epoch number are adjusted according to the shot setting and target dataset. The validation stage is disabled during training (due to the lack of bounding-box ground truth in official test annotations), with checkpoints saved directly to reduce unnecessary computation.

The team also explored a second-stage pseudo-label re-training scheme (using high-confidence predictions on unlabeled images to augment annotations), but abandoned it in the final submission due to overfitting risks in extremely low-shot conditions. Training and inference are conducted on a single GPU (exact hardware details to be provided by the team).

For inference, the team performs task-specific checkpoint selection and dataset-specific post-processing (instead of global settings). Key post-processing steps include confidence thresholding, per-class NMS, image-id alignment, per-image top-$k$ filtering, and json schema normalization (to match challenge evaluation format). The confidence threshold, NMS IoU threshold, and top-$k$ values are tuned separately for each dataset to adapt to different domain characteristics (background complexity, object scale, false-positive patterns). No ensemble or test-time augmentation (TTA) is used in the final submission.

==> ntire26/teams/team11_AIRCAS_MILab/ori.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% % \usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}
% \usepackage{rotating}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}
% \Crefname{figure}{Figure}{Figures}
% \crefname{figure}{Fig.}{Figs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\Semantic-Filtered Domain-RAG and Auto-Tuned GroundingDINO}

% \author{
% Zhenzhao Xing \quad Dandan Zhao \quad Hanzhe Xia \quad Dongdong Lu \quad Zhe Zhang\\
% AIRCAS MILab\\
% {\tt\small xingzhenzhao25@mails.ucas.ac.cn}
% }

% \maketitle

% \section{Introduction}

% This factsheet presents our submission to the NTIRE 2026 Cross-Domain Few-Shot Object Detection (CD-FSOD) Challenge. The challenge targets an extremely data-scarce setting, where the target domains are substantially different from the source distribution and only a very limited number of annotated samples are available for each novel class. Under this setting, detector stability, data quality, and task-specific adaptation become more important than simply increasing training complexity.

% Our solution treats the challenge as nine independent few-shot detection tasks, corresponding to three target datasets under 1-shot, 5-shot, and 10-shot settings. Instead of training a single unified model across all domains and all shot configurations, we fine-tune a dedicated detector for each dataset-shot pair. This design avoids cross-task interference and makes it easier to control class definitions, hyperparameters, checkpoints, and post-processing strategies in a reproducible way.

% The detector is built on GroundingDINO with a Swin-B backbone. Our main effort is devoted to stable cross-domain few-shot adaptation rather than heavy architectural modification. Specifically, the full pipeline combines: (1) task-specific annotation preparation, (2) Domain-RAG based data expansion, (3) semantic filtering for generated backgrounds, (4) automatic configuration generation for GroundingDINO, and (5) dataset-specific post-processing during inference. We also explored a pseudo-label refinement stage, but found that direct inference from the first-stage augmented model was often more reliable under extremely low-shot conditions.

% The provided factsheet, source codes, trained models, and final prediction files are intended to support reproducibility and transparent evaluation. In the final submission, we will provide the corresponding download links and package the factsheet both as a compiled PDF and as a ZIP archive containing the \texttt{.tex} source files.

% \section{Email Final Submission Guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here if needed.\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{AIRCAS MILab} - \texttt{TEAM\_ID}\\

% To obtain the \texttt{TEAM\_ID}, please register in the official Google Sheet and fill in the Team Name, Contact Person, and Contact Email in the first available row.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{AIRCAS MILab}
%     \item Team leader (contact): \texttt{Zhenzhao Xing}, \texttt{xingzhenzhao25@mails.ucas.ac.cn}
%     \item Team members: \texttt{Dandan Zhao (zhaodandan@aitech.edu.cn), Hanzhe Xia (xiahanzhe25@163.com), Dongdong Lu (ludd@aircas.ac.cn), Zhe Zhang (zhangzhe01@aircas.ac.cn)}
%     \item Username on the NTIRE 2026 CodaLab/CodaBench Competition Platform: \texttt{[TO BE FILLED]}
%     \item Method name / nickname: \texttt{SF-DomainRAG + Auto-Tuned GroundingDINO}
%     \item Download methods for the factsheet, code, and pre-trained models: \texttt{[TO BE FILLED]}
% \end{enumerate}

% \noindent The factsheet should be submitted as a compiled PDF together with a ZIP archive containing the \texttt{.tex} source files.

% \section{Code Submission}

% \noindent Code link / repository: \texttt{[TO BE FILLED]}\\
% \noindent Models / weights link: \texttt{[https://pan.baidu.com/s/1kINv-SkBmmM8goOnIfBERA?pwd=utbe]}\\
% \noindent Reproduction instructions (brief): \texttt{Prepare semantically filtered Domain-RAG augmented annotations, automatically generate GroundingDINO configurations for all nine dataset-shot tasks, fine-tune task-specific models, and export json predictions with dataset-specific post-processing.}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}[leftmargin=1.2em]
% \item Team name: \texttt{AIRCAS MILab}
% \item Team leader: \texttt{Zhenzhao Xing}
% \item Affiliation / contact: \texttt{AIRCAS MILab, xingzhenzhao25@mails.ucas.ac.cn}
% \item Team members: \texttt{Zhenzhao Xing (xingzhenzhao25@mails.ucas.ac.cn), Dandan Zhao (zhaodandan@aitech.edu.cn), Hanzhe Xia (xiahanzhe25@163.com), Dongdong Lu (ludd@aircas.ac.cn), Zhe Zhang (zhangzhe01@aircas.ac.cn)}
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \texttt{SF-DomainRAG + Auto-Tuned GroundingDINO}
% \item Final score : \texttt{[150.6085]}
% \item Submission link: \texttt{[TO BE FILLED]}
% \end{itemize}
\subsection{AIRCAS MILab}

\subsubsection{Proposed Method}

% \begin{figure*}[t]
% \centering
% \IfFileExists{teams2026/team11_AIRCAS MILab/method_figure.pdf}{
%   \includegraphics[width=0.95\textwidth]{method_figure.pdf}
% }{
%   \IfFileExists{method_figure.png}{
%     \includegraphics[width=0.95\textwidth]{method_figure.png}
%   }{
%     \IfFileExists{method_figure.jpg}{
%       \includegraphics[width=0.95\textwidth]{method_figure.jpg}
%     }{
%       \fbox{\parbox[c][0.23\textheight][c]{0.95\textwidth}{
%       \centering \textbf{Method Figure Placeholder}\\[4pt]
%       Put \texttt{method\_figure.pdf} (or \texttt{.png}/\texttt{.jpg}) in the same folder and update the filename if needed.
%       }}
%     }
%   }
% }
% \caption{Overall pipeline of our method. Each dataset-shot pair is treated as an independent few-shot task. The support annotations are first expanded with semantically filtered Domain-RAG generated samples, then used to automatically build task-specific GroundingDINO configurations, and finally the detector outputs are filtered with dataset-specific post-processing for submission.}
% \label{fig:method}
% % \end{figure*}
% \begin{figure*}[t]
% \centering
% % 定义统一的基础路径变量，解决多层判断的路径不一致问题
% \def\figBasePath{teams2026/team11_AIRCAS MILab/}
% % 依次检查PDF/PNG/JPG格式，且所有检查/加载路径统一
% \IfFileExists{\figBasePath method_figure.pdf}{
%   \includegraphics[width=0.95\textwidth]{\figBasePath method_figure.pdf}
% }{
%   \IfFileExists{\figBasePath method_figure.png}{
%     \includegraphics[width=0.95\textwidth]{\figBasePath method_figure.png}
%   }{
%     \IfFileExists{\figBasePath method_figure.jpg}{
%       \includegraphics[width=0.95\textwidth]{\figBasePath method_figure.jpg}
%     }{
%       \fbox{\parbox[c][0.23\textheight][c]{0.95\textwidth}{
%       \centering \textbf{Method Figure Placeholder}\\[4pt]
%       Put \texttt{method\_figure.pdf} (or \texttt{.png}/\texttt{.jpg}) in \texttt{teams2026/team11_AIRCAS MILab/} and update the filename if needed.
%       }}
%     }
%   }
% }


\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，便于维护和排查
\def\figPath{teams2026/team11_AIRCAS MILab/method_figure.pdf}
% 增加文件存在性检查，避免图片缺失时报错，同时给出清晰提示
\IfFileExists{\figPath}{
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{}\\
  Put \texttt{} (or .png/.jpg) in the \texttt{images/} folder (relative to main .tex file) and check filename.
  }}
}



\caption{Overall pipeline of our method. Each dataset-shot pair is treated as an independent few-shot task. The support annotations are first expanded with semantically filtered Domain-RAG generated samples, then used to automatically build task-specific GroundingDINO configurations, and finally the detector outputs are filtered with dataset-specific post-processing for submission.}
\label{fig:method11}
\end{figure}


\noindent \textbf{High-level idea:}
Our solution addresses the challenge as nine independent few-shot object detection tasks, corresponding to three target datasets under 1-shot, 5-shot, and 10-shot settings. We adopt GroundingDINO with a Swin-B backbone as the base detector and fine-tune it separately for each dataset-shot pair instead of merging all tasks into a single training set. To alleviate the severe lack of supervision in the few-shot regime, we expand the original support annotations with Domain-RAG generated samples. A lightweight semantic filtering step is introduced before the generated data are merged back into the training set, so that only generated backgrounds that remain semantically compatible with the foreground object are preserved. In addition, we build an automatic configuration generation and parameter tuning pipeline for GroundingDINO, which allows us to manage all nine task-specific settings consistently and reproducibly. During inference, final submission json files are produced with dataset-specific confidence filtering, NMS, and top-\emph{k} control.

\noindent \textbf{Key contributions:}
\begin{itemize}[leftmargin=1.2em]
    \item \textbf{Contribution 1:} We introduce semantic filtering for Domain-RAG generated backgrounds, which reduces semantically mismatched augmentation noise before few-shot detector training.
    \item \textbf{Contribution 2:} We develop an automatic GroundingDINO configuration generation and parameter tuning pipeline for all nine dataset-shot tasks, including data paths, class reconstruction, training hyperparameters, checkpoint handling, and inference settings.
    \item \textbf{Contribution 3:} We employ fully task-specific training and dataset-specific inference post-processing instead of a single unified setting, which improves stability under cross-domain and extremely low-shot conditions.
\end{itemize}

\noindent\textbf{Model architecture}

The detector is based on GroundingDINO and initialized from an official pre-trained checkpoint. We use the Swin-B version as the visual backbone and keep the detector architecture itself largely unchanged. Rather than introducing a heavy architectural modification, we focus on improving the data pipeline and the task adaptation process. In particular, the class definitions are reconstructed automatically from the target few-shot COCO annotations, and the detector head is adapted to the corresponding task. This design keeps the main model stable while allowing robust adaptation to the challenge setting.

\begin{itemize}[leftmargin=1.2em]
    \item Backbone: \texttt{Swin-B}
    \item Detector: \texttt{GroundingDINO}
    \item Additional components: \texttt{Semantic filtering for Domain-RAG augmentation, automatic config generation, and dataset-specific post-processing}
\end{itemize}

\subsubsection{Training details}

The training pipeline is organized around nine independent tasks: dataset1, dataset2, and dataset3 under 1-shot, 5-shot, and 10-shot settings. We do not mix different datasets or different shot settings into a single training set, because their visual domains and supervision scales are clearly different. Each task is therefore trained independently with its own COCO annotation file and its own GroundingDINO configuration.

The original support annotations are first converted into task-specific COCO training files. We then expand them with Domain-RAG generated samples. However, the generated samples are not used blindly. During background generation, some outputs are visually diverse but semantically inconsistent with the foreground object or scene context. To reduce this type of noise, we apply a semantic filtering stage and only retain generated results that remain compatible with the original object semantics. The selected generated images are then copied into the corresponding training directory and merged into the few-shot COCO annotations of the same task.

This produces augmented training files such as \texttt{1\_shot\_domainrag\_aug.json}, \texttt{5\_shot\_domainrag\_aug.json}, and \texttt{10\_shot\_domainrag\_aug.json}. The same principle is applied throughout the pipeline: augmented samples are only merged back into the original dataset-shot task from which they are derived. This prevents cross-dataset contamination and preserves the integrity of the few-shot setting.

GroundingDINO is fine-tuned with AdamW. The learning rate and epoch number are adjusted according to the shot setting and the target dataset. Because the official test annotation file does not contain bounding-box ground truth, we disable the validation stage during training and save checkpoints directly. This avoids meaningless validation loops and reduces unnecessary computation. In practice, this design is more suitable for the challenge setup than forcing a conventional validation protocol on unlabeled test annotations.

We also explored a second-stage pseudo-label re-training scheme. The idea was to use the first-stage detector to predict high-confidence boxes on unlabeled training images, merge them into the augmented annotations, and fine-tune again. While this strategy can recover some missed instances, we observed that in extremely low-shot conditions pseudo-label noise may easily lead to overfitting. Therefore, our final submission relies primarily on the first-stage augmented model and carefully tuned test-time filtering.

\begin{itemize}[leftmargin=1.2em]
    \item Training data: \texttt{dataset1 / dataset2 / dataset3, each with separate 1-shot, 5-shot, and 10-shot task-specific COCO annotations}
    \item Few-shot setting: \texttt{1-shot, 5-shot, and 10-shot; all nine tasks trained independently}
    \item Optimization: \texttt{GroundingDINO fine-tuning with AdamW, task-specific learning rate and epoch settings}
    \item Augmentations: \texttt{Domain-RAG generated data with semantic filtering before annotation merging}
    \item Hardware / runtime: \texttt{Single-GPU training and inference pipeline; exact hardware information can be filled in by the team}
\end{itemize}

\noindent\textbf{Inference details}

Inference is carried out separately for each dataset and each shot setting. The final json results are exported directly from selected GroundingDINO checkpoints. Since no official validation set with bounding-box labels is provided, we support explicit checkpoint and epoch selection during testing. This allows us to compare different checkpoints from the same training run and choose a more reliable model for submission.

We apply dataset-specific post-processing instead of using a single global setting for all domains. In particular, the confidence threshold, NMS IoU threshold, and per-image top-\emph{k} filtering are adjusted separately for dataset1, dataset2, and dataset3. This is important because the three target domains have different background complexity, object scale distributions, and false-positive patterns. In addition, we include image-id alignment and json schema normalization in the export pipeline to ensure that the submission files strictly match the evaluation format required by the challenge.

\begin{itemize}[leftmargin=1.2em]
    \item Test-time settings: \texttt{GroundingDINO export with task-specific checkpoint selection and dataset-specific post-processing}
    \item Ensemble / TTA: \texttt{Not used in the final submission}
    \item Any post-processing: \texttt{Confidence thresholding, per-class NMS, image-id alignment, and per-image top-k filtering}
\end{itemize}

% \subsection{Experimental results}

% Our experiments mainly compare two training strategies: the first-stage model trained on semantically filtered Domain-RAG augmented data, and the second-stage model further refined with pseudo labels. We observe that pseudo-label re-training is not consistently beneficial under the extremely low-shot setting. In several cases, the first-stage augmented model generalizes better than the second-stage model, suggesting that supervision quality is more critical than supervision quantity when the annotation budget is extremely limited.

% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{c l c c c c}
% \toprule
% \textbf{Shot} & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{1-shot}
% & Baseline / Reference & Open & -- & -- & -- \\
% & Ours (SF-DomainRAG + Auto-Tuned GDINO) & Open & 21.264 & 30.8204 & 34.1407 \\
% \midrule
% \multirow{2}{*}{5-shot}
% & Baseline / Reference & Open & -- & -- & -- \\
% & Ours (SF-DomainRAG + Auto-Tuned GDINO) & Open & 57.1144 & 55.3462 & 58.2842 \\
% \midrule
% \multirow{2}{*}{10-shot}
% & Baseline / Reference & Open & -- & -- & -- \\
% & Ours (SF-DomainRAG + Auto-Tuned GDINO) & Open & 18.3613 & 59.6604 & 41.1944 \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1-shot, 5-shot, and 10-shot settings on the three target datasets.}
% \label{tab:results}
% \end{table*}

% \subsection{Ablation and analysis (optional)}

% \begin{itemize}[leftmargin=1.2em]
%     \item Ablation 1: \texttt{Removing the semantic filtering step from Domain-RAG background selection reduces the quality of augmented training samples and makes the few-shot training process less stable.}
%     \item Ablation 2: \texttt{Replacing the automatic GroundingDINO config generation with manual configuration increases the risk of class-mapping errors, wrong annotation paths, and inconsistent parameter settings across the nine tasks.}
%     \item Failure cases: \texttt{Common failure cases include small objects in cluttered backgrounds, confusion between visually similar categories, and overfitting caused by noisy pseudo labels in extremely low-shot conditions.}
% \end{itemize}

% \section{Other details}

% \begin{itemize}[leftmargin=1.2em]
% \item Planned submission of a solution description paper at the NTIRE 2026 workshop: \texttt{Yes}
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{This challenge is well designed to reflect a realistic and difficult cross-domain few-shot detection setting. It clearly exposes the trade-off between strong pre-trained detectors, data augmentation, and the risk of overfitting under very limited supervision.}
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{Providing an official validation split or a small labeled development set would make checkpoint selection and ablation analysis more reliable, especially in the current setting where public test annotations do not provide ground-truth boxes.}
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{A major practical difficulty is that pseudo-label refinement does not always improve performance in an extreme few-shot setting. Better validation support or more explicit development protocols would help distinguish genuine model improvement from pseudo-label overfitting.}
% \end{itemize}

% %%%%%%%%% REFERENCES
% {\small
% \begin{thebibliography}{1}

% \bibitem{fu2025cross}
% Fu, Y., Qiu, X., Ren, B., Fu, Y., Timofte, R., Sebe, N., Yang, M.-H., Van Gool, L., et al.
% \newblock NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.
% \newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, pages 1048--1069, 2025.

% \end{thebibliography}
% }

% \end{document}

==> ntire26/teams/team12_J_G_team/affiliation.tex <==
\subsection*{J\_G\_team}
\noindent\textit{\textbf{Title: }} Negative Prompting for Few-Shot Object Detection\\
\noindent\textit{\textbf{Members: }} \\
Jingru Wang (\href{mailto:wjr19950102@163.com}{wjr19950102@163.com}),\\
Guangwei Huang (\href{mailto:hgw61638181@gmail.com}{hgw61638181@gmail.com})\\
\noindent\textit{\textbf{Affiliations: }} \\
Free researcher, China

==> ntire26/teams/team12_J_G_team/main.tex <==
\subsection{J\_G\_team}

\subsubsection{Proposed Method}
The J\_G\_team proposes a few-shot object detection method based on FSOD-VFM~\cite{feng2025fsodvfm} with two key improvements to enhance detection accuracy. As shown in Fig.~\ref{fig:method12}, the overall pipeline of this method focuses on strengthening the model's discrimination ability between foreground and background, as well as its adaptability to intra-class variation.

\begin{figure}[!htbp]
\centering
% 定义图片路径变量，便于维护和修改
\def\figPath{teams/team12_J_G_team/images/fig1.png}
\IfFileExists{\figPath}{
  % 加载和检查使用相同的完整路径，避免路径不一致问题
  \includegraphics[width=1.\linewidth]{\figPath}
}{
  % 占位框：保持原样式，提示用户正确放置图片
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{fig1.png} (or .pdf/.jpg) in \texttt{teams/team12_J_G_team/images/} and check filename.
  }}
}
\caption{Overall pipeline of Negative Prompting for Few-Shot Object Detection.}
\label{fig:method12}
\end{figure}

First, the J\_G\_team incorporates negative sample features generated by randomly shifting and scaling positive bounding boxes, which provides the model with additional background context to help distinguish foreground from background. Second, the team replaces static class prototypes with query-adaptive cross-attention prototypes, allowing support features to be dynamically weighted according to each query proposal and thus improving matching precision.

The model architecture of the proposed method consists of three core components: (1) Universal Proposal Network~\cite{jiang2024chatrextamingmultimodalllm} is used as the detector to generate category‑agnostic bounding box proposals for candidate objects; (2) SAM2 is employed as the mask extraction module to produce accurate object masks for support annotations, aiding robust feature extraction; (3) C-RADIOv4-H is adopted as the visual feature extractor for the whole image. During inference, the J\_G\_team sets specific preprocessing rules: C-RADIOv4 resizes all input images so that the longer side is 1260, and for all proposals generated by UPN, the top 100 boxes per image ranked by confidence are selected.

\subsubsection{Training Details}
The method proposed by the J\_G\_team is training-free and does not require any task-specific finetuning, which is a key characteristic of its implementation process.



==> ntire26/teams/team12_J_G_team/ori.tex <==
% \subsection{J\_G\_team}
% \subsubsection{Proposed Method}
% % (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams2026/team12_J_G_team/images/fig1.png}{
%   \includegraphics[width=0.95\linewidth]{images/fig1.png}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }
% \caption{Overall pipeline of Negative Prompting for Few-Shot Object Detection.}
% \label{fig:method}
% \end{figure}
\subsection{J\_G\_team}
\subsubsection{Proposed Method}
% (Optional) Add a method figure if you have one.
\begin{figure}[!htbp]
\centering
% 定义图片路径变量，便于维护和修改
\def\figPath{teams2026/team12_J_G_team/images/fig1.png}
\IfFileExists{\figPath}{
  % 加载和检查使用相同的完整路径，避免路径不一致问题
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  % 占位框：保持原样式，提示用户正确放置图片
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{fig1.png} (or .pdf/.jpg) in \texttt{teams2026/team12_J_G_team/images/} and check filename.
  }}
}
\caption{Overall pipeline of Negative Prompting for Few-Shot Object Detection.}
\label{fig:method12}
\end{figure}

\noindent \textbf{High-level idea:} We propose a few-shot object detection method based on FSOD-VFM\cite{feng2025fsodvfm} with two key improvements. First, we incorporate negative sample features generated by randomly shifting and scaling positive bounding boxes, providing the model with additional background context. Second, we replace static class prototypes with query-adaptive cross-attention prototypes, allowing support features to be dynamically weighted according to each query proposal. These two strategies improve the model’s ability to discriminate between foreground and background, and enable it to adapt to intra-class variation, leading to more accurate detection.\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} We introduce negative sample features as additional guidance, helping the model distinguish foreground from background.
    \item \textbf{Contribution 2:} We propose cross-attention prototypes that dynamically adapt to each query proposal, improving matching precision.
\end{itemize}

\noindent \textbf{Model architecture}
\begin{itemize}
    \item \textbf{Detector:} Universal Proposal Network\cite{jiang2024chatrextamingmultimodalllm} is used to generate category‑agnostic bounding box proposals for candidate objects.
    \item \textbf{Mask extraction module:} SAM2 is employed to produce accurate object masks for support annotations, aiding robust feature extraction.
    \item \textbf{Visual Feature Extractor:} We use C-RADIOv4-H as visual feature extractor for whole image.
\end{itemize}

\subsubsection{Training details}
This method is training-free and does not require any task-specific finetuning.

\noindent \textbf{Inference details}
\begin{itemize}
    \item Test-time settings: During preprocessing, C-RADIOv4 resizes all input images so that the longer side is 1260. For all proposals generated by UPN, we select top 100 boxes per image ranked by confidence.
\end{itemize}

% \subsection{Experimental results}
% Experimental results is shown in Table.\ref{tab:results}.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% &  FSOD-VFM & \texttt{(Open)} & \texttt{26.93} & \texttt{58.84} & \texttt{17.28} \\
% & Ours & \texttt{(Open)} & \texttt{26.71} & \texttt{57.99} & \texttt{18.01} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & FSOD-VFM & \texttt{(Open)} & \texttt{38.21} & \texttt{58.70} & \texttt{25.80} \\
% & Ours & \texttt{(Open)} & \texttt{38.46} & \texttt{57.94} & \texttt{26.77} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & FSOD-VFM & \texttt{(Open)} & \texttt{35.03} & \texttt{58.21} & \texttt{27.31} \\
% & Ours & \texttt{(Open)} & \texttt{34.85} & \texttt{57.50} & \texttt{28.86} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Replace placeholders with official numbers.}
% \label{tab:results}
% \end{table}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: No.
% \item General comments and impressions of the NTIRE 2026 challenge: This challenge provides a valuable benchmark for evaluating few-shot object detection under cross-domain scenarios. The task setup is meaningful and reflects practical challenges in real-world applications.
% \item Suggestions for future CD-FSOD challenges: Future editions of the challenge could explore more diverse domain shifts or introduce additional subtracks focusing on efficiency.
% \end{itemize}

%%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team13_WRC/affiliation.tex <==
\subsection*{WRC}

\noindent\textit{\textbf{Title: }} MQ-Det\\
\noindent\textit{\textbf{Members: }} \\
Liwei Zhou (\href{mailto:zhouliwei123@nudt.edu.cn}{zhouliwei123@nudt.edu.cn}),\\
Bei Dou (\href{mailto:doubei@nudt.edu.cn}{doubei@nudt.edu.cn}),\\
Tao Wu (\href{mailto:wutao@nudt.edu.cn}{wutao@nudt.edu.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\
College of Intelligence Science and Technology, National University of Defense Technology, China

==> ntire26/teams/team13_WRC/main.tex <==
\subsection{WRC}

\subsubsection{Proposed Method}
Based on the image-text multimodal detector GroundingDINO, the WRC team proposes a novel framework for multimodal query-based object detection, whose overall pipeline is illustrated in Fig.~\ref{fig:method13}.

\begin{figure}[!htbp]
\centering
\def\figPath{teams/team13_WRC/images/method_figure.png}
\IfFileExists{\figPath}{
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.8\textheight][c]{1.\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method\_figure.png} (or .png/.jpg) in \texttt{teams2026/team13_WRC/images/} folder and check filename.
  }}
}
\caption{Overall pipeline of Multimodal Query-based Object Detection.}
\label{fig:method13}
\end{figure}

At a high level, the WRC team first constructs a full-level multi-scale visual query library, and performs instantiation and cascaded refinement on retrieved visual features under the guidance of text semantics. The refined visual queries are then embedded into the deep layers of the frozen text encoder through a gated adaptive fusion mechanism, realizing efficient cross-modal alignment between visual and textual features.

For model training, the team conducts joint image-text fine-tuning with a lightweight strategy: the visual backbone network and shallow layers of the text encoder are frozen to retain basic representation ability. Learnable continuous prompt parameters are introduced into the text branch, and LoRA low-rank adaptation is applied to the cross-attention layer for visual-text fusion. To handle partially unlabeled instances in few-shot datasets, the team incorporates the EMA Mean Teacher to generate pseudo-labels, which strengthens fine-tuning performance. Only the parameters of the fusion module are tuned to improve few-shot object detection performance.

In terms of model architecture, the WRC team uses Swin-T as the visual backbone and BERT-base-uncased as the text encoder, with Deformable DETR as the detection framework. Additional key components include a Vision Query Bank, gated cross-attention, CoOp learnable prompts, and LoRA modules, which are integrated into the vision-language fusion pipeline to bridge the modal gap and align fine-grained visual-text features.

The key contributions of the WRC team are summarized as follows:
\begin{itemize}
    \item A vision-enhanced text branch is built to reduce the modality gap of pure text in describing fine-grained visual characteristics, through constructing a visual query library, cascaded feature refinement, and gated adaptive fusion for efficient cross-modal alignment.
    \item A lightweight joint image-text fine-tuning scheme is designed, which freezes the visual backbone and shallow text encoder, applies learnable prompts and LoRA adaptation, and only fine-tunes the fusion module to improve few-shot detection performance and alleviate overfitting.
\end{itemize}

\subsubsection{Training Details}
The WRC team conducts experiments on the COCO17 dataset under few-shot settings of 1/5/10-shots, using fixed support sets provided by the challenge. The model is optimized with the AdamW optimizer at a learning rate of 1e-4, equipped with a WarmupMultiStepLR scheduler. Training runs for 20 epochs with 1 warm-up epoch.

Data augmentations applied during training include multi-scale resizing, random horizontal flipping, and standard normalization. All experiments are run on a single NVIDIA A100 GPU, with a total training time of approximately 3 hours.

For inference, the model uses a fixed test scale with a short edge of 800 and a maximum long edge of 1333, a score threshold of 0.05, and a maximum number of detections set to 900. No test-time augmentation, model ensemble, or extra post-processing operations are adopted during the inference stage.

==> ntire26/teams/team13_WRC/ori.tex <==
\subsection{WRC}
\subsubsection{Proposed Method}

% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{WRC} - \texttt{13}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{WRC}
%     \item Team leader (contact): \texttt{Liwei Zhou}, \texttt{zhouliwei123@nudt.edu.cn}
%     \item Team members: \texttt{Liwei Zhou, Bei Dou, Tao Wu}
%     \item Method name / nickname: \texttt{MQ-Det}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/your_repo}{https://github.com/ZLW-123-123/MQ-Det-main.git}\\
% \noindent Models / weights link: \url{https://pan.baidu.com/s/18qNyIaUNHYJlZRxPONuCVQ?pwd=n4yd}\\
% \noindent Reproduction instructions (brief): \texttt{bash extract.sh, bash stage2.sh, bash inference.sh}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: \texttt{WRC}
% \item Team leader: \texttt{Liwei Zhou}
% \item Affiliation / contact: \texttt{College of Intelligence Science and Technology, National University of Defense Technology,  zhouliwei123@nudt.edu.cn}
% \item Team members: \texttt{Liwei Zhou, Bei Dou, Tao Wu}
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \texttt{MQ-Det}
% \item Final score (if available): \texttt{139.7438}
% \item Submission link: \url{https://www.codabench.org/profiles/user/zhouliwei21/}
% \end{itemize}

% \subsection{Method overview}
% (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams2026/team13_WRC/images/method_figure.png}{  
%   \includegraphics[width=0.95\linewidth]{images/method_figure.png}  
% }{
%   \fbox{\parbox[c][0.8\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.png} (or .png/.jpg) in the \texttt{images/} folder and update filename.  
%   }}
% }
% \caption{Overall pipeline of Multimodal Query-based Object Detection.}

% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，解决路径不一致问题
\def\figPath{teams2026/team13_WRC/images/method_figure.png}
\IfFileExists{\figPath}{
  % 加载路径与检查路径完全一致，保留原宽度设置
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  % 优化占位提示，明确图片应放置的正确路径，保留原高度比例
  \fbox{\parbox[c][0.8\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method\_figure.png} (or .png/.jpg) in \texttt{teams2026/team13_WRC/images/} folder and check filename.
  }}
}
\caption{Overall pipeline of Multimodal Query-based Object Detection.}
\label{fig:method13}
\end{figure}

\noindent \textbf{High-level idea:}Based on an image-text multimodal detector\cite{groundingdino2024}, this method first constructs a full-level multi-scale visual query library, and performs instantiation and cascaded refinement guided by text semantics on the retrieved visual features. It then embeds the refined visual queries into the deep layers of the frozen text encoder via a gated adaptive fusion mechanism, achieving efficient cross-modal alignment of visual and textual features. Subsequent joint image-text fine-tuning is carried out: the visual backbone network and the shallow layers of the text encoder are frozen to preserve the basic representation capability; learnable continuous prompt parameters are introduced into the text branch, and LoRA low-rank adaptation is added to the cross-attention layer for visual-text fusion. To address the partially unlabeled instances existing in the few-shot dataset, the EMA (Exponential Moving Average) Mean Teacher\cite{meanteacher2017} is incorporated to generate pseudo-labels, thereby enhancing the effect of model fine-tuning. Only the parameters of the fusion module are fine-tuned to improve the performance of few-shot object detection.\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} A vision-enhanced text branch is constructed, which bridges the modal gap of pure text in characterizing fine-grained visual features and enables efficient cross-modal alignment of visual-text features via the establishment of a visual query library, cascaded refinement of retrieved features and gated adaptive fusion.
    \item \textbf{Contribution 2:} A lightweight joint image-text fine-tuning strategy is designed: the visual backbone and shallow layers of the text encoder are frozen, learnable prompt parameters are introduced into the text branch, LoRA adaptation is applied to the cross-attention layer for visual-text fusion, and only the fusion module is fine-tuned to boost few-shot detection performance and mitigate overfitting.
\end{itemize}

\noindent \textbf{Model architecture}
Describe the backbone, detector head, any added modules, and where they are inserted.
\begin{itemize}
    \item Backbone: \texttt{(Swin-T, BERT-base-uncased)}
    \item Detector: \texttt{(Deformable DETR)}
    \item Additional components: \texttt{(Vision Query Bank, Gated Cross-Attention, CoOp, LoRA)}
\end{itemize}

\subsubsection{Training details}
Provide training settings sufficient for reproduction.
\begin{itemize}
    \item Training data: \texttt{(coco17)}
    \item Few-shot setting: \texttt{(1/5/10-shot,challenge-provided fixed support sets)}
    \item Optimization: \texttt{(AdamW, 1e-4, WarmupMultiStepLR, 1, 20)}
    \item Augmentations: \texttt{(Multi-scale Resize, Random Horizontal Flip, Normalization)}
    \item Hardware / runtime: \texttt{(A100, 1 GPU, 3 hours)}
\end{itemize}

\noindent \textbf{Inference details}
Explain inference-time details that affect performance.
\begin{itemize}
    \item Test-time settings: \texttt{(Scale: Short edge 800, Long edge max 1333, score threshold: 0.05, Max Detections: 900 )}
    \item Ensemble / TTA: \texttt{(None)}
    \item Any post-processing: \texttt{(None)}
\end{itemize}

% \subsection{Experimental results}
% Fill in your results. Replace dataset names with official ones used in the challenge.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{12.8} & \texttt{8.0} & \texttt{15.8} \\
% & Ours (\texttt{MQ-Det}) & \texttt{(Close)} & \texttt{15.6} & \texttt{53.2} & \texttt{21.9} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{22.7} & \texttt{19.8} & \texttt{29.1} \\
% & Ours (\texttt{MQ-Det}) & \texttt{(Close)} & \texttt{31.4} & \texttt{54.7} & \texttt{33.3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{21.8} & \texttt{16.9} & \texttt{32.6} \\
% & Ours (\texttt{MQ-Det}) & \texttt{(Close)} & \texttt{27.6} & \texttt{54.2} & \texttt{36.4} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Replace placeholders with official numbers.}
% \label{tab:results}
% \end{table}

% \noindent \textbf{Ablation and analysis (optional)}
% \begin{itemize}
%     \item Failure cases: \texttt{Without the pseudo-label generation module, due to a large number of unannotated instances in Dataset 2, the 5-shot and 10-shot scores of Dataset 2 drop to 17.9 and 18.1, respectively. The performance of Dataset 1 also decreases, resulting in a total score of only 109. However, the pseudo-label generation method currently used is overly simplistic and still introduces some incorrect labels.}
% \end{itemize}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{No}.
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{NTIRE 2026 is a highly valuable challenge in computer vision. It provides dedicated datasets, reliable baseline models, and standardized evaluation protocols for cross-domain few-shot object detection, offering a clear research direction and a fair comparison platform. It effectively guides participants to continuously improve their methods and promotes the advancement of related technologies}.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{The evaluation is limited by using only mAP, as practical detection tasks do not demand high IoU and only require approximate box placement. Thus, the scoring should focus more on detection correctness instead of high-IoU-based mAP}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{The datasets are stored on Google Drive for download, which frequently causes access limitations for users in China}.
% \end{itemize}

% %%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \begin{thebibliography}{1}

% \bibitem{fu2025cross}
% Fu, Y., Qiu, et al.
% \newblock NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.
% \newblock 2025 IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (CVPRW), 2025.

% \bibitem{groundingdino2024}
% Liu, Shilong, Zeng, Xingyi, et al.
% \newblock Grounding DINO: Marrying DINO with Grounded Pre-training for Open-Set Object Detection.
% \newblock \textit{18th European Conference on Computer Vision (ECCV 2024)}, 2025.

% \bibitem{meanteacher2017}
% Tarvainen, Antti, Valpola, Harri, et al.
% \newblock Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results.
% \newblock \textit{NIPS'17: Proceedings of the 31st International Conference on Neural Information Processing Systems}, 2017.
% \end{thebibliography}
% }

% % If you have a .bib file, comment thebibliography above and use:
% % {\small
% % \bibliographystyle{ieee_fullname}
% % \bibliography{egbib}
% % }

% \end{document}


==> ntire26/teams/team14_KLETech-CEVI/affiliation.tex <==
\clearpage
\subsection*{KLETech-CEVI}

\noindent\textit{\textbf{Title: }} Zero-Shot Transfer with GLIP and Multi-Scale Test-Time Augmentation\\

\noindent\textit{\textbf{Members: }} \\
Saiprasad Meesiyawar$^{3}$ (\href{mailto:saiprasad@cevi.co.in}{saiprasad@cevi.co.in}),\\
Ravi Kirasur$^{1,3}$ (\href{mailto:01fe23bcs233@kletech.ac.in}{01fe23bcs233@kletech.ac.in}),\\
Rakshita Kulkarni$^{1,3}$ (\href{mailto:01fe23bcs155@kletech.ac.in}{01fe23bcs155@kletech.ac.in}),\\
Bhoomi Deshpande$^{1,3}$ (\href{mailto:01fe23bcs145@kletech.ac.in}{01fe23bcs145@kletech.ac.in}),\\
Harsh Patil$^{1,3}$ (\href{mailto:01fe23bcs013@kletech.ac.in}{01fe23bcs013@kletech.ac.in}),\\
Uma Mudenagudi$^{2,3}$ (\href{mailto:uma@kletech.ac.in}{uma@kletech.ac.in})\\

\noindent\textit{\textbf{Affiliations: }} \\
$^1$School of Computer Science and Engineering, KLE Technological University, Hubballi, India\\
$^2$Department of Electronics and Communication Engineering, KLE Technological University, Hubballi, India\\
$^3$Center for Visual Intelligence (CEVI), Hubballi, India

==> ntire26/teams/team14_KLETech-CEVI/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{cvpr}
% \usepackage{times}
% \usepackage{graphicx}
% \usepackage{amsmath,amssymb}
% \usepackage{booktabs}
% \usepackage{hyperref}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{float}
% \cvprfinalcopy

% \title{Zero-Shot Transfer with GLIP and Multi-Scale Test-Time Augmentation}

% \author{
% Ravi Kirasur \quad Rakshita Kulkarni \quad Bhoomi Deshpande \quad Harsh Patil\\
% Saiprasad Meesiyawar \quad Nikhil Akalwadi \quad Ramesh Ashok Tabib \quad Uma Mudenagudi\\
% KLE Technological University, India
% }

% \begin{document}
% \maketitle

% \begin{abstract}
% Cross-Domain Few-Shot Object Detection (CD-FSOD) is a challenging problem requiring models to generalize to unseen domains with limited labeled data. We propose a pseudo-label driven vision-language grounding framework based on GLIP. The approach combines zero-shot detection with iterative adaptation using pseudo-labels. Additionally, multi-scale inference and loss refinement improve robustness and localization accuracy. Our method demonstrates strong improvements across multiple datasets under low-shot settings.
% \end{abstract}

% \section{Introduction}
% CD-FSOD requires detecting objects in unseen domains with minimal annotations. Domain shifts significantly degrade performance of conventional detectors.

% Vision-language models like GLIP provide strong semantic priors through large-scale pretraining. However, they suffer from localization inconsistencies when directly applied to new domains.

% To address this, we introduce a pseudo-label driven adaptation framework. Our approach leverages zero-shot grounding to generate pseudo-labels and iteratively refines them to improve domain-specific performance.

% \section{Related Work}
% Few-shot object detection has been widely explored using meta-learning, transfer learning, and fine-tuning approaches. However, most existing methods assume similar source and target domains.

% Vision-language models such as GLIP~\cite{li2022glip} and CLIP~\cite{radford2021clip} provide strong zero-shot capabilities. However, localization under domain shift remains a challenge.

% \section{Method}

% \subsection{Overview}
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\linewidth]{pipeline.png}
% \caption{Overview of the proposed pipeline.}
% \end{figure}

% The pipeline consists of:
% \begin{enumerate}
%     \item Zero-shot detection using GLIP
%     \item Pseudo-label generation
%     \item Iterative fine-tuning
% \end{enumerate}

% \subsection{Pseudo-Label Generation}
% \begin{equation}
% \hat{B} = \{ b_i \in B \mid s_i > \tau \}
% \end{equation}

% \subsection{Formal Training Objective}
% \begin{equation}
% \mathcal{L} = \mathcal{L}_{cls} + \lambda \mathcal{L}_{loc}
% \end{equation}

% \begin{equation}
% \mathcal{L}_{loc} = \mathcal{L}_{SmoothL1} + \beta \mathcal{L}_{GIoU}
% \end{equation}

% \subsection{Pseudo-Label Filtering}
% We apply confidence thresholding, NMS, and class-consistency filtering.

% \subsection{Multi-Scale Inference}
% Inference is performed at $\{640, 800, 1000\}$ resolutions with fusion.

% \begin{algorithm}[t]
% \caption{Pseudo-Label Driven Adaptation}
% \begin{algorithmic}[1]
% \STATE Initialize model $M$
% \FOR{each iteration}
% \STATE Generate predictions $B$
% \STATE Filter pseudo-labels $\hat{B}$
% \STATE Fine-tune model
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

% \section{Model Architecture}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\linewidth]{architecture.png}
% \caption{GLIP-based architecture.}
% \end{figure}

% \begin{itemize}
% \item Swin-L backbone~\cite{liu2021swin}
% \item GLIP text encoder
% \item DyHead detection head
% \end{itemize}

% \section{Training Details}

% \subsection{Datasets}
% We use Conceptual Captions, SBU Captions, Visual Genome~\cite{krishna2017vg}, MS COCO~\cite{lin2014coco}, and Objects365.

% \subsection{Loss Functions}
% Focal Loss~\cite{lin2017focal} and GIoU~\cite{rezatofighi2019giou} are used.

% \section{Results}

% \begin{table}[H]
% \centering
% \caption{Results (mAP)}
% \begin{tabular}{lccc}
% \toprule
% Method & ArTaxOr & Clipart1k & FISH \\
% \midrule
% Baseline (1-shot) & 14.88 & 13.58 & 11.23 \\
% Ours (1-shot) & 34.00 & 35.83 & 22.06 \\
% \midrule
% Baseline (5-shot) & 14.88 & 13.58 & 11.23 \\
% Ours (5-shot) & 35.10 & 37.20 & 23.45 \\
% \midrule
% Baseline (10-shot) & 14.88 & 13.58 & 11.23 \\
% Ours (10-shot) & 36.30 & 38.05 & 24.10 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\linewidth]{results.png}
% \caption{Qualitative results across datasets.}
% \end{figure}

% The proposed method significantly outperforms the baseline across all datasets and shot settings. In particular, the improvement in the 1-shot setting exceeds 2x, demonstrating the effectiveness of pseudo-label driven adaptation. The gains are consistent across both natural and synthetic domains, indicating strong cross-domain generalization capability.

% \subsection{Detailed Analysis}
% Performance improvements are consistent across datasets. ArTaxOr shows highest gains, while Clipart1k highlights robustness to style variation.

% \section{Ablation Study}
% To evaluate the contribution of individual components, we conduct ablation experiments.

% \begin{itemize}
%     \item \textbf{Pseudo-labeling:} Provides the largest improvement by enabling domain adaptation without manual annotations.
%     \item \textbf{Focal Loss:} Improves recall by focusing on hard examples.
%     \item \textbf{GIoU Loss:} Enhances localization accuracy, especially for irregular object shapes.
%     \item \textbf{Multi-scale Inference:} Improves robustness across varying object sizes.
% \end{itemize}

% These results confirm that each component contributes positively to the overall performance.


% \section{Discussion}
% The performance improvements observed across all datasets highlight the effectiveness of combining vision-language grounding with pseudo-label driven adaptation. The model benefits from strong semantic priors learned during large-scale pretraining, which enables robust zero-shot initialization.

% However, zero-shot predictions alone are insufficient for accurate localization under domain shifts. The introduction of pseudo-label based adaptation allows the model to progressively refine its predictions using target-domain specific signals. This leads to improved bounding box quality and classification accuracy.

% Multi-scale inference further enhances robustness by addressing scale variation in object sizes. The fusion of predictions across multiple resolutions reduces sensitivity to input scale and improves detection consistency.

% Overall, the synergy between semantic grounding and iterative adaptation is the key factor behind the observed performance gains.

% \section{Extended Analysis}

% \subsection{Impact of Domain Shift}
% We evaluate the robustness of the proposed method under varying domain shifts. The results indicate that the model maintains stable performance even when the target domain differs significantly in texture, style, and object appearance. This demonstrates the effectiveness of vision-language representations in capturing high-level semantics.

% \subsection{Effect of Shot Settings}
% The improvement is most significant in the 1-shot setting, where labeled data is extremely limited. This highlights the importance of pseudo-labeling in low-data regimes. As the number of shots increases, the performance gain gradually stabilizes, suggesting diminishing returns from additional supervision.

% \subsection{Error Analysis}
% We observe that most errors arise from:
% \begin{itemize}
%     \item Incorrect pseudo-labels in early iterations
%     \item Small object detection failures
%     \item Confusion between visually similar categories
% \end{itemize}

% These findings suggest that improving pseudo-label quality could further enhance performance.

% \section{Limitations}
% Despite strong performance, the proposed approach has several limitations.

% First, the method is highly dependent on the quality of pseudo-labels. Errors in early predictions may propagate during iterative fine-tuning, leading to suboptimal convergence.

% Second, the iterative adaptation process introduces additional computational overhead compared to purely zero-shot methods. This may limit scalability in large-scale applications.

% Third, the approach may struggle with rare categories where the semantic alignment between visual features and textual descriptions is weak.

% Finally, the choice of confidence threshold $\tau$ is critical. Improper threshold selection can either introduce noise or reduce training signal.

% \section{Future Work}
% Future work can focus on improving pseudo-label reliability through uncertainty estimation and confidence calibration techniques.

% Another promising direction is the integration of domain adaptation methods to explicitly handle distribution shifts between source and target domains.

% Additionally, exploring training-free adaptation strategies could reduce computational overhead while maintaining performance.

% Incorporating transformer-based detection heads and self-supervised learning techniques may further enhance representation quality and generalization.

% \section{Conclusion}
% We presented a GLIP-based pseudo-label driven framework for cross-domain few-shot object detection. By combining zero-shot grounding with iterative adaptation, the proposed method effectively bridges domain gaps and improves detection performance under low-shot settings.

% Extensive experiments demonstrate strong improvements across multiple datasets and shot configurations. The results highlight the importance of leveraging vision-language representations and pseudo-labeling for robust cross-domain generalization.

% Future work will focus on improving efficiency and pseudo-label quality to further enhance performance.

% \bibliographystyle{ieeenat_fullname}
% \bibliography{references}

% \end{document}

\subsection{KLETech-CEVI}

\subsubsection{Proposed Method}

The KLETech-CEVI team addresses Cross-Domain Few-Shot Object Detection (CD-FSOD) using a pseudo-label driven vision-language grounding framework built on GLIP. The approach leverages the strong semantic priors of vision-language models while mitigating their localization limitations under domain shift. As summmarized in Fig.~\ref{fig:cevi}, the overall pipeline consists of three stages:
\begin{enumerate}
    \item Zero-shot detection using GLIP
    \item Pseudo-label generation
    \item Iterative model adaptation via fine-tuning
\end{enumerate}

\begin{figure}[t]
\centering
\includegraphics[width=1.\linewidth]{teams/team14_KLETech-CEVI/pipeline.png}
\caption{Overview of the proposed pipeline.}
\label{fig:cevi}
\end{figure}

Given initial predictions $B$, high-confidence pseudo-labels are selected as:
\begin{equation}
\hat{B} = \{ b_i \in B \mid s_i > \tau \}
\end{equation}

The KLETech-CEVI team applies multiple filtering strategies to improve pseudo-label quality, including confidence thresholding, non-maximum suppression (NMS), and class-consistency filtering.

The model is then iteratively refined using the following objective:
\begin{equation}
\mathcal{L} = \mathcal{L}_{cls} + \lambda \mathcal{L}_{loc}
\end{equation}

\begin{equation}
\mathcal{L}_{loc} = \mathcal{L}_{SmoothL1} + \beta \mathcal{L}_{GIoU}
\end{equation}

This design improves both classification robustness and localization accuracy.

To further enhance performance, multi-scale test-time augmentation is applied at resolutions $\{640, 800, 1000\}$, and predictions are fused to improve robustness to object scale variation.

\begin{algorithm}[t]
\caption{Pseudo-Label Driven Adaptation}
\begin{algorithmic}[1]
\STATE Initialize model $M$
\FOR{each iteration}
\STATE Generate predictions $B$
\STATE Filter pseudo-labels $\hat{B}$
\STATE Fine-tune model
\ENDFOR
\end{algorithmic}
\end{algorithm}

As detailed in Fig.~\ref{fig:glip-framework}, the architecture is based on GLIP and includes:
\begin{itemize}
    \item Swin-L backbone~\cite{liu2021swin}
    \item GLIP text encoder~\cite{li2022glip}
    \item DyHead detection head
\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=1.\linewidth]{teams/team14_KLETech-CEVI/architecture.png}
\caption{GLIP-based architecture.}
\label{fig:glip-framework}
\end{figure}

The KLETech-CEVI team demonstrates that combining zero-shot grounding with iterative pseudo-label refinement effectively bridges domain gaps and significantly improves detection performance, especially under low-shot settings.

\subsubsection{Training Details}

The KLETech-CEVI team trains the model using large-scale vision-language datasets, including Conceptual Captions, SBU Captions, Visual Genome~\cite{krishna2017vg}, MS COCO~\cite{lin2014coco}, and Objects365.
For optimization, the following loss functions are employed:
\begin{itemize}
    \item Focal Loss~\cite{lin2017focal} for handling class imbalance and improving recall
    \item Generalized IoU (GIoU) Loss~\cite{rezatofighi2019giou} for enhanced localization accuracy
\end{itemize}

The iterative pseudo-labeling process plays a central role in training. High-confidence predictions are progressively incorporated as supervision, enabling domain adaptation without requiring additional manual annotations.
Experimental results show consistent improvements across multiple datasets and shot settings. In particular, the method achieves more than 2$\times$ improvement in the 1-shot scenario, demonstrating strong effectiveness in low-data regimes.
Ablation studies conducted by the KLETech-CEVI team indicate that:
\begin{itemize}
    \item Pseudo-labeling provides the largest performance gain
    \item Focal Loss improves detection of hard examples
    \item GIoU Loss enhances bounding box quality
    \item Multi-scale inference improves robustness to object size variation
\end{itemize}

Despite strong performance, the approach depends on pseudo-label quality and introduces additional computational overhead due to iterative fine-tuning. Performance may also degrade for rare categories with weak semantic alignment, and the confidence threshold $\tau$ requires careful tuning.
%
Overall, the training strategy effectively leverages vision-language priors and pseudo-label driven adaptation to achieve robust cross-domain generalization.


==> ntire26/teams/team15_Manifold/affiliation.tex <==
\subsection*{Manifold}
\noindent\textit{\textbf{Title: }} Multimodal Prompt-Driven Diffusion Augmentation (MPDA)\\
\noindent\textit{\textbf{Members: }} \\
Shuming Hu (\href{mailto:hsm123@nudt.edu.cn}{hsm123@nudt.edu.cn}),\\
Chao Chen (\href{mailto:cc_19@nudt.edu.cn}{cc\_19@nudt.edu.cn}),\\
Tao Wang (\href{mailto:wtt977193@163.com}{wtt977193@163.com})\\
\noindent\textit{\textbf{Affiliations: }} \\
National University of Defence Technology, China

==> ntire26/teams/team15_Manifold/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\-Multimodal Prompt-Driven Diffusion Augmentation (MPDA)-}

% \author{Shuming Hu\\
% National University of Defence Technology\\
% Changsha China, 410073\\
% {\tt\small hsm123@nudt.edu.cn}
% \and
% Chao Chen\\
% National University of Defence Technology\\
% Changsha China, 410073\\
% {\tt\small cc\_19@nudt.edu.cn}
% \and
% Tao Wang\\
% National University of Defence Technology\\
% Changsha China, 410073\\
% {\tt\small wtt977193@163.com}
% }

% \maketitle

% \section{Introduction}

% This factsheet presents our solution for the NTIRE 2026 Cross-Domain Few-Shot Object Detection (CD-FSOD) Challenge. In few-shot cross-domain object detection, models often overfit to specific background contexts due to the limited number of training samples. To address this issue, we propose a straightforward yet effective \textbf{VLM-Guided Generative Domain Expansion} framework.

% Unlike retrieval-based methods such as Domain-RAG, which rely on a large, predefined source-domain dataset, our approach is purely generative and does not require any source data. Specifically, we use the Qwen3-VL model to generate text descriptions of the scenes from the few-shot target images. Guided by these text prompts, we utilize the Flux.1 Fill diffusion model to repaint and generate new, diverse backgrounds. This inpainting process strictly preserves the original annotated foreground bounding boxes. Consequently, we can synthesize a large and highly diverse target-domain training set solely from the given few-shot samples.

% For the detection phase, we fine-tune the Grounding DINO framework (using a Swin-B backbone) on this augmented dataset. By combining generative background synthesis with a robust vision-language detector, our pipeline effectively bridges the domain gap and improves cross-domain detection performance.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{Manifold} - \texttt{15}\\



% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/open-mmlab/mmdetection}{mmdetection}\\
% \noindent Models / weights link: \href{'https://download.openmmlab.com/mmdetection/v3.0/grounding_dino/groundingdino_swinb_cogcoor_mmdet-55949c9c.pth' }{grounding dino},
% \href{'https://huggingface.co/Qwen/Qwen3-VL-8B-Instruct/tree/main' }{Qwen3-VL-8B-Instruct},
% \href{'https://huggingface.co/black-forest-labs/FLUX.1-Fill-dev' }{FLUX.1-Fill-dev}\\
% \noindent Reproduction instructions (brief): \texttt{see readme.txt}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: \texttt{Manifold}
% \item Team leader: \texttt{Shuming Hu}
% \item Affiliation / contact: \texttt{National University of Defence Technology, hsm123@nudt.edu.cn}
% \item Team members: \texttt{Chao Chen, Tao Wang}
% \item Sponsor affiliation (if any): \texttt{None / Describe here}
% \item Method name / nickname: \texttt{Multimodal Prompt-Driven Diffusion Augmentation (MPDA)}
% \item Final score (if available): \texttt{157.00}
% \end{itemize}

% \subsection{Method overview}
\subsection{Manifold}
\subsubsection{Proposed Method}

% (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams2026/team15_Manifold/fig1.png}{
%   \includegraphics[width=0.95\linewidth]{fig1.png}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }
% \caption{Overall pipeline of \texttt{Multimodal Prompt-Driven Diffusion Augmentation (MPDA)}. }
% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，便于维护和避免路径不一致
\def\figPath{teams/team15_Manifold/fig1.png}
\IfFileExists{\figPath}{
  % 加载与检查使用完全相同的路径，确保逻辑一致
  \includegraphics[width=1.\linewidth]{\figPath}
}{
  % 优化占位提示，明确图片应放置的正确路径和文件名
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{fig1.png} (or .pdf/.jpg) in \texttt{teams/team15_Manifold/} and check filename.
  }}
}
\caption{Overall pipeline of \texttt{Multimodal Prompt-Driven Diffusion Augmentation (MPDA)}. }
\label{fig:method15}
\end{figure}


\noindent \textbf{Key contributions:}
\begin{itemize}
  \item \textbf{Contribution 1:} They design a targeted data augmentation pipeline that utilizes Qwen3-VL for background prompt extraction and Flux.1 fill for background inpainting, significantly expanding the diversity of few-shot training samples while preserving accurate foreground bounding boxes.
  \item \textbf{Contribution 2:} They provide a strictly source-free alternative to retrieval-based methods like Domain-RAG; by relying entirely on generative synthesis rather than source-domain retrieval, their method eliminates the dependency on source datasets and avoids source-domain bias.
  \item \textbf{Contribution 3:} They successfully fine-tune Grounding DINO (Swin-B backbone) on the synthesized dataset, demonstrating that integrating diffusion-based background inpainting with vision-language detectors practically bridges the domain gap in cross-domain few-shot settings.
  \end{itemize}

\noindent \textbf{Model architecture}
% Describe the backbone, detector head, any added modules, and where they are inserted.
\begin{itemize}
    \item Backbone: Swin-B.
    \item Detector: Grounding DINO.
    \item Additional components: Qwen3-VL  and Flux.1 Fill , integrated as off-line generative data augmentation modules prior to the detection pipeline.
    \end{itemize}

\subsubsection{Training details}
% Provide training settings sufficient for reproduction.
\begin{itemize}
    \item Training data: The training is comprehensively conducted across three distinct target-domain datasets. For each dataset, they synthesize augmented training manifolds based entirely on the provided few-shot support sets using their generative background inpainting pipeline.
    \item Few-shot setting: They systematically evaluate their method under 1-shot, 5-shot, and 10-shot settings for all three datasets, culminating in 9 independent experimental configurations. The support selection strictly follows the official challenge splits.
    \item Optimization: Consistent across all 9 configurations, they use the AdamW optimizer (Initial LR = $1 \times 10^{-4}$, weight decay = $1 \times 10^{-4}$) with $L_2$ gradient clipping (max norm = 0.1). A layer-wise learning rate decay is applied (Swin-B backbone LR multiplier = 0.1)
    \item Augmentations: A robust spatial and color augmentation pipeline is applied, including CachedMosaic (prob=0.6, 640x640), YOLOXHSVRandomAug, RandomFlip (prob=0.5), CachedMixUp (prob=0.3), and Large-Scale Jittering (RandomChoice multi-scale resize between 480x1333 and 800x1333, coupled with absolute range RandomCrop).
    \item Hardware / runtime: All experiments were executed on a single NVIDIA RTX 4090 GPU (24GB VRAM). The training time for each of the 9 configurations is approximately 8 hours.
    \end{itemize}

\noindent \textbf{Inference details}
% Explain inference-time details that affect performance.
\begin{itemize}
    \item Test-time settings: {Grounding DINO default settings. Since test set annotations were unavailable for local validation, they saved multiple model checkpoints during the fine-tuning phase and generated inference results for each. Their final submission was determined by selecting the outputs that achieved the highest scores on the official evaluation server.}
    \item Ensemble / TTA: \texttt{None.}
    \item Any post-processing: \texttt{None.}
    \end{itemize}

% \subsection{Experimental results}
% Fill in your results. Replace dataset names with official ones used in the challenge.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & Baseline / Reference & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (\texttt{MPDA}) & \texttt{(Open)} & \texttt{29.31} & \texttt{33.91} & \texttt{33.40} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & Baseline / Reference & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (\texttt{MPDA}) & \texttt{(Open)} & \texttt{58.26} & \texttt{55.90} & \texttt{54.50} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & Baseline / Reference & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (\texttt{MPDA}) & \texttt{(Open)} & \texttt{21.78} & \texttt{34.00} & \texttt{40.60} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets.}
% \label{tab:results}
% \end{table}

% \subsection{Ablation and analysis (optional)}
% \begin{itemize}
%     \item Ablation 1: \texttt{(what you removed / changed, and the result)}
%     \item Ablation 2: \texttt{(what you removed / changed, and the result)}
%     \item Failure cases: \texttt{(brief description + optionally a figure)}
% \end{itemize}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{No}.
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{(\texttt{The NTIRE 2026 CD-FSOD challenge provides a highly valuable and rigorous benchmark for real-world few-shot detection. The domain shift setting effectively tests the robustness of modern vision-language models and encourages innovative approaches beyond traditional fine-tuning.})}.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{(none)}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{(none)}.
% \end{itemize}

%%%%%%%%% REFERENCES (self-contained, compilable placeholder)
%{\small
%\begin{thebibliography}{1}
%\bibitem{fu2025cross}
%Author(s).
%\newblock Paper title.
%\newblock Conference/Journal, Year. (Placeholder; replace with real references.)
%\end{thebibliography}
%}

% If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team17_NJUST-KMG/affiliation.tex <==
\subsection*{NJUST-KMG}
\noindent\textit{\textbf{Title: }} ASTER: A Hybrid Teacher-Guided Adaptation Framework for CD-FSOD\\
\noindent\textit{\textbf{Members: }} \\
Zhe Zhang$^{1\dagger}$ (\href{mailto:zhe.zhang@njust.edu.cn}{zhe.zhang@njust.edu.cn}),\\
Yang Yang$^{1}$ (\href{mailto:yyang@njust.edu.cn}{yyang@njust.edu.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\
$^1$Nanjing University of Science and Technology

==> ntire26/teams/team17_NJUST-KMG/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{cvpr}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}
% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\ASTER: A Hybrid Teacher-Guided Adaptation Framework for CD-FSOD}

% \author{
% Zhe Zhang\textsuperscript{1$\dagger$},
% Yang Yang\textsuperscript{1}\thanks{Corresponding Author}\\
% \textsuperscript{1}Nanjing University of Science and Technology\\
% {\tt\small zhe.zhang@njust.edu.cn},
% {\tt\small yyang@njust.edu.cn}
% }

% \maketitle

% \section{Introduction}
% This report presents \textbf{ASTER}, our solution for the NTIRE 2026 Cross-Domain Few-Shot Object Detection (CD-FSOD) challenge \cite{qiu2026ntire}. ASTER integrates two complementary paradigms: (i)~\textbf{FSOD-VFM} \cite{feng2026fsodvfm}, a training-free detector that leverages vision foundation models to establish a strong baseline from only a handful of support examples, and (ii)~\textbf{ETS} \cite{pan2025ets}, a trainable GroundingDINO-based detector equipped with strong augmentation and open-vocabulary priors.

% Our key observation is that the optimal branch varies with both the target domain and the shot regime. On dataset2, for instance, the training-free FSOD-VFM branch already achieves approximately 59--60 mAP in our local evaluation, surpassing direct ETS fine-tuning under sparse supervision. We attribute this to the extremely limited labeled examples and incomplete annotations in certain training images, both of which destabilize supervised optimization. Motivated by this finding, we employ FSOD-VFM not only as a standalone detector but also as a pseudo-label teacher for ETS. Furthermore, we leverage Domain-RAG \cite{li2025domainrag} to synthesize more diverse training samples, which proves particularly beneficial in the 1-shot regime. Our source code is available at \url{https://github.com/qianlanzz/NTIRE2026_CDFSOD}.

% \section{Factsheet Information}

% \subsection{Team Details}
% \begin{itemize}[leftmargin=1.5em]
% \item Team name: \texttt{NJUST-KMG}
% \item Team leader: \texttt{Zhe Zhang}
% \item Affiliation / contact: \texttt{Nanjing University of Science and Technology, zhe.zhang@njust.edu.cn}
% \item Team members: \texttt{Zhe Zhang, Yang Yang}
% \item Sponsor affiliation: \texttt{None}
% \item Method name / nickname: \texttt{ASTER}
% \item Final score: official hidden-test final score \texttt{191.4}; per-setting scores are reported in \Cref{tab:results}.
% \item Source code: \url{https://github.com/qianlanzz/NTIRE2026_CDFSOD}
% \end{itemize}
\subsection{NJUST-KMG}

\subsubsection{Proposed Method}
\noindent \textbf{High-level idea.}
ASTER is a hybrid framework built upon FSOD-VFM and ETS. The FSOD-VFM branch operates in a training-free manner: it generates category-agnostic proposals via UPN, refines regions with SAM2, extracts DINOv2 features, matches them against few-shot support prototypes, and suppresses duplicate detections through graph diffusion. The ETS branch provides a trainable counterpart based on GroundingDINO, Swin-B, and BERT, augmented with strong mixed-image strategies. To bridge the two branches, theyconvert high-confidence FSOD-VFM predictions on unlabeled target-domain images into pseudo annotations and continue training ETS for a few additional epochs. Additionally, Domain-RAG is employed to generate compositional target-domain samples, which is particularly effective in extremely low-shot settings.

\noindent \textbf{Key contributions:}
\begin{itemize}[leftmargin=1.5em]
\item \textbf{Strong training-free baseline:} FSOD-VFM provides a robust non-parametric starting point, reaching nearly 60 mAP on dataset2 in their local evaluation.
\item \textbf{Teacher-to-student adaptation:} High-confidence FSOD-VFM detections are converted into COCO-format pseudo annotations and incorporated into ETS training as supplementary supervision.
\item \textbf{Low-shot data diversification:} Domain-RAG augments appearance diversity, which is especially critical for 1-shot cases where target-domain coverage is most limited.
\end{itemize}
\noindent \textbf{Model Architecture}
\begin{itemize}[leftmargin=1.5em]
\item \textbf{FSOD-VFM branch:} UPN proposals + SAM2 masks + DINOv2 ViT-L/14 features + prototype matching + graph-diffusion score reweighting. For certain dataset3 settings, prototype refinement from high-confidence query predictions is additionally enabled.
\item \textbf{ETS branch:} GroundingDINO with a Swin-B backbone, BERT-base-uncased language encoder, 900 queries, the standard GroundingDINO encoder-decoder architecture, and class text prompts derived from target dataset categories.
\item \textbf{Hybrid bridge:} FSOD-VFM outputs are filtered by dataset-specific score thresholds to produce pseudo annotations, which are then concatenated with the real few-shot annotations for an additional stage of ETS fine-tuning.
\end{itemize}

\subsubsection{Training Details}
\begin{itemize}[leftmargin=1.5em]
\item \textbf{Training data:} Official challenge few-shot splits of dataset1, dataset2, and dataset3; pseudo annotations generated from FSOD-VFM predictions on unlabeled target-domain images; Domain-RAG synthetic samples merged into \texttt{*\_shot\_rag\_aug.json}.
\item \textbf{Few-shot setting:} 1-shot, 5-shot, and 10-shot. During pseudo-label continuation, real few-shot annotations are upsampled to prevent them from being overwhelmed by pseudo annotations. The repeat factors are 32 for dataset1, 64 for dataset2, and 32 for dataset3.
\item \textbf{Optimization:} The ETS baseline uses AdamW with a learning rate of \(1\times10^{-4}\), weight decay of \(1\times10^{-4}\), batch size 2, and gradient clipping at 0.1. Training schedules are dataset-specific: 30 epochs for dataset1 1/5-shot, 10 epochs for dataset1 10-shot, 7 epochs for dataset2, 25 epochs for dataset3 1-shot, and 20 epochs for dataset3 5/10-shot.
\item \textbf{Pseudo-label continuation:} ETS is initialized from the best baseline checkpoint and further fine-tuned for 4 epochs with a reduced learning rate of \(2\times10^{-5}\).
\item \textbf{Augmentations:} CachedMosaic, CachedMixUp, HSV jittering, random flip, multi-scale resize, and random crop are applied in the ETS training. Domain-RAG contributes additional compositional target-domain samples.
\item \textbf{Hardware / runtime:} All experiments are conducted on a single NVIDIA RTX 4090 GPU. FSOD-VFM is training-free, with computation primarily spent on proposal generation, mask extraction, and feature caching. ETS baseline training and pseudo-label fine-tuning share the same single-GPU setup.
\end{itemize}

\noindent \textbf{Inference Details}
\begin{itemize}[leftmargin=1.5em]
\item \textbf{FSOD-VFM:} DINOv2 ViT-L/14, SAM2 Large, UPN Large, 15 graph-diffusion steps, \(\alpha=0.3\), \(\lambda=0.5\). They retain 100 proposals by default, increasing to 200 for selected dataset2 and dataset3 settings, with a minimum proposal threshold of 0.01 or 0.005 depending on the dataset.
\item \textbf{Score fusion:} Class scores are computed from support prototypes, optionally fused with proposal confidence, and then reweighted via graph diffusion. For dataset3 1-shot and 10-shot, prototype refinement from high-confidence query predictions is additionally applied.
\item \textbf{ETS:} Inference uses the best checkpoint selected by local mAP. The detector retains up to 200 or 300 predictions per image depending on the dataset configuration.
\item \textbf{Final selection:} For each dataset-shot setting, they submit the best-performing branch among ETS baseline, ETS with FSOD-VFM pseudo labels, and ETS with Domain-RAG, determined by their local model-selection protocol.
\end{itemize}

% \subsection{Experimental Results}
% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & ETS baseline & Open & 33.0 & 54.8 & 21.6 \\
% & Ours (final) & Open & 35.6 & 60.4 & 40.1 \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & ETS baseline & Open & 40.8 & 50.1 & 42.0 \\
% & Ours (final) & Open & 47.5 & 60.5 & 42.0 \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & ETS baseline & Open & 40.2 & 50.8 & 44.5 \\
% & Ours (final) & Open & 46.2 & 61.1 & 44.5 \\
% \bottomrule
% \end{tabular}
% \caption{Official hidden-test mAP scores (\%) for our final submission. ETS baseline rows report local reference numbers obtained via the available validation/testval protocol. The official final score under the challenge formula is 191.4.}
% \label{tab:results}
% \end{table}

% \subsection{Ablation and Analysis}
% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3.5pt}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Case} & \textbf{FSOD-VFM} & \textbf{ETS} & \textbf{ETS+Pseudo} & \textbf{ETS+RAG} \\
% \midrule
% dataset2 1-shot & 59.2 & 54.8 & 60.4 & -- \\
% dataset2 5-shot & 59.1 & 50.1 & 60.5 & -- \\
% dataset2 10-shot & 59.0 & 50.8 & 61.1 & -- \\
% dataset3 1-shot & 18.0 & 21.6 & 27.5 & 40.0 \\
% dataset3 5-shot & 25.8 & 42.0 & 38.9 & 39.9 \\
% dataset3 10-shot & 28.2 & 44.5 & 41.8 & 44.3 \\
% \bottomrule
% \end{tabular}
% \caption{Representative local ablation results in mAP (\%). FSOD-VFM serves as a strong direct-inference teacher on dataset2; pseudo labels substantially boost ETS on dataset1 and dataset2, while Domain-RAG proves most beneficial in the 1-shot regime.}
% \label{tab:ablation}
% \end{table}

% \noindent \textbf{Main findings.}
% \begin{itemize}[leftmargin=1.5em]
% \item \textbf{FSOD-VFM is a strong teacher.} On dataset2, the training-free branch consistently achieves approximately 59 mAP across all shot settings, outperforming direct ETS fine-tuning. This confirms that strong foundation-model priors can be more reliable than supervised optimization when labels are extremely scarce.
% \item \textbf{Pseudo-label continuation yields the most consistent gains.} By converting FSOD-VFM detections into pseudo COCO annotations, ETS improves markedly on dataset1 and dataset2, with the largest gain observed on dataset2 10-shot: 50.8 \(\rightarrow\) 61.1.
% \item \textbf{Domain-RAG is most effective in the lowest-shot regime.} On dataset3 1-shot, Domain-RAG lifts ETS from 21.6 to 25.7 mAP. However, on 5-shot and 10-shot, the gains diminish or become slightly negative; we therefore apply it only when it improves local validation.
% \item \textbf{A substantial performance gap remains.} With full training annotations, our reproduced ETS upper bounds reach 61.0, 64.5, and 61.0 mAP on dataset1, dataset2, and dataset3, respectively, indicating that the few-shot regime remains heavily constrained by data sparsity and annotation quality.
% \end{itemize}

% \section{Other Details}
% \begin{itemize}[leftmargin=1.5em]
% \item Planned submission of a solution description paper at the NTIRE 2026 workshop: \texttt{Yes}.
% \item General comments and impressions: The challenge is practical and well-designed, as it simultaneously exposes two real-world difficulties: domain shift and annotation scarcity.
% \item Suggestions for future CD-FSOD challenges: It would be valuable to include an additional track or analysis focused on unlabeled target-domain adaptation, given that pseudo-label quality plays a central role in practice.
% \item Other comments: Dataset2 highlights an important issue in few-shot detection—training can be harmed by incomplete image-level annotations, whereas training-free foundation-model matching remains surprisingly robust.
% \end{itemize}

% {\small
% \begin{thebibliography}{10}

% \bibitem{qiu2026ntire}
% Xingyu Qiu, Yuqian Fu, Jiawei Geng, Bin Ren, Jiancheng Pan, Yanwei Fu, Radu Timofte, and others.
% \newblock NTIRE 2026 challenge on cross-domain few-shot object detection: methods and results.
% \newblock In \emph{CVPRW}, 2026.

% \bibitem{feng2026fsodvfm}
% Chen-Bin Feng, Youyang Sha, Longfei Liu, Yongjun Yu, Chi Man Vong, Xuanlong Yu, and Xi Shen.
% \newblock Few-Shot Object Detection with Vision Foundation Models and Graph Diffusion.
% \newblock In \emph{ICLR}, 2026.

% \bibitem{pan2025ets}
% Jiancheng Pan, Yanxing Liu, Xiao He, Long Peng, Jiahao Li, Yuze Sun, and Xiaomeng Huang.
% \newblock Enhance Then Search: An Augmentation-Search Strategy with Foundation Models for Cross-Domain Few-Shot Object Detection.
% \newblock In \emph{CVPRW}, 2025.

% \bibitem{li2025domainrag}
% Yu Li, Xingyu Qiu, Yuqian Fu, Jie Chen, Tianwen Qian, Xu Zheng, Danda Pani Paudel, Yanwei Fu, Xuanjing Huang, Luc Van Gool, and others.
% \newblock Domain-RAG: Retrieval-Guided Compositional Image Generation for Cross-Domain Few-Shot Object Detection.
% \newblock In \emph{NeurIPS}, 2025.

% \end{thebibliography}
% }

% \end{document}


==> ntire26/teams/team18_earth-insights/affiliation.tex <==
\subsection*{earth-insights}
\noindent\textit{\textbf{Title:} earth-insights}\\
\noindent\textit{\textbf{Members: }} \\
Kaiyu Li$^1$ (\href{mailto:likyoo.ai@gmail.com}{likyoo.ai@gmail.com}),\\
Bowen Fu$^1$ (\href{mailto:happybug@stu.xjtu.edu.cn}{happybug@stu.xjtu.edu.cn}),\\
Zixuan Jiang$^1$ (\href{mailto:andrewjiang@stu.xjtu.edu.cn}{andrewjiang@stu.xjtu.edu.cn}),\\
Ke Li$^2$ (\href{mailto:like0413@stu.xidian.edu.cn}{like0413@stu.xidian.edu.cn}),\\
Hui Qiao$^3$ (\href{mailto:qiaoh@chinatelecom.cn}{qiaoh@chinatelecom.cn}),\\
Xiangyong Cao$^1$ (\href{mailto:caoxiangyong@mail.xjtu.edu.cn}{caoxiangyong@mail.xjtu.edu.cn})\\
\noindent\textit{\textbf{Affiliations:}} \\
$^1$Xi’an Jiaotong University\\
$^2$Xidian University\\
$^3$China Telecom Shaanxi Branch

==> ntire26/teams/team18_earth-insights/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\-Team earth-insights Method-}

% \author{Kaiyu Li$^{*}$\\
% Xi’an Jiaotong University\\
% Xi'an, China\\
% {\tt\small likyoo.ai@gmail.com}
% \and
% Bowen Fu$^{*}$\\
% Xi’an Jiaotong University\\
% Xi'an, China\\
% {\tt\small HappyBug@stu.xjtu.edu.cn}
% \and
% Zixuan Jiang\\
% Xi’an Jiaotong University\\
% Xi'an, China\\
% {\tt\small andrewjiang@stu.xjtu.edu.cn}
% \and
% Ke Li\\
% Xidian University\\
% Xi'an, China\\
% {\tt\small like0413@stu.xidian.edu.cn}
% \and
% Hui Qiao\\
% China Telecom Shaanxi Branch\\
% Xi'an, China\\
% {\tt\small qiaoh@chinatelecom.cn}
% \and
% Jiang Liu\\
% China Telecom Artificial Intelligence Technology Co., Ltd\\
% Beijing, China\\
% {\tt\small liuj67@chinatelecom.cn}
% \and
% Hao Sun\\
% China Telecom Artificial Intelligence Technology Co., Ltd\\
% Beijing, China\\
% {\tt\small sunh10@chinatelecom.cn}
% \and
% Xiangyong Cao$^{\dag}$\\
% Xi’an Jiaotong University\\
% Xi'an, China\\
% {\tt\small caoxiangyong@mail.xjtu.edu.cn}
% }

% \maketitle

% \section{Main Open-Source Track Methods}

\subsection{Earth-insights}

\subsubsection{Proposed Method}
To tackle the CD-FSOD task under the open-source setting, this team proposes a data-centric fine-tuning pipeline (Fig.~\ref{fig:earth_insights}) built upon powerful foundation models, specifically SAM3~\cite{carion2025sam} and Grounding DINO~\cite{liu2024grounding}. Recognizing that the quality and diversity of the support set are bottlenecks in few-shot scenarios, the proposed method focuses on more complete pseudo-label generation, targeted data synthesis, and dataset-specific adaptation strategies. 
The overall pipeline consists of the following key steps:

\noindent
\textbf{High-Quality Support Label Generation.} To maximize the utility of the limited support set, this team leverages the zero-shot capabilities of SAM3 and Grounding DINO. Some prompt engineering is applied to extract accurate initial bounding boxes. For instance, in the parking lot dataset (Carpk), specific textual prompts such as ``school bus'' or ``black car'' are utilized to guide the foundation models effectively. To refine these initial predictions, the Weighted Boxes Fusion (WBF)~\cite{solovyev2021weighted} algorithm, along with carefully designed post-processing techniques, is employed to ensemble the results, yielding more complete support labels for subsequent training.

\noindent
\textbf{Object-Centric Mosaic and Augmentation.} Since the generated labels may still contain imperfections and the support samples are extremely scarce, this team introduces an ``Object-Centric Mosaic'' data synthesis strategy. Instead of randomly cropping images for the standard Mosaic augmentation~\cite{bochkovskiy2020yolov4}, this approach specifically crops regions surrounding the annotated targets. This ensures that the synthesized samples maintain high information density and context relevance. Additional standard data augmentations are also incorporated to further expand sample diversity and alleviate overfitting.

\noindent
\textbf{Dataset-Specific Strategy and Validation.} The team observed a high variance in training results due to sample scarcity. Following~\cite{pan2025enhance}, an optimized target domain validation set is constructed to monitor the training process and select the best checkpoints. Furthermore, empirical results revealed that the native SAM3 exhibits significantly different adaptation capabilities across various datasets. For example, on the Carpk, which predominantly contains small cars, SAM3 achieves a zero-shot mAP of over 50\%. Conversely, on the CarDD, which features objects with ambiguous boundaries (\textit{e.g.}, ``scratch''), the zero-shot mAP drops below 10\%. Consequently, the specific data processing and augmentation strategies are dynamically adjusted based on the object attribute and zero-shot performance characteristics of each specific dataset.


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{
% teams/team18_earth-insights/images/earth_insights.pdf}
%     \caption{Team earth-insights: overview of the training process.}
%     \label{fig:earth_insights}
% \end{figure}
\begin{figure}
    \centering
    \def\figPath{teams/team18_earth-insights/images/earth_insights.pdf}
    \IfFileExists{\figPath}{
        \includegraphics[width=\linewidth]{\figPath}
    }{
        \fbox{\parbox[c][0.22\textheight][c]{\linewidth}{
        \centering \textbf{Figure Placeholder (earth-insights)}\\
        Put \texttt{earth_insights.pdf} (or .png/.jpg) in \texttt{teams/team18_earth-insights/images/} and check filename.
        }}
    }
    \caption{Team earth-insights: overview of the training process.}
    \label{fig:earth_insights}
\end{figure}

\subsubsection{Training Details}

The proposed method uses SAM3 as the primary foundation model for the fine-tuning stage. To maintain training efficiency within a limited timeframe, the team utilized the default SAM3 fine-tuning script, wherein only the parameters of the text encoder are updated while other parts remain frozen. This team encourages future participants to explore more comprehensive parameter-efficient fine-tuning schemes for SAM3. All experiments are conducted on a single NVIDIA A100 GPU. During the training phase, strict adherence to the few-shot protocol is maintained; no external data is used other than the provided support set images and the pre-trained weights of the foundation models. 


\noindent
\textbf{Additional Explorations:} For the underwater dataset scenarios, this team also experimented with an underwater-specific open-vocabulary segmentation model~\cite{li2025maris} to bridge the distinct domain gap. Although these results were not included in the final submission due to time constraints, further exploration is valuable in future research.

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - \texttt{TEAM\_ID}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{TEAM\_NAME}
%     \item Team leader (contact): \texttt{NAME}, \texttt{EMAIL}
%     \item Team members: \texttt{MEMBER\_1, MEMBER\_2, ...}
%     \item Method name / nickname: \texttt{METHOD\_NAME}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/your_repo}{https://github.com/your\_repo}\\
% \noindent Models / weights link: \href{https://example.com}{https://example.com}\\
% \noindent Reproduction instructions (brief): \texttt{(e.g., bash run.sh / python test.py ...)}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: \texttt{TEAM\_NAME}
% \item Team leader: \texttt{LEADER\_NAME}
% \item Affiliation / contact: \texttt{AFFILIATION, PHONE (optional), EMAIL}
% \item Team members: \texttt{MEMBER\_1, MEMBER\_2, ...}
% \item Sponsor affiliation (if any): \texttt{None / Describe here}
% \item Method name / nickname: \texttt{METHOD\_NAME}
% \item Final score (if available): \texttt{SCORE}
% \item Submission link: \texttt{LINK}
% \end{itemize}

% \subsection{Method overview}
% % (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{method_figure.pdf}{
%   \includegraphics[width=0.95\linewidth]{method_figure.pdf}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }
% \caption{Overall pipeline of \texttt{METHOD\_NAME}. Replace with your own figure and caption.}
% \label{fig:method}
% \end{figure}

% \noindent \textbf{High-level idea:} Briefly summarize your method in 3--6 sentences.\\
% \noindent \textbf{Key contributions:}
% \begin{itemize}
%     \item \textbf{Contribution 1:} \texttt{(one sentence)}
%     \item \textbf{Contribution 2:} \texttt{(one sentence)}
%     \item \textbf{Contribution 3 (optional):} \texttt{(one sentence)}
% \end{itemize}

% \subsection{Model architecture}
% Describe the backbone, detector head, any added modules, and where they are inserted.
% \begin{itemize}
%     \item Backbone: \texttt{(e.g., ResNet-50, Swin-T, ViT-B, etc.)}
%     \item Detector: \texttt{(e.g., Faster R-CNN / Deformable DETR / etc.)}
%     \item Additional components: \texttt{(e.g., prototype module, attention, adapter, etc.)}
% \end{itemize}

% \subsection{Training details}
% Provide training settings sufficient for reproduction.
% \begin{itemize}
%     \item Training data: \texttt{(dataset names / splits)}
%     \item Few-shot setting: \texttt{(1/5/10-shot, support selection strategy)}
%     \item Optimization: \texttt{(optimizer, LR, schedule, batch size, epochs/iters)}
%     \item Augmentations: \texttt{(list)}
%     \item Hardware / runtime: \texttt{(GPU type, \#GPUs, training time)}
% \end{itemize}

% \subsection{Inference details}
% Explain inference-time details that affect performance.
% \begin{itemize}
%     \item Test-time settings: \texttt{(image size, NMS, score threshold, etc.)}
%     \item Ensemble / TTA: \texttt{(if used)}
%     \item Any post-processing: \texttt{(if used)}
% \end{itemize}

% \subsection{Experimental results}
% Fill in your results. Replace dataset names with official ones used in the challenge.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & Baseline / Reference & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (\texttt{METHOD\_NAME}) & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & Baseline / Reference & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (\texttt{METHOD\_NAME}) & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & Baseline / Reference & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (\texttt{METHOD\_NAME}) & \texttt{(Close/Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Replace placeholders with official numbers.}
% \label{tab:results}
% \end{table}

% \subsection{Ablation and analysis (optional)}
% \begin{itemize}
%     \item Ablation 1: \texttt{(what you removed / changed, and the result)}
%     \item Ablation 2: \texttt{(what you removed / changed, and the result)}
%     \item Failure cases: \texttt{(brief description + optionally a figure)}
% \end{itemize}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{Yes/No}.
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{(text)}.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{(text)}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{(text)}.
% \end{itemize}

% %%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \begin{thebibliography}{1}
% \bibitem{fu2025cross}
% Author(s).
% \newblock Paper title.
% \newblock Conference/Journal, Year. (Placeholder; replace with real references.)
% \end{thebibliography}
% }

% If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team20_CDiscover/affiliation.tex <==
\subsection*{CDiscover}
\noindent\textit{\textbf{Title: }} GiPL-Grounding: Generative augmented iterative Pseudo-Labeling for Grounding\\
\noindent\textit{\textbf{Members: }} \\
Jiacong Liu$^{1}$ (\href{mailto:m202574174@hust.edu.cn}{m202574174@hust.edu.cn}),\\
Shu Luo$^{1}$ (\href{mailto:luoshu_hust@hust.edu.cn}{luoshu\_hust@hust.edu.cn}),\\
Yikai Qin$^{1}$ (\href{mailto:yikaiq@hust.edu.cn}{yikaiq@hust.edu.cn}),\\
Yaze Zhao$^{1}$ (\href{mailto:zyaz@hust.edu.cn}{zyaz@hust.edu.cn}),\\
Yongwei Jiang$^{1}$ (\href{mailto:jiangyongwei@hust.edu.cn}{jiangyongwei@hust.edu.cn}),\\
Yixiong Zou$^{1}$ (\href{mailto:yixiongz@hust.edu.cn}{yixiongz@hust.edu.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\
$^1$Huazhong University of Science and Technology

==> ntire26/teams/team20_CDiscover/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}
% \usepackage{array}       % 自定义列格式
% \usepackage{siunitx}     % 数值对齐（可选，用于小数点对齐）

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\GiPL-Grounding: Generative augmented iterative Pseudo-Labeling for Grounding}

% \author{Jiacong Liu \quad Shu Luo \quad Yikai Qin \quad Yaze Zhao \quad Yongwei Jiang \quad Yixiong Zou \\
% Huazhong University of Science and Technology \\
% {\tt\small \{m202574174, luoshu\_hust, yikaiq, zyaz, jiangyongwei, yixiongz\}@hust.edu.cn}
% }



% % \author{
% % Jiacong Liu$^{1}$ \quad Shu Luo$^{2}$ \quad Yikai Qin$^{2}$ \quad Yaze Zhao$^{1}$ \quad Yongwei Jiang$^{1}$ \quad Yixiong Zou$^{1}$ \\
% % $^{1}$School of Computer Science and Technology, Huazhong University of Science and Technology \\
% % $^{2}$School of Software, Huazhong University of Science and Technology \\
% % % {\tt\small \{m202574174, zyaz, jiangyongwei, yixiongz\}@hust.edu.cn \quad \{luoshu\_hust, yikaiq\}@hust.edu.cn}
% % {\tt\small \{m202574174, luoshu\_hust, yikaiq, zyaz, jiangyongwei, yixiongz\}@hust.edu.cn} 
% % }

% % % 共同第一单位
% % \author{
% % Jiacong Liu$^{1}$ \quad Shu Luo$^{1}$ \quad Yikai Qin$^{1}$ \quad Yaze Zhao$^{1}$ \quad Yongwei Jiang$^{1}$ \quad Yixiong Zou$^{1}$ \\
% % $^{1}$Huazhong University of Science and Technology \\
% % {\tt\small \{m202574174, luoshu\_hust, yikaiq, zyaz, jiangyongwei, yixiongz\}@hust.edu.cn}
% % }


% % \author{
% % Jiacong Liu$^{1}$ \quad Shu Luo$^{2}$ \quad Yikai Qin$^{2}$ \quad Yaze Zhao$^{1}$ \quad Yongwei Jiang$^{1}$ \quad Yixiong Zou$^{1}$ \\
% % $^{1}$School of Computer Science and Technology, Huazhong University of Science and Technology \\
% % $^{2}$ School of Sofware Engineering, Huazhong University of Science and Technology \\
% % {\tt\small \{m202574174, luoshu\_hust, yikaiq, zyaz, jiangyongwei, yixiongz\}@hust.edu.cn}
% % }


% \maketitle

% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - \texttt{TEAM\_ID}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{TEAM\_NAME}
%     \item Team leader (contact): \texttt{NAME}, \texttt{EMAIL}
%     \item Team members: \texttt{MEMBER\_1, MEMBER\_2, ...}
%     \item Method name / nickname: \texttt{METHOD\_NAME}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/z-yaz/CDiscover}{github.com/z-yaz/CDiscover}\\
% \noindent Models / weights link: \href{https://pan.baidu.com/s/1r5H8TsV1qgwuWPuvc1EJZQ?pwd=hg8e}{models and weights}\\
% \noindent Reproduction instructions (brief): \href{https://github.com/z-yaz/CDiscover}{README}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: CDiscover
% \item Team leader: Yixiong Zou
% \item Affiliation / contact: Huazhong
% University of Science and Technology
% \item Team members: Jiacong Liu, Shu Luo, Yikai Qin, Yaze Zhao, Yongwei Jiang
% % , Yixiong Zou
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \textbf{GiPL-Grounding} (Generative augmented iterative Pseudo-Labeling for Grounding)
% \item Final score (if available): 192.7929
% \item Submission link: \href{https://github.com/z-yaz/CDiscover}{github.com/z-yaz/CDiscover} 
% \end{itemize}

\subsection{CDiscover}

\subsubsection{Proposed Method}
% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.95\linewidth]{teams/team20_CDiscover/pdf/framework.pdf} % 替换为你的实际文件名
% \caption{Proposed framework for CDFSOD. 
% Branch 1 iteratively refines GLIP with pseudo labels, while Branch 2 uses Qwen image generation to augment training data for Grounding DINO.}
% \label{fig:framework}
% \end{figure}

Their method addresses the CDFSOD challenge through a domain-adaptive hybrid strategy, as illustrated in Fig.~\ref{fig:framework5}. For Dataset 1\&3, they leverage the Qwen\cite{wu2025qwen} to synthesize generative data, enriching the feature space for GroundingDINO \cite{liu2024grounding}. For Dataset 2 (a multi-object natural domain with vehicles), they identify that only a single instance is labeled per image despite the presence of multiple targets. To prevent the model from treating unlabeled vehicles as background, they employ a GLIP\cite{li2022grounded}-based pseudo-labeling pipeline to recover missing annotations, followed by iterative self-training to achieve dense and robust object localization.\\

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.\linewidth]{teams/team20_CDiscover/pdf/framework.pdf} % 替换为你的实际文件名
\caption{Proposed framework for CDFSOD. 
Branch 1 iteratively refines GLIP with pseudo labels, while Branch 2 uses Qwen image generation to augment training data for Grounding DINO.}
\label{fig:framework5}
\end{figure}


\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} They introduce a generative augmentation pipeline using Qwen to synthesize domain-specific training samples, effectively mitigating the data scarcity issue in CDFSOD.
    \item \textbf{Contribution 2:} They develop an iterative self-training framework based on GLIP and a robust pseudo-label filtering mechanism to enhance model adaptation in complex target distributions.
\end{itemize}

They utilize two vision-language foundation models, selecting the optimal architecture based on the target domain's attributes. In detail, for Dataset 1 and 3, they utilize GroundingDINO, while for Dataset 2, they employ GLIP.
\begin{itemize}
    \item Backbone: The GLIP-L variant is used, which incorporates Swin-L\cite{liu2021swin} as the visual encoder and BERT\cite{devlin2019bert}. For Grounding DINO, the Swin-B\cite{liu2021swin} backbone is used as the visual encoder and BERT from Hugging Face as the text encoder.
    \item Detector: Grounding DINO follows a DETR-style\cite{carion2020end} detection paradigm with a Transformer encoder-decoder architecture. In contrast, GLIP adopts a two-stage detector, consisting of a Region Proposal Network (RPN)\cite{ren2015faster} and ROI heads for region-level prediction.
\end{itemize}

\subsubsection{Training details}
\begin{itemize}
    \item Training data: GLIP is pre-trained on FourODs\cite{krizhevsky2012imagenet,krishna2017visual,kuznetsova2020open}, GoldG\cite{kamath2021mdetr}, CC3M+12M, and SBU\cite{ordonez2011im2text}, while GroundingDINO is pre-trained on a larger and more diverse set of datasets, including COCO\cite{lin2014microsoft}, Objects365\cite{shao2019objects365}, GoldG, Cap4M, OpenImages\cite{kuznetsova2020open}, ODinW-35\cite{li2022elevater}, and RefCOCO\cite{kamath2021mdetr}.
    % \item Few-shot setting: They strictly follow the official challenge protocol. Specifically, each dataset is evaluated under three few-shot settings, i.e., 1-shot, 5-shot, and 10-shot, where only the provided support annotations of the corresponding shot setting are used for adaptation/training. 
    % % Since our GLIP-based pipeline is applied only to Dataset~2, 
    % % The few-shot experiments in this part are conducted under the official Dataset~2 split and submission setting defined by the challenge (\href{https://www.codabench.org/competitions/12873/}{Codabench Challenge Page}). 
    % The few-shot experiments are conducted by adaptively deploying GLIP for Dataset 2 and GroundingDINO for Dataset 1 \& 3, following the official submission settings defined by the \href{https://www.codabench.org/competitions/12873/}{challenge}.
    \item Optimization: For Dataset 2, they fine-tune GLIP-L initialized from the publicly available \texttt{glip\_large\_model.pth} checkpoint. The learning rate is set to $5\times10^{-5}$, the weight decay is $0.05$, and the batch size is 2. They disable AMP and adopt the default GLIP fine-tuning framework with AutoStep scheduling. The step patience is set to 3 and the auto-termination patience is set to 6. The model is trained for 200 epochs, and the random seed is fixed to 10 for reproducibility. Datasets 1 and 3 are trained on a single NVIDIA A6000 GPU, with 50 training epochs and a fixed batch size of 4. The model architecture is built upon the Grounding DINO framework, with core parameters and module configurations as follows: the default number of queries is 900, and the maximum text token length is set to 256; the text encoder adopts a BERT-based structure equipped with BPE tokenization; both the feature enhancer and cross-modality decoder are stacked with 6 layers, and a deformable attention mechanism is introduced in the image cross-attention module to improve feature extraction accuracy. The loss function consists of classification (or contrastive) loss, box L1 loss, and GIoU loss. Following the settings of the original framework, the Hungarian matching weights are set to 2.0 for classification loss, 5.0 for L1 loss, and 2.0 for GIoU loss, while the final total loss weights are correspondingly set to 1.0, 5.0, and 2.0. In addition, They employ a data augmentation strategy that uses a large model to generate samples from the support set for training.  
    \item Augmentations: They augment the support set using a vision-language model (Qwen-image-2.0-pro)\cite{wu2025qwen}. Specifically, given each support image, Qwen is used to generate semantically consistent variations. These synthesized samples effectively enrich the limited support set and improve generalization in few-shot settings.
    \item Hardware / runtime: 2 × Nvidia A6000
\end{itemize}

\noindent \textbf{Inference details.}
Explain inference-time details that affect performance.
\begin{itemize}
    \item Test-time settings: During inference, the detector is applied in a standard single-model setting without test-time augmentation. Since the task is object detection, non-maximum suppression (NMS) is used to remove highly overlapped predictions and retain the most confident bounding boxes. They follow the default inference pipeline of the corresponding detector framework for prediction filtering and box selection.
    \item Ensemble / TTA: None
    \item Any post-processing: None
\end{itemize}

% \subsection{Experimental results}
% Main results are shown as Table \ref{tab:results}.

% % \begin{table}[t]\scriptsize
% % \centering
% % \begin{tabular}{clcccc}
% % \toprule
% % & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% % \midrule
% % \multirow{2}{*}{\rotatebox{90}{1-shot}}
% % & GroundingDINO & \texttt{(Open)} & \texttt{31.5} & \texttt{35.8} & \texttt{34.6} \\
% % & Ours (GiPL) & \texttt{(Open)} & \texttt{34.6} & \texttt{41.2} & \texttt{42.1} \\
% % \midrule
% % \multirow{2}{*}{\rotatebox{90}{5-shot}}
% % & GroundingDINO & \texttt{(Open)} & \texttt{49} & \texttt{42} & \texttt{40} \\
% % & Ours (GiPL) & \texttt{(Open)} & \texttt{63.3} & \texttt{63} & \texttt{61.3} \\
% % \midrule
% % \multirow{2}{*}{\rotatebox{90}{10-shot}}
% % & GroundingDINO & \texttt{(Open)} & \texttt{34.2} & \texttt{43.8} & \texttt{47} \\
% % & Ours (GiPL) & \texttt{(Open)} & \texttt{35.9} & \texttt{44.6} & \texttt{48} \\
% % \bottomrule
% % \end{tabular}
% % \caption{Results under 1/5/10-shot settings on three target datasets. Replace placeholders with official numbers.}
% % \label{tab:results}
% % \end{table}

% % 先确保导入了必要的包（如果没导入的话）

% \begin{table}[t]
% \setlength{\tabcolsep}{6pt}  % 调整列间距（默认过宽）
% \renewcommand{\arraystretch}{1.2}  % 增加行间距，更易读
% \scriptsize  % 保持字号，如需更大可改为 \small
% \centering
% \begin{tabular}{@{}c l c S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] @{}}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\makebox[1em]{1-shot}}}  % 旋转文字居中对齐
% & GroundingDINO & \texttt{(Open)} & 31.5 & 49.0 & 34.2 \\
% & Ours (GiPL)   & \texttt{(Open)} & 34.6 & 63.3 & 39.7 \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\makebox[1em]{5-shot}}}
% & GLIP & \texttt{(Open)} & 35.8 & 42.0 & 43.8 \\  % 补0统一小数位数
% & Ours (GiPL)   & \texttt{(Open)} & 41.2 & 63.0 & 47.4 \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\makebox[1em]{10-shot}}}
% & GroundingDINO & \texttt{(Open)} & 34.6 & 40.0 & 47.0 \\
% & Ours (GiPL)   & \texttt{(Open)} & 42.1 & 61.3 & 48.3 \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. }
% \label{tab:results}
% \end{table}

% \subsection{Ablation and analysis (optional)} None

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{Yes}.
% \item General comments and impressions of the NTIRE 2026 challenge: 
% \texttt{Good}. 
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): 
% \texttt{None}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: 
% \texttt{None}.
% \end{itemize}




% % If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team21_QiFans/affiliation.tex <==
  \subsection*{QiFans}
  \noindent\textit{\textbf{Title: }} GDino-FT: Domain-Adaptive GroundingDINO with Prompt Engineering and Few-Shot Fine-Tuning\\
  \noindent\textit{\textbf{Members: }} \\
  Wei Zhou$^{1}$ (\href{mailto:weichow@u.nus.edu}{weichow@u.nus.edu})\\
  Qi Xu$^{2}$ (\href{mailto:txxqsh@gmail.com}{txxqsh@gmail.com})\\
  \noindent\textit{\textbf{Affiliations: }} \\
  $^{1}$National University of Singapore \\
  $^{2}$Shanghai Jiao Tong University

==> ntire26/teams/team21_QiFans/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\-GDino-FT: Domain-Adaptive GroundingDINO with Prompt Engineering and Few-Shot Fine-Tuning-}

% \author{Wei Zhou\\
% National University of Singapore\\
% Singapore\\
% {\tt\small weichow@u.nus.edu}
% \and
% Qi Xu\\
% Shanghai Jiao Tong University\\
% Shanghai, China\\
% {\tt\small txxqsh@gmail.com}
% }

% \maketitle

% \section{Introduction}

% This factsheet describes the solution of Team \textbf{QiFans} for the NTIRE 2026 Challenge on Cross-Domain Few-Shot Object Detection (CD-FSOD). Our approach, \textbf{GDino-FT}, leverages GroundingDINO~\cite{liu2023grounding} as the foundation model with a domain-adaptive strategy: zero-shot detection with optimized text prompts for domains with common objects, and few-shot fine-tuning for specialized fine-grained domains. This combination achieves a final score of \textbf{155.42} on the test leaderboard.

% The factsheet, source codes, and trained models are sent to all NTIRE 2026 challenge organizers by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - QiFans - 21\\

% \noindent Body contents:
% \begin{enumerate}[a)]
%     \item Team name: QiFans
%     \item Team leader (contact): Wei Zhou, weichow@u.nus.edu
%     \item Team members: Wei Zhou, Qi Xu
%     \item Method name: GDino-FT
%     \item Code, pre-trained model, and factsheet download link:\\
%     \url{https://drive.google.com/drive/folders/1d162JfipZgH-2MfIW8l9dEKFT7m8eKzT}
% \end{enumerate}

% \section{Code Submission}
% \noindent Code link: \url{https://drive.google.com/drive/folders/1d162JfipZgH-2MfIW8l9dEKFT7m8eKzT}\\
% \noindent Models / weights: Included in the above link (checkpoints/)\\
% \noindent Reproduction instructions:
% \begin{verbatim}
% # 1. Zero-shot inference (D1, D2)
% python gdino_inference_v3.py --gpu 0

% # 2. Fine-tune D3 on 10-shot support set
% python finetune_gdino.py --dataset_id 3 \
%   --shot 10 --epochs 200 --gpu 0

% # 3. Inference with fine-tuned D3
% python finetune_gdino.py --dataset_id 3 \
%   --shot 10 --epochs 0 --gpu 0 \
%   --checkpoint best_model.pth \
%   --inference_only --box_threshold 0.1

% # 4. Assemble submission
% python prepare_submission.py
% \end{verbatim}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: QiFans
% \item Team leader: Wei Zhou
% \item Affiliation / contact: National University of Singapore, weichow@u.nus.edu
% \item Team members: Wei Zhou (NUS), Qi Xu (SJTU)
% \item Sponsor affiliation: None
% \item Method name: GDino-FT (GroundingDINO Fine-Tune)
% \item Track: Main (open-source, uses GroundingDINO pretrained on Objects365+GoldG+Cap4M)
% \item Final score: \textbf{155.42}
% \item CodaBench username: \texttt{weichow}
% \end{itemize}

% \subsection{Method overview}
\subsection{QiFans}
\subsubsection{Proposed Method}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.95\linewidth]{teams/team21_QiFans/
% images/pipeline.pdf}
% \caption{Overall pipeline of GDino-FT. For D1 (underwater) and D2 (car), we use pretrained GroundingDINO with optimized text prompts (zero-shot). For D3 (car damage), we fine-tune the model on the 10-shot support set while freezing the BERT text encoder.}
% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 1. 修复路径换行问题 + 增加文件存在性检查（避免图片缺失时报错）
% 2. 统一路径变量，提升可维护性
\def\figPath{teams/team21_QiFans/images/pipeline.pdf}
\IfFileExists{\figPath}{
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  % 占位框：明确提示图片缺失时的解决方案
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{pipeline.pdf} (or .png/.jpg) in \texttt{teams/team21_QiFans/images/} and check filename.
  }}
}
\caption{Overall pipeline of GDino-FT. For D1 (underwater) and D2 (car), they use pretrained GroundingDINO with optimized text prompts (zero-shot). For D3 (car damage), they fine-tune the model on the 10-shot support set while freezing the BERT text encoder.}
\label{fig:method9}
\end{figure}

\noindent \textbf{High-level idea:} They use GroundingDINO (Swin-B) as a unified foundation model for all three target domains. Their key insight is that \emph{different target domains require fundamentally different strategies}: zero-shot prompt engineering for domains containing common objects (D1: underwater, D2: car), and few-shot fine-tuning for specialized fine-grained domains where text-image alignment is weak (D3: car damage). For D1, they craft descriptive multi-synonym prompts to improve recall on uncommon marine categories. For D3, they fine-tune the visual backbone and detection head on the 10-shot support set with heavy data augmentation while freezing the BERT text encoder. Model architecture is given in Fig.~\ref{fig:method9}.

\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Domain-adaptive strategy selection:} Automatically choosing between zero-shot and fine-tuning based on domain characteristics, achieving strong performance across diverse target domains.
    \item \textbf{Optimized prompt engineering:} Descriptive multi-synonym prompts with phrase-to-class mapping doubled D1 mAP (11.23 $\to$ 23.42).
    \item \textbf{Effective few-shot fine-tuning:} Fine-tuning GroundingDINO on just 60 images improved D3 from 9.12 to 36.08 mAP (+26.96), with heavy augmentation preventing overfitting.
\end{itemize}

\noindent \textbf{Model architecture}
\begin{itemize}
    \item Backbone: Swin-B (pretrained on Objects365 + GoldG + Cap4M via GroundingDINO)
    \item Detector: GroundingDINO --- DINO-based open-set detector with cross-modality text-image fusion
    \item Text encoder: BERT-base-uncased (frozen during fine-tuning)
    \item Total parameters: $\sim$172M ($\sim$62M trainable when BERT is frozen)
    \item Foundation models used: GroundingDINO, BERT-base-uncased (2 total)
\end{itemize}

\subsubsection{Training details}
\begin{itemize}
    \item Training data: Only the officially provided 10-shot support set for D3 (60 images, 60 annotations, 6 categories). D1 and D2 use zero-shot only (no support set training).
    \item Few-shot setting: 10-shot for D3. Support images used as-is from the provided JSON annotations.
    \item Optimization: AdamW optimizer, backbone LR=$1\times10^{-5}$, head LR=$5\times10^{-5}$, weight decay=0.05, cosine schedule with 100-step warmup, 200 epochs, batch size 2, mixed precision (FP16), gradient clipping (max norm 0.1)
    \item Loss: Hungarian matching with focal loss ($\alpha$=0.25, $\gamma$=2.0) + L1 loss + GIoU loss, weighted 2:5:2
    \item Augmentations: Random horizontal flip, multi-scale resize (480--800, max 1333), random crop (384--600), color jitter ($p$=0.8), Gaussian blur ($p$=0.3)
    \item Hardware / runtime: 1$\times$ NVIDIA H800 80GB GPU, D3 fine-tuning $\sim$30 minutes
\end{itemize}

\noindent \textbf{Inference details}
\begin{itemize}
    \item D1 (Underwater): Zero-shot, optimized multi-synonym prompt, box\_threshold=0.10, text\_threshold=0.10. Phrase-to-class mapping (e.g., ``sea cucumber'' $\to$ ``holothurian'').
    \item D2 (Car): Zero-shot, simple prompt ``car .'', box\_threshold=0.15, text\_threshold=0.15.
    \item D3 (Car damage): Fine-tuned model, box\_threshold=0.10, text\_threshold=0.10.
    \item Ensemble / TTA: None
    \item Post-processing: Phrase-to-class mapping only. No NMS beyond GroundingDINO's built-in processing.
\end{itemize}

% \subsection{Experimental results}

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{D1} & \textbf{D2} & \textbf{D3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & CD-ViTO Baseline & Close & -- & -- & -- \\
% & Ours (GDino-FT) & Open & 23.42 & 57.06 & 36.08 \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & CD-ViTO Baseline & Close & -- & -- & -- \\
% & Ours (GDino-FT) & Open & 23.42 & 57.06 & 36.08 \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & CD-ViTO Baseline & Close & -- & -- & -- \\
% & Ours (GDino-FT) & Open & 23.42 & 57.06 & 36.08 \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Total weighted score: \textbf{155.42}.}
% \label{tab:results}
% \end{table}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.95\linewidth]{images/per_dataset.pdf}
% \caption{Per-dataset comparison of zero-shot baseline vs.\ our method. D3 (car damage) shows the largest improvement from fine-tuning (+26.96 mAP).}
% \label{fig:per_dataset}
% \end{figure}

\noindent \textbf{Ablation and analysis}

\begin{table}[t]\scriptsize
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Configuration} & \textbf{D1} & \textbf{D2} & \textbf{D3} & \textbf{Total} \\
\midrule
(a) ZS, basic prompts & 11.23 & 57.06 & 9.12 & 103.21 \\
(b) ZS, optimized prompts & 23.42 & 41.04 & 7.14 & 95.47 \\
(c) Best ZS per domain & 23.42 & 57.06 & 9.12 & 119.47 \\
(d) (c) + FT D3 & 23.42 & 57.06 & 33.78 & 152.35 \\
(e) (d) + lower threshold & 23.42 & 57.06 & 36.08 & \textbf{155.42} \\
\bottomrule
\end{tabular}
\caption{Ablation study showing progressive improvements from prompt optimization and fine-tuning.}
\label{tab:ablation}
\end{table}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.95\linewidth]{images/ablation.pdf}
% \caption{Ablation results. Prompt optimization boosts D1 (+12 mAP), fine-tuning dramatically improves D3 (+27 mAP), while D2 is near-optimal with simple zero-shot detection.}
% \label{fig:ablation}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，便于维护和排查
\def\figPath{teams/team21_QiFans/images/ablation.pdf}
% 增加文件存在性检查，避免图片缺失时报错，同时给出清晰提示
\IfFileExists{\figPath}{
  \includegraphics[width=1.\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{1.\linewidth}{
  \centering \textbf{Ablation Figure Placeholder}\\
  Put \texttt{ablation.pdf} (or .png/.jpg) in the \texttt{images/} folder (relative to main .tex file) and check filename.
  }}
}
\caption{Ablation results. Prompt optimization boosts D1 (+12 mAP), fine-tuning dramatically improves D3 (+27 mAP), while D2 is near-optimal with simple zero-shot detection.}
\label{fig:ablation}
\end{figure}


\noindent Key findings from their ablation study:
\begin{itemize}
    \item \textbf{Prompt engineering for specialized domains:} Descriptive multi-synonym prompts doubled D1 mAP (11.23 $\to$ 23.42). However, adding synonyms to common objects \emph{hurts} D2 (57.06 $\to$ 41.04) due to spurious false positives.
    \item \textbf{Fine-tuning for fine-grained domains:} D3 improved from 9.12 to 36.08 mAP (+26.96) through fine-tuning on just 60 images, demonstrating the critical importance of domain adaptation for specialized damage categories.
    \item \textbf{Lower thresholds improve recall:} Reducing box\_threshold from 0.2 to 0.1 for D3 improved mAP from 33.78 to 36.08.
    \item \textbf{Failure case:} Self-training with pseudo-labels on support images degraded performance (126.55), likely due to noise in pseudo-labels for fine-grained damage types.
\end{itemize}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: Yes.
% \item General comments and impressions of the NTIRE 2026 challenge: The challenge provides an excellent benchmark for evaluating cross-domain generalization. The diversity of test domains (underwater creatures, vehicles, car damage) effectively tests different aspects of few-shot detection, from common to highly specialized categories.
% \item Suggestions for future CD-FSOD challenges: Providing a local evaluation script would reduce dependency on the evaluation queue and accelerate method iteration. Per-shot validation during the development phase would also help participants develop truly shot-aware methods.
% \item Other comments: GroundingDINO's strong text-image alignment makes it an effective foundation for cross-domain detection, but fine-grained categories (damage types) remain challenging without domain-specific adaptation.
% \end{itemize}

% %%%%%%%%% REFERENCES
% {\small
% \begin{thebibliography}{4}
% \bibitem{liu2023grounding}
% S.~Liu, Z.~Zeng, T.~Ren, F.~Li, H.~Zhang, J.~Yang, C.~Li, J.~Yang, H.~Su, J.~Zhu, and L.~Zhang.
% \newblock Grounding DINO: Marrying DINO with grounded pre-training for open-set object detection.
% \newblock In \emph{ECCV}, 2024.

% \bibitem{liu2021swin}
% Z.~Liu, Y.~Lin, Y.~Cao, H.~Hu, Y.~Wei, Z.~Zhang, S.~Lin, and B.~Guo.
% \newblock Swin Transformer: Hierarchical vision transformer using shifted windows.
% \newblock In \emph{ICCV}, 2021.

% \bibitem{devlin2019bert}
% J.~Devlin, M.-W. Chang, K.~Lee, and K.~Toutanova.
% \newblock BERT: Pre-training of deep bidirectional transformers for language understanding.
% \newblock In \emph{NAACL}, 2019.

% \bibitem{fu2025cross}
% Y.~Fu, X.~Qiu, J.~Geng, B.~Ren, J.~Pan, Z.~Wu, H.~Tang, Y.~Fu, R.~Timofte, N.~Sebe, and M.~Elhoseiny.
% \newblock NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.
% \newblock In \emph{CVPRW (NTIRE)}, 2025.
% \end{thebibliography}
% }

% \end{document}


==> ntire26/teams/team22_nudt_0110Dplter/affiliation.tex <==
\subsection*{nudt\_0110Dplter}
\noindent\textit{\textbf{Title: }} MSPF-ETS\\
\noindent\textit{\textbf{Members: }} \\
Wang Li (Team Leader) (\href{mailto:483617013@qq.com}{483617013@qq.com}),\\
Qisheng Xu (\href{mailto:qishengxu@nudt.edu.cn}{qishengxu@nudt.edu.cn}),\\
Changjian Wang (\href{mailto:wangcj@nudt.edu.cn}{wangcj@nudt.edu.cn}),\\
Kele Xu (\href{mailto:xukelele@nudt.edu.cn}{xukelele@nudt.edu.cn}),\\
Hui Geng (\href{mailto:gengh666666@163.com}{gengh666666@163.com}),\\
Xuyao Deng (\href{mailto:dengxuyao@nudt.edu.cn}{dengxuyao@nudt.edu.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\
National University of Defense Technology

==> ntire26/teams/team22_nudt_0110Dplter/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\-MSPF-ETS-}

% \author{liwang\\
% None\\
% Changsha, China\\
% {\tt\small 483617013@qq.com}
% }

% \maketitle

% \subsubsection{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \subsubsection{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - \texttt{TEAM\_ID}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{none}
%     \item Team leader (contact): \texttt{liwang}
%     \item Team members: \texttt{none}
%     \item Method name / nickname: \texttt{MSPF-ETS}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \subsubsection{Code Submission}
% \noindent Code link / repository: \href{https://github.com/your_repo}{https://github.com/your\_repo}\\
% \noindent Models / weights link: \href{https://example.com}{https://example.com}\\
% \noindent Reproduction instructions (brief): \texttt{(e.g., bash run.sh / python test.py ...)}

% \subsubsection{Factsheet Information}

% % 4. Factsheet Information

% % 4.1. Team details
% \subsubsection{Team details}
% \begin{itemize}
%     \item Team name: \textbf{none} % 请填写您的队伍名称
%     \item Team leader: \textbf{liwang} % 请填写队长姓名
%     \item Affiliation /contact: \textbf{AFFILIATION}, PHONE (optional), \textbf{483617013@qq.com} % 请填写单位与联系邮箱
%     \item Team members: \textbf{none} % 请填写队员姓名
%     \item Sponsor affiliation (if any): None 
%     \item Method name /nickname: \textbf{MSPF-ETS} (Multi-Scale Prototype Fusion with Enhanced Training Strategy)
%     \item Final score (if available): \textbf{73.71} (Overall weighted mean mAP with 2:1:1 ratio)
%     \item Submission link: \url{https://github.com/ohMargin/NTIRE2026c-FSOD}
% \end{itemize}

% 4.2. Method overview
\subsection{nudt\_0110Dplter}
\subsubsection{Method overview}

\textbf{High-level idea:} 
Building upon CD-ViTO baseline, they propose two key optimizations to address the challenges of CD-FSOD: 1) They introduce a multi-scale prototype fusion mechanism that constructs image pyramids (scales of 0.9x, 1.0x, 1.1x, and 1.2x) and employs temperature-scaled soft weighting (temperature=0.1) to generate robust prototype features resilient to scale variations. 2) They design an Enhanced Training Strategy (ETS) incorporating RandomFlip, RandomChoiceResize (11 discrete scales), and RandomCrop to significantly expand the diversity of limited support sets, mitigating overfitting. These lightweight optimizations integrate seamlessly with CD-ViTO's learnable instance features and domain prompter, achieving substantial performance gains especially on targets with significant indefinable boundaries (IB).

\textbf{Key contributions:}
\begin{itemize}
    \item Contribution 1: A multi-scale prototype extraction module that fuses DINOv2 features from multiple image scales via learnable soft-weighted aggregation, enhancing scale-invariance without increasing inference cost.
    \item Contribution 2: An Enhanced Training Strategy (ETS) specifically designed for few-shot scenarios, utilizing RandomChoiceResize across 11 scales and RandomCrop to augment extremely limited support sets (1-10 shots).
    \item Contribution 3: A practical optimization framework that maintains the parameter efficiency of CD-ViTO (only +0.8M trainable parameters) while significantly improving cross-domain generalization on challenging underwater and industrial defect datasets.
\end{itemize}

% 4.3. Model architecture
\subsubsection{Model architecture}

Their method builds upon the CD-ViTO (Cross-Domain Vision Transformer) architecture, inheriting its core components including the learnable instance features ($M_{LIF}$), instance reweighting module ($M_{IR}$), and domain prompter ($M_{DP}$). They introduce two key augmentations to the prototype extraction and training pipeline:

\begin{itemize}
    \item \textbf{Backbone:} A frozen DINOv2 ViT-L/14 pre-trained on ImageNet-22K via self-supervised learning.
    \item \textbf{Detector:} DE-ViT based open-set detector with Region Proposal Network (RPN), RoI Align, Detection Head ($M_{DET}$), and One-vs-Rest Classification Head ($M_{CLS}$).
    \item \textbf{Additional components:} 
    \begin{enumerate}
        \item \textit{Multi-Scale Prototype Extraction (MSPE):} During support set processing, they generate an image pyramid with scales [0.9, 1.0, 1.1, 1.2], extract patch tokens from each scale using DINOv2, and fuse them via temperature-scaled softmax weighting (temperature=0.1) to obtain scale-robust prototypes.
        \item \textit{ETS Augmentation Pipeline:} Sequential application of RandomFlip (prob=0.5), RandomChoiceResize (short edge randomly selected from [480, 512, 544, 576, 608, 640, 672, 704, 736, 768, 800], max\_size=1333), and RandomCrop (target size 384$\times$600) applied dynamically to support set images during training.
    \end{enumerate}
\end{itemize}

% % 4.4. Training details
% \subsubsection{Training details}

% \begin{itemize}
%     \item \textbf{Training data:} We utilize the publicly available CD-ViTO (DE-ViT) model weights pre-trained on MS-COCO train2017, without conducting additional pre-training on source domain data. Target domains: Three datasets (Dataset1, Dataset2, Dataset3) with novel categories disjoint from COCO. We follow the "pretrain, finetune, and test" pipeline consistent with CD-ViTO, where only fine-tuning on few-shot target support sets is performed.
%     \item \textbf{Few-shot setting:} We evaluate under 1-shot, 5-shot, and 10-shot protocols using balanced K-shot sampling (exactly K object instances per class, as opposed to K images). Support sets are randomly sampled from target domain training splits.
%     \item \textbf{Optimization:} We employ SGD optimizer with a learning rate of 0.002 and momentum 0.9. Training epochs: 80 epochs for 1-shot settings, 40 epochs for 5-shot and 10-shot settings. Batch size is set to 1 per GPU due to the extremely small support set size. Only the top two modules ($M_{DET}$ and $M_{CLS}$) along with our multi-scale fusion parameters are fine-tuned; the DINOv2 backbone remains frozen.
%     \item \textbf{Augmentations:} We apply our proposed \textbf{ETS (Enhanced Training Strategy)} pipeline: 
%     \begin{enumerate}
%         \item RandomFlip: horizontal flip with probability 0.5
%         \item RandomChoiceResize: randomly select short edge size from [480, 512, 544, 576, 608, 640, 672, 704, 736, 768, 800] pixels, with maximum long edge constrained to 1333 pixels
%         \item RandomCrop: fixed crop size of 384$\times$600 pixels to enhance local feature learning
%     \end{enumerate}
%     These augmentations are applied online to support set images during each training iteration to maximize diversity.
%     \item \textbf{Hardware /runtime:} Experiments conducted on \textbf{1$\times$ NVIDIA A800 GPU}. Multi-scale prototype extraction adds approximately 5\% computational overhead during training but zero overhead during inference.
% \end{itemize}

% % 4.5. Inference details
% \subsection{Inference details}

% \begin{itemize}
%     \item \textbf{Test-time settings:} We use the original image resolution without resizing during inference. The Top-K parameter for DE-ViT is set to 5 (or $K=N$ when the number of classes $N<5$). Non-Maximum Suppression (NMS) is applied with standard IoU threshold of 0.5. The confidence score threshold is set to 0.0 to retain all proposals for evaluation.
%     \item \textbf{Ensemble /TTA:} No test-time augmentation (TTA) or model ensemble is used. Single-model inference is performed to ensure fair comparison.
%     \item \textbf{Any post-processing:} Standard COCO evaluation protocol is followed without additional post-processing. The predicted boxes are directly compared against ground truth using COCO API with IoU thresholds ranging from 0.50 to 0.95.
% \end{itemize}

% % 4.6. Experimental results
% \subsection{Experimental results}

% As shown in Table~\ref{tab:results}, our MSPF-ETS method demonstrates significant improvements over the CD-ViTO baseline:

% \begin{itemize}
%     \item \textbf{Dataset2} (likely underwater/industrial domain with significant IB): Substantial gains of +2.82\% (1-shot), +1.44\% (5-shot), and +4.67\% (10-shot), validating the effectiveness of multi-scale feature extraction for handling indefinable boundaries.
%     \item \textbf{Dataset3} (likely aerial/remote sensing domain): Consistent improvements across all shots (+7.38\% for 1-shot, +0.67\% for 5-shot, +1.28\% for 10-shot), demonstrating enhanced generalization.
%     \item \textbf{Overall Performance:} The weighted mean mAP (2:1:1 ratio) improved from \textbf{65.03} to \textbf{73.71} (+8.68 points), with particular strength in 1-shot scenarios where data augmentation is most critical.
% \end{itemize}

% % 4.7. Ablation and analysis (optional)
% \subsection{Ablation and analysis}

% \begin{itemize}
%     \item \textbf{Ablation 1 -- Multi-scale Fusion Scales:} We ablate the number of scales in prototype extraction. Using only single-scale (1.0x) yields significantly lower performance on Dataset2 (1-shot mAP drops from 6.49\% to 4.12\%), confirming that multi-scale fusion is crucial for handling scale variations in cross-domain transfer.
    
%     \item \textbf{Ablation 2 -- ETS Components:} Removing RandomChoiceResize and using fixed-size resize (800px) reduces Dataset3 1-shot mAP by 3.2\%. Removing RandomCrop further degrades performance by 1.8\%, indicating that the combination of multi-scale resizing and random cropping effectively mitigates overfitting on extremely small support sets.
    
%     \item \textbf{Failure cases:} Our method shows marginal degradation on Dataset1 under 5-shot and 10-shot settings compared to the baseline. We attribute this to the specific characteristics of Dataset1 (potentially ArTaxOr-like with small inter-class variance), where aggressive augmentation might introduce noise that confuses the instance reweighting module ($M_{IR}$). Figure~\ref{fig:failure} illustrates cases where small arthropod-like objects with subtle inter-class differences are misclassified after aggressive cropping.
    
%     \begin{figure}[h]
%         \centering
%         % \includegraphics[width=0.8\textwidth]{failure_cases.pdf} % 请在此处插入失败案例可视化
%         \caption{Failure cases on Dataset1 (5-shot). Red boxes indicate false positives where aggressive RandomCrop operations during training caused the model to focus on non-discriminative local patterns.}
%         \label{fig:failure}
%     \end{figure}
% \end{itemize}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{Yes}.
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{(none)}.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{(none)}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{(none)}.
% \end{itemize}



% If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }


==> ntire26/teams/team23_French_Borelli/affiliation.tex <==
\subsection*{French Borelli}

\noindent\textit{\textbf{Title: }} Triple-Tower\\
\noindent\textit{\textbf{Members: }} \\
Adhémar de Senneville (\href{mailto:adhemar.senneville@gmail.com}{adhemar.senneville@gmail.com}),\\
Flavien Armangeon (\href{mailto:flavien.armangeon@gmail.com}{flavien.armangeon@gmail.com})\\
\noindent\textit{\textbf{Affiliations: }} \\
Centre Borelli, ENS Paris-Saclay, 4 avenue des Sciences, Gif-sur-Yvette, France

==> ntire26/teams/team23_French_Borelli/main.tex <==
% mian\documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \usepackage{comment}
% \usepackage{xcolor}
% \definecolor{gray}{gray}{0.5}
% \newcommand{\AD}[2]{{\color{gray}#1}{\color{blue}#2}}
% \newcommand{\TODO}[1]{{\color{red}TODO #1}}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\Triple-Tower}

% \author{
% Adhémar de Senneville\thanks{Equal contribution.}\\
% Centre Borelli\\
% ENS Paris-Saclay\\
% 4, avenue des Sciences\\
% 91190 Gif-sur-Yvette, France\\
% {\tt\small adhemar.senneville@gmail.com}
% \and
% Flavien Armangeon\footnotemark[1]\\
% Centre Borelli\\
% ENS Paris-Saclay\\
% 4, avenue des Sciences\\
% 91190 Gif-sur-Yvette, France\\
% {\tt\small flavien.armangeon@gmail.com}
% }
% \maketitle

% \begin{comment}
% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \end{comment}
% %\section{Email final submission guide}

% %\noindent \textbf{To:}\\
% %{xyqiu24@m.fudan.edu.cn}\\
% %{yuqian.fu.ai@gmail.com}\\
% %{jwgeng25@m.fudan.edu.cn}\\
% %{bin.ren.mondo@gmail.com}\\
% %{jiancheng.pan.plus@gmail.com}\\
% %{zongwei.wu@uni-wuerzburg.de}\\
% %{howard.haotang@gmail.com}\\
% %{yanweifu@fudan.edu.cn}\\
% %{radu.timofte@uni-wuerzburg.de}\\
% %{niculae.sebe@unitn.it}\\
% %{mohamed.elhoseiny@kaust.edu.sa}\\

% %\noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% %\noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - %\texttt{TEAM\_ID}\\

% %\href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.

% %\noindent Body contents should include:
% %\begin{enumerate}[a)]
% %    \item Team name: French Borelli
% %    \item Team leader (contact): Adhémar de Senneville, adhemar.senneville@gmail.com
% %    \item Team members: Adhémar de Senneville, Flavien Armangeon
% %    \item Method name / nickname: Triple-Tower
% %    \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% %\end{enumerate}

% %\noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% We thank the organizers of the challenge. It was an honor to participate and hope that our approach can be useful for their work. We are registered for the \textbf{main track}.

% We would be grateful to be included as co-author in the final workshop report, which will be presented at the CVPR 2026 Workshop. More details on our approach can be given if necessary.
% Our primary research objective in designing Triple-Tower was to develop a compute-efficient method.
% \section{Code Submission}

% \noindent Code link / repository:

% \noindent  \href{https://github.com/farmangeon/NTIRE\_CD-FSOD}{https://github.com/farmangeon/NTIRE\_CD-FSOD}

% \vspace*{2mm}

% \noindent WeDetect Base Weights:

% \noindent \href{https://github.com/WeChatCV/WeDetect/tree/main}{https://github.com/WeChatCV/WeDetect/tree/main}

% \vspace*{2mm}

% \noindent DINOv3 Large Weights:

% \noindent \href{https://huggingface.co/facebook/dinov3-vitl16-pretrain-lvd1689m}{https://huggingface.co/facebook/dinov3-vitl16-pretrain-lvd1689m}

% \vspace*{2mm}
% \noindent Reproduction instructions (brief): First, export class embeddings with \texttt{./WeDetect/get\_prototypes.sh}.

% Then train the object detector with \texttt{./WeDetect/train\_multy.sh}. Finally, train the vision model with \texttt{./WeDetect/train\_vision.sh}. Update the paths in \texttt{./WeDetect/config/paths.py}.

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: French Borelli
% \item Team leader: Adhémar de Senneville, adhemar.senneville@gmail.com
% \item Affiliation / contact: Centre Borelli - Ecole Normale Superieur Paris-Saclay, +33 7 82 55 82 38, adhemar.senneville@gmail.com
% \item Team members: Adhémar de Senneville, Flavien Armangeon
% \item Sponsor affiliation (if any): None
% \item Method name / nickname: Triple-Tower
% \item Final score (if available): 118.058
% \item Submission link: \href{https://miniodis-rproxy.lisn.upsaclay.fr/coda-v2-prod-private/dataset/2026-03-17-1773786892/a503ddf42e1c/post_best_2.zip?AWSAccessKeyId=codabench-prod&Signature=LVQML9AJCzxW%2Bgxc5eyG53lxNqc%3D&Expires=1774227258}{ID-634957}
% \end{itemize}

\subsection{French Borelli}
\subsubsection{Proposed Method}
% (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams2026/team23_French Borelli/method_figure.png}{
%   \includegraphics[width=0.95\linewidth,trim=30 10 100 10,clip]{method_figure.png}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }
% \caption{Overall pipeline of Triple-Tower. 
% We start from a double-tower open-vocabulary detector composed of a language tower and a vision tower. The language tower encodes class names into language prototypes, while the vision tower extracts image features and predicts object bounding boxes. We introduce a third uni-modal tower, a vision-only model trained with a nearest centroid classifier (NCC), which builds visual prototypes from the support set. 
% }
% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，解决路径不一致问题，同时保留trim/clip裁剪参数
\def\figPath{teams/team23\_French\_Borelli/method_figure.png}
\IfFileExists{\figPath}{
  % 加载路径与检查路径完全一致，保留原有的裁剪参数（trim=30 10 100 10,clip）
  \includegraphics[width=1.\linewidth,trim=30 10 100 10,clip]{\figPath}
}{
  % 优化占位提示，明确图片应放置的正确路径和文件名
  \fbox{\parbox[c][0.22\textheight][c]{1.\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method\_figure.png} (or .pdf/.jpg) in \texttt{teams2026/team23\_French\_Borelli/} and check filename.
  }}
}
\caption{Overall pipeline of Triple-Tower. 
They start from a double-tower open-vocabulary detector composed of a language tower and a vision tower. The language tower encodes class names into language prototypes, while the vision tower extracts image features and predicts object bounding boxes. They introduce a third uni-modal tower, a vision-only model trained with a nearest centroid classifier (NCC), which builds visual prototypes from the support set. 
}
\label{fig:method23}
\end{figure}


\noindent \textbf{High-level idea:} 
Open-vocabulary detectors are designed for zero-shot generalization, but there is no straightforward way to improve their performance in few-shot settings beyond standard fine-tuning.
In this work, They argue that few-shot adaptation benefits from decoupling localization from classification. The detector already localizes well, while classification can be improved with a vision-only auxiliary model that exploits richer visual structure than language-aligned features. The model architecture is shown in Fig.~\ref{fig:method23}.

Their method starts by fine-tuning the open-vocabulary detector WeDetect~\cite{fu2025wedetect}.
During fine-tuning, they add pseudo annotations, since they observe that unannotated objects in the training set hurt performance by biasing the detector toward predicting fewer objects.
Finally, they improve the class prediction of each detected bounding box with a vision-only model, DINOv3~\cite{simeoni2025dinov3}. 
To remain compute-efficient, they perform parameter efficient fine-tuning by only training LayerNorm layers (0.03\% of weights).
\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} \textbf{Vision Boosting}: Using a vision model with parameter efficient fine-tuning to boost few-shot classification performance.
    \item \textbf{Contribution 2:} \textbf{Pseudo Annotations}: Periodically adding high-confidence detector predictions from the support set as pseudo annotations during training. 
  %  \item \textbf{Contribution 3 (optional):} \texttt{(one sentence)}
\end{itemize}

\noindent \textbf{Model architecture}
\begin{itemize}
    \item Backbone: WeDetect~\cite{fu2025wedetect} (ConvNeXt-base and X-BERT-base) and DINOv3~\cite{simeoni2025dinov3} (ViT-L)
%    \item Detector: \texttt{(e.g., Faster R-CNN / Deformable DETR / etc.)}
%    \item Additional components: \texttt{(e.g., prototype module, attention, adapter, etc.)}
\end{itemize}

\subsubsection{Training details}
\begin{itemize}
    \item Training data: No additional training data
    \item Pseudo Annotations:
    Pseudo annotations are generated during the fine-tuning of WeDetect over 100 epochs. Starting from epoch 15, they run the detector on the support set every 5 epochs and add high-confidence predictions to the training annotations. Predictions whose score is above a fixed threshold are kept, new detections with excessive overlap (IoU$\geq$0.70) with existing support annotations are discarded.
    \item Vision Boosting:
    After fine-tuning the open-vocabulary detector, they train the vision backbone with an Nearest Centroid Classifier (NCC) loss on all labels and pseudo labels.
    \item Optimization:
    For WeDetect: they optimize the detector with AdamW, using a learning rate of \texttt{2e-5}, weight decay \texttt{0.05}, batch size \texttt{4}, and a total of \texttt{100} training epochs. 
    %The learning rate uses a linear warmup during the first \texttt{1000} iterations, followed by a linear decay over training.
    For DINOv3: they optimize the detector with AdamW, using a learning rate of \texttt{0.005} over \texttt{20} epochs with batch size \texttt{50}
    \item Augmentations:
    Training uses random horizontal flip, multi-scale resizing, random cropping, YOLO-style mosaic augmentation, random affine transformations, MixUp, HSV augmentation, blur, median blur, grayscale conversion, and CLAHE. 
    For aerial datasets (dataset2), they add rotation augmentation.
    \item Hardware / runtime:
    All experiments were conducted on a single NVIDIA GeForce RTX 3090. Training over all datasets takes approximately 12min in total, with 10min for the detector and 2min for the vision models.
\end{itemize}

\noindent \textbf{Inference details}
\begin{itemize}
    \item Test-time settings:
     Images are resized to \texttt{640$\times$640} using keep-ratio resizing followed by letterbox padding. During inference, They use multi-label prediction, a score threshold of \texttt{0.0001}, pre-NMS filtering with \texttt{nms\_pre=30000}, non-maximum suppression with IoU threshold \texttt{0.7}, and keep at most \texttt{200} detections per image.
    \item Ensemble:  At inference, the final classification logits are obtained by adding the predictions of the vision-based classifier and the language-based classifier.
%    \item Any post-processing: \texttt{(if used)}
\end{itemize}

% \subsection{Experimental results}

% Figure~\ref{fig:pseudo} illustrates pseudo-annotation results. During training, a ground truth image contains only one annotation, while many objects of interest are present. This observation penalises the model for cars well detected but not annotated, thus reduces the performance. This is why we add pseudo labels at multiple epochs based on the predictions with high score. This improves the performance while being computer efficient.

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/pseudo_4_20161030_GF2_00154.png}
%     \caption{Examples of pseudo-annotations under 10-shot setting at the end of training (100 epochs). Green boxes show the ground truth, while orange boxes show the pseudo-labels. The pseudo-annotation retrieves all the cars.}
%     \label{fig:pseudo}
% \end{figure}


% Table~\ref{tab:results} gives the performance obtained by submitting the results on the official challenge webpage.

% \begin{table}[!htbp]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% Shots& \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{1}{*}{1}
% %& Baseline / Reference & \texttt{(Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (Triple-Tower) & \texttt{(Open)} & 21.25 & 35.87 & 16.10 \\
% \midrule
% \multirow{1}{*}{5}
% %& Baseline / Reference & \texttt{(Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (Triple-Tower) & \texttt{(Open)} & 25.89 & 41.14 & 26.93 \\
% \midrule
% \multirow{1}{*}{10}
% %& Baseline / Reference & \texttt{(Open)} & \texttt{--} & \texttt{--} & \texttt{--} \\
% & Ours (Triple-Tower) & \texttt{(Open)} & 29.29 & 51.55 & 32.91 \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets.}
% \label{tab:results}
% \end{table}
% %Triple-Tower {'dataset1': {'1shot': 21.25397163210162, '5shot': 25.89480525925732, '10shot': 29.293568607566943}, 'dataset2': {'1shot': 35.87383351774674, '5shot': 41.13749307836178, '10shot': 51.5536903958853}, 'dataset3': {'1shot': 16.102327337078833, '5shot': 26.92610753468973, '10shot': 32.90810263054695}}





% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: Yes.
% \item General comments and impressions of the NTIRE 2026 challenge:
% The competition was well-structured and organized. We unfortunately noticed too late that new methods and approaches were encouraged by reading this document.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): 
% A reasoning track that emphasizes the use of state-of-the-art multimodal models could be interesting.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.:
% Having limited computational resources makes it hard to be competitive.
% \end{itemize}

%%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% \begin{comment}
% {\small
% \begin{thebibliography}{1}
% \bibitem{fu2025cross}
% Author(s).
% \newblock Paper title.
% \newblock Conference/Journal, Year. (Placeholder; replace with real references.)
% \end{thebibliography}
% }
% \end{comment}

% % If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team24_FewShotEverything/affiliation.tex <==
\clearpage
\subsection*{FewShotEverything}
\noindent\textit{\textbf{Title:}} AIPR: Data Augmentation and Iterative Pseudo-labeling with Prototype Refinement for Cross-Domain Few-Shot Object Detection\\
\noindent\textit{\textbf{Members: }} \\
Yazhe Lyu\textsuperscript{1} (\href{yazhelv@hust.edu.cn}{yazhelv@hust.edu.cn})\\
Zhimeng Xin\textsuperscript{2} (\href{zhimengxin15@gmail.com}{zhimengxin15@gmail.com})\\
Zijian Zhuang\textsuperscript{1} (\href{zhuangzijian@hust.edu.cn}{zhuangzijian@hust.edu.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\ 
\textsuperscript{1} School of Computer Science and Technology, Huazhong University of Science and Technology \\
\textsuperscript{2} School of Cyber Science and Engineering, Huazhong University of Science and Technology \\

==> ntire26/teams/team24_FewShotEverything/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}
% % \usepackage{hyphenat}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\
% AIPR: Data augmentation and Iterative Pseudo-labeling with Prototype Refinement for Cross-Domain Few-Shot Object Detection}

% \author{
% Yazhe Lyu\textsuperscript{1} \qquad
% Zhimeng Xin\textsuperscript{2} \qquad
% Zijian Zhuang\textsuperscript{1} \\
% \textsuperscript{1}School of Computer Science and Technology, Huazhong University of Science and Technology \\
% \textsuperscript{2}School of Cyber Science and Engineering, Huazhong University of Science and Technology \\
% {\tt\small yazhelv@hust.edu.cn \qquad zhimengxin15@gmail.com \qquad zhuangzijian@hust.edu.cn}
% }
% \maketitle

% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025ntire}, trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - \texttt{TEAM\_ID}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{TEAM\_NAME}
%     \item Team leader (contact): \texttt{NAME}, \texttt{EMAIL}
%     \item Team members: \texttt{MEMBER\_1, MEMBER\_2, ...}
%     \item Method name / nickname: \texttt{METHOD\_NAME}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/zhimengXin/CD-FSOD-Challenge}{https://github.com/zhimengXin/CD-FSOD-Challenge}\\
% \noindent Models / weights link: \href{https://pan.baidu.com/s/1EcE5vMqr7Kp1Bp2lYztxmA?pwd=2ibp}{Baidu Netdisk Link}\\
% \noindent Reproduction instructions (brief): \href{https://github.com/zhimengXin/CD-FSOD-Challenge/blob/main/README.md} {README}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: FewShotEverything
% \item Team leader: Yazhe Lyu
% \item Affiliation / contact: \\
% School of Computer Science and Technology, Huazhong University of Science and Technology. yazhelv@hust.edu.cn
% \item Team members: \\
% Zhimeng Xin, Zijian Zhuang
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: AIPR
% \item Final score (if available): 134.3072
% \item Submission link: \\
% \href{https://pan.baidu.com/s/1nStDlS2fWhoT_W8ctJXB-g?pwd=xygy}{Factsheet Link}\\
% \href{https://github.com/zhimengXin/CD-FSOD-Challenge}{Code Link}
% \end{itemize}
\subsection{FewShotEverything}

\subsubsection{Proposed Method}
% (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=\linewidth]{teams/team24_FewShotEverything/images/method.pdf}
% \caption{Overall pipeline of AIPR.}
% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，提升可维护性并增加容错能力
\def\figPath{teams/team24_FewShotEverything/images/method.pdf}
% 增加文件存在性检查，避免图片缺失时报错，给出精准提示
\IfFileExists{\figPath}{
  \includegraphics[width=\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method.pdf} (or .png/.jpg) in \texttt{teams/team24_FewShotEverything/images/} and check filename.
  }}
}
\caption{Overall pipeline of AIPR.}
\label{fig:method}
\end{figure}

% \begin{figure}[!htbp]
% \centering
% \IfFileExists{images/generation.pdf}{
%   \includegraphics[width=\linewidth]{images/generation.pdf}
% }{
%   \fbox{\parbox[c][0.2\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   }}
% }
% \caption{Overall pipeline of \texttt{METHOD\_NAME}. Replace with your own figure and caption.}
% \label{fig:generation}
% \end{figure}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=\linewidth]{teams/team24_FewShotEverything/images/generation.pdf}
% \caption{Overall pipeline of the data generation process for data augmentation.}
% \label{fig:generation}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，提升可维护性并增加容错能力
\def\figPath{teams/team24_FewShotEverything/images/generation.pdf}
% 增加文件存在性检查，避免图片缺失时报错，给出精准提示
\IfFileExists{\figPath}{
  \includegraphics[width=\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{\linewidth}{
  \centering \textbf{Data Generation Figure Placeholder}\\
  Put \texttt{generation.pdf} (or .png/.jpg) in \texttt{teams/team24_FewShotEverything/images/} and check filename.
  }}
}
\caption{Overall pipeline of the data generation process for data augmentation.}
\label{fig:generation}
\end{figure}


\noindent \textbf{High-level idea:} They proposed a Cross-Domain Few-Shot Object Detection (CDFSOD) framework based on the CD-ViTO baseline\cite{fu2024cross} under the closed-setting.
The framework consists of three modules: (1) \textbf{Training-Set Data Augmentation module (TDAM)} that enhances sample diversity and exposes the model to more varied object appearances in target domain, which improves robustness to domain shift between the source and target domains.
(2) \textbf{Prototype Refinement Module (PRM)} that refines foreground prototype extraction by concentrating on semantically relevant object regions, which effectively mitigates the influence of surrounding noise and irrelevant background, leading to more reliable cross-domain prototypes.
(3) \textbf{Iterative Pseudo-Labeling Module (IPLM)}, which addresses incomplete support annotations by progressively identifying unlabeled target instances in support images. Specifically, it identifies cases where only a single instance is labeled per image despite the presence of multiple targets. To prevent the model from treating unlabeled vehicles as background in dataset2, the supervision is enriched through iterative pseudo-label refinement.
Together, these modules improve detection performance and effectively reduce the impact of domain shift.


\noindent \textbf{Key contributions:}
\begin{itemize}
  \item \textbf{Contribution 1:} A Training-Set Data Augmentation module is proposed by leveraging a VLM to synthesize support-like images and corresponding detection annotations, enhancing sample diversity and improving robustness to domain shift between the source and targets.
    \item \textbf{Contribution 2:} A Prototype Refinement Module is introduced to improve foreground prototype extraction by focusing on semantically relevant object regions, thereby reducing the interference of background noise and producing more reliable cross-domain prototypes.
    \item \textbf{Contribution 3 (optional):} An Iterative Pseudo-Labeling Module is designed to address incomplete support annotations by progressively mining unlabeled target instances and refining pseudo-labels, which provides additional supervision for target-domain adaptation.
\end{itemize}

\noindent\textbf{Model architecture.}
Describe the backbone, detector head, any added modules, and where they are inserted.
\begin{itemize}
    \item Backbone: Following baseline work \cite{fu2024cross}, they utilize the pre-trained ViT-L/14 variant from DINOv2 as backbone, which is initialized with weights learned through self-supervised learning on large-scale image datasets. This backbone extracts high-level semantic features from input images via its multi-layer transformer encoder.
    \item Detector:  They then integrate the backbone with the Faster R-CNN~\cite{fasterrcnn} architecture, which consists of a Region Proposal Network (RPN) and a detection head for classification and bounding box regression. 
    \item Additional components: Following baseline work \cite{fu2024cross}, they utilize the pre-trained ViT-L/14 variant from DINOv2 as the backbone for prototype extraction, leveraging its powerful feature representation capabilities to enhance the accuracy of CD-FSOD.
\end{itemize}




\subsubsection{Training details}
Provide training settings sufficient for reproduction.
\begin{itemize}
    \item Training data: Following closed-source setting and CD-ViTO~\cite{fu2024cross}, COCO~\cite{lin2014microsoft} is used as the source-domain dataset for base training, since its large-scale annotations and diverse object categories provide strong transferable detection features. The three datasets provided by the challenge are treated as the target-domain data.
    \item Few-shot setting: Following provided annotation splits of the targets, they evaluate under 1-shot, 5-shot, and 10-shot settings, where each class is assigned 1, 5, or 10 annotated support instances, respectively, and only the support annotations corresponding to each shot setting are used for model adaptation and training.
    \item Optimization: The Training-Set Data Augmentation module and Prototype Refinement Module are used for all three datasets, while the Iterative Pseudo-Labeling Module is additionally applied to Dataset2, which is a single-class dataset with incomplete training annotations. 
    The trainable parameters are fine-tuned with dataset-specific training epochs under different experimental settings. For all datasets, the model is optimized using SGD with a base learning rate of 0.001, and the batch size is set to 16 images per batch.
    \item Augmentations: The target-domain training set is augmented via Qwen-Image2.0\cite{wu2025qwen}. Given a target-domain image and a designed text prompt, Qwen-Image2.0 generates additional images that are visually similar, while preserving domain characteristics and target objects. These synthesized images, along with the corresponding prompts, are then fed into a Qwen-VL model\cite{wang2024qwen2} to produce pseudo-labels, including object categories and bounding boxes.
    \item Hardware / runtime: Experiments are conducted on two NVIDIA A6000 GPUs.
\end{itemize}

\noindent\textbf{Inference details}
Explain inference-time details that affect performance.
\begin{itemize}
    \item Test-time settings: they follow the default inference
pipeline of the corresponding detector framework for
prediction filtering and box selection.
    \item Ensemble / TTA: None
    \item Post-processing: In the iterative pseudo-labeling module, low-confidence pseudo labels generated from initial training data are removed based on a confidence threshold.
\end{itemize}

% \subsection{Experimental results}
% The experimental results are presented in \cref{tab:results}.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\tiny 1-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{14.909} & \texttt{19.943} & \texttt{19.545} \\
% & Ours (\texttt{METHOD\_NAME}) & \texttt{(Close)} & \texttt{23.025} & \texttt{41.527} & \texttt{21.728} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\tiny 5-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{22.580} & \texttt{30.044} & \texttt{24.466} \\
% & Ours (\texttt{METHOD\_NAME}) & \texttt{(Close)} & \texttt{29.482} & \texttt{46.654} & \texttt{34.822} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\tiny 10-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{21.480} & \texttt{25.466} & \texttt{33.759} \\
% & Ours (\texttt{METHOD\_NAME}) & \texttt{(Close)} & \texttt{31.087} & \texttt{51.893} & \texttt{36.318} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets.}
% \label{tab:results}
% \end{table}

% \noindent\textbf{Ablation and analysis }
% Table~\ref{tab:ablation} presents the ablation results of the proposed modules under the 10-shot setting. Starting from the CD-ViTO baseline, three components are progressively introduced to evaluate their individual contributions.
% \begin{itemize}
%     \item \textbf{Effect of TDAM.} After adding the \textbf{Training-Set Data Augmentation Module (TDAM)}, the performance improves consistently on all three datasets. This indicates that augmenting the target-domain training set effectively enriches sample diversity and improves the model's robustness to domain shift.

%     \item \textbf{Effect of PRM.} Incorporating the \textbf{Prototype Refinement Module (PRM)} further boosts performance. The improvement demonstrates that refining foreground prototype extraction with semantically relevant object regions helps suppress background noise and produces more reliable cross-domain prototypes.

%     \item \textbf{Effect of IPLM.} The \textbf{Iterative Pseudo-Labeling Module (IPLM)} is applied only to Dataset2, where the training annotations are incomplete. This result shows that iterative pseudo-label refinement can effectively recover missing supervision and provide additional useful training signals for adaptation.
% \end{itemize}

% \begin{table}[t]
% \scriptsize
% \centering
% \begin{tabular}{ccccc}
% \toprule
% \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% Baseline  & \texttt{(Close)} & \texttt{21.480} & \texttt{25.466} & \texttt{33.759} \\
% + TDAM  & \texttt{(Close)} & \texttt{28.686} & \texttt{37.904} & \texttt{35.130} \\
% + PRM  & \texttt{(Close)}    & \texttt{31.087} & \texttt{39.761} & \texttt{36.318} \\
% + IPLM & \texttt{(Close)}  & \texttt{-} & \texttt{51.893} & \texttt{-} \\
% \bottomrule
% \end{tabular}
% \caption{Results under different few-shot settings on three target datasets.}
% \label{tab:ablation}
% \end{table}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{No}.
% \item General comments and impressions of the NTIRE 2026 challenge: The NTIRE 2026 challenge offers a valuable benchmark for CDFSOD, emphasizing domain shift and limited annotations. It encourages the development of robust and generalizable methods, and provides a well-designed evaluation protocol for fair comparison.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): Besides mAP, additional metrics on robustness to domain shift, inference efficiency, and annotation efficiency would provide a more comprehensive evaluation. 
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: It would be beneficial if different settings could be ranked separately on the Codabench platform, as this would provide a clearer and fairer comparison among methods under different evaluation protocols.
% \end{itemize}

% %%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% % {\small
% % \begin{thebibliography}{1}
% % \bibitem{fu2025cross}
% % Author(s).
% % \newblock Paper title.
% % \newblock Conference/Journal, Year. (Placeholder; replace with real references.)
% % \end{thebibliography}
% % }

% % If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team2_Fusion-Few/affiliation.tex <==
\subsection*{Fusion-Few}
\noindent\textit{\textbf{Title: }} FusionFormer\\
\noindent\textit{\textbf{Members: }} \\
Hongchun Zhu (\href{mailto:vice2city@qq.com}{vice2city@qq.com})\\
\noindent\textit{\textbf{Affiliations: }} \\
University of Electronic Science and Technology of China, China.

==> ntire26/teams/team2_Fusion-Few/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\FusionFormer}

% \author{Hongchun Zhu\\
% University of Electronic Science and Technology of China\\
% Chengdu, China, 611731\\
% {\tt\small vice2city@qq.com}
% }

% \maketitle

% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}, trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - \texttt{TEAM\_ID}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{TEAM\_NAME}
%     \item Team leader (contact): \texttt{NAME}, \texttt{EMAIL}
%     \item Team members: \texttt{MEMBER\_1, MEMBER\_2, ...}
%     \item Method name / nickname: \texttt{METHOD\_NAME}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/vice2city/FusionFormer_code}{FusionFormer_code}\\
% \noindent Models / weights link: \href{https://drive.google.com/drive/folders/1OuuGuw1HGJaIELblslh7c3Mrd7wMw7UF?usp=sharing}{Google Drive}\\
% \noindent Reproduction instructions (brief): bash scripts/fsfinetune.sh dataset shot-set

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: \texttt{Fusion-Few}
% \item Team leader: \texttt{Hongchun Zhu}
% \item Affiliation: \texttt{University of Electronic Science and Technology of China}
% \item Team members: \texttt{Ji Zhang, Pengpeng Zeng, Xuanhan Wang, Lianli Gao, Jingkuan Song}
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \texttt{FusionFormer}
% \item Final score (if available): \texttt{108.48}
% \item Submission link: \href{https://miniodis-rproxy.lisn.upsaclay.fr/coda-v2-prod-private/dataset/2026-03-17-1773774796/fd1c5d0799a1/test9.zip?AWSAccessKeyId=codabench-prod&Signature=gamc7QsHj1U1f5TxWqgt0aYjkhI%3D&Expires=1774263611}{link}
% \end{itemize}

\subsection{Fusion-Few}
\subsubsection{Proposed Method}

% (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams/team2_Fusion-Few/method_figure.pdf}{
%   \includegraphics[width=0.95\linewidth]{method_figure.pdf}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }


% \caption{Overview of the FusionFormer framework. The architecture leverages a frozen DINOv2 ViT backbone for feature extraction. It features a Siamese-style encoder-decoder structure integrated with Object-Background Discrimination (OBD) and Object-Object Discrimination (OOD) modules to mitigate cross-domain feature confusion. The final detection head employs a multi-strategy ensemble (Prototype Cosine, Graph Diffusion, and MLP) to enhance classification robustness in few-shot scenarios.}
% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，解决路径不一致问题，提升可维护性
\def\figPath{teams/team2_Fusion-Few/method_figure.pdf}
\IfFileExists{\figPath}{
  % 加载路径与检查路径完全一致，保留原宽度设置
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  % 优化占位提示，明确图片应放置的正确路径
  \fbox{\parbox[c][0.22\textheight][c]{1.\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method\_figure.pdf} (or .png/.jpg) in \texttt{teams/team2_Fusion-Few/} and check filename.
  }}
}

\caption{Overview of the FusionFormer framework. The architecture leverages a frozen DINOv2 ViT backbone for feature extraction. It features a Siamese-style encoder-decoder structure integrated with Object-Background Discrimination (OBD) and Object-Object Discrimination (OOD) modules to mitigate cross-domain feature confusion. The final detection head employs a multi-strategy ensemble (Prototype Cosine, Graph Diffusion, and MLP) to enhance classification robustness in few-shot scenarios.}
\label{fig:method2}
\end{figure}

\noindent \textbf{High-level idea:} They present FusionFormer, a Transformer-based architecture specifically engineered for Cross-Domain Few-Shot Object Detection (CD-FSOD). The core objective is to mitigate the severe feature confusion inherent in cross-domain scenarios. Built upon the CDFormer~\cite{meng2025cdformer} backbone, their method introduces a learnable background token within the Object-Background Discrimination (OBD) module and contrastive learning within the Object-Object Discrimination (OOD) module to enhance background separation and inter-class distinctness. To further improve inference robustness, they propose an offline ensemble strategy that synergistically fuses predictions from a linear classifier, a graph diffusion model, and OOD-based feature caching. Combined with reinforced source-domain augmentation, test-time pseudo-labeling, and Test-Time Augmentation (TTA), FusionFormer effectively bridges the domain gap and exhibits superior generalization on unseen target domains.\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Enhanced Detection Framework:} A CDFormer~\cite{meng2025cdformer}-based architecture that fundamentally addresses feature confusion in cross-domain settings via the dual-pronged OBD and OOD modules.
    \item \textbf{Innovative Multi-Head Ensemble:} An offline ensemble mechanism that integrates a linear layer, graph diffusion, and feature-cache information to significantly boost prediction accuracy.
    \item \textbf{Comprehensive Optimization Pipeline:} A robust training-to-inference workflow incorporating specialized augmentation, high-confidence pseudo-label mining, and TTA to minimize performance degradation.
\end{itemize}

\noindent \textbf{Model architecture.}
Describe the backbone, detector head, any added modules, and where they are inserted.
\begin{itemize}
    \item Backbone: A frozen DINOv2 ViT-L/14 is used as the main feature extractor. To refine spatial granularity, a convolutional layer is appended to downsample stride-14 features to stride-28, ensuring better alignment for object detection.
    \item Detector: The detector follows a Deformable-DETR architecture, comprising a 6-layer Encoder and a 6-layer Decoder. The decoder is configured as a category-agnostic meta-decoder with 300 queries to maintain flexibility across domains.
    \item Additional components:
    \begin{itemize}
        \item Query-Support Interaction: A SingleHeadSiameseAttention module is integrated into the first encoder layer to facilitate cross-modal feature interaction between query and support branches.
        \item Episodic Category Codes: Category prototypes derived from support branch are injected into the main branch per episode to provide strong class-specific priors.
        \item Multi-type Prediction Heads: the regression head utilizes a standard MLP; the classification task is handled by a triple-head ensemble: a linear layer, a graph diffusion model, and an OOD-based feature cache.
    \end{itemize}
\end{itemize}


% \subsubsection{Experimental results}
% Fill in your results. Replace dataset names with official ones used in the challenge.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & Baseline & \texttt{Close} & \texttt{0.232} & \texttt{0.173} & \texttt{0.102} \\
% & Ours (\texttt{FusionFormer}) & \texttt{Close} & \texttt{0.245} & \texttt{0.279} & \texttt{0.159} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & Baseline & \texttt{Close} & \texttt{0.310} & \texttt{0.186} & \texttt{0.196} \\
% & Ours (\texttt{FusionFormer}) & \texttt{Close} & \texttt{0.333} & \texttt{0.278} & \texttt{0.318} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & Baseline & \texttt{Close} & \texttt{0.315} & \texttt{0.163} & \texttt{0.199} \\
% & Ours (\texttt{FusionFormer}) & \texttt{Close} & \texttt{0.335} & \texttt{0.279} & \texttt{0.344} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets.}
% \label{tab:results}
% \end{table}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{Yes}.
% \item General comments and impressions of the NTIRE 2026 challenge: The challenge presents a rigorous and timely benchmark for evaluating the adaptability of object detection systems in extreme scenarios.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{None}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{None}.
% \end{itemize}

%%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \begin{thebibliography}{1}
% \bibitem{fu2025cross}
% Author(s).
% \newblock Paper title.
% \newblock Conference/Journal, Year. (Placeholder; replace with real references.)
% \end{thebibliography}
% }

% If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }


==> ntire26/teams/team5_SAIDA/affiliation.tex <==
\subsection*{SAIDA}
\noindent\textit{\textbf{Title: }} Synthetic-Augmented Iterative Domain Adaptation\\
\noindent\textit{\textbf{Members: }} \\
Kyeongryeol Go,\\
Taewoong Jang\\
\noindent\textit{\textbf{Affiliations: }} \\
Superb AI

==> ntire26/teams/team5_SAIDA/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\- Synthetic-Augmented Iterative Domain Adaptation -}

% \author{Kyeongryeol Go\\
% Superb AI\\
% Seoul, South Korea\\
% {\tt\small krgo@superb-ai.com}
% \and
% Taewoong Jang\\
% Superb AI\\
% Seoul, South Korea\\
% {\tt\small twjang@superb-ai.com}
% }

% \maketitle

% \noindent \textbf{{Team details}}
% \begin{itemize}
% \item Track: Main
% \item Team / method name: \texttt{SAIDA}
% \item Team leader: \texttt{Kyeongryeol Go}
% \item Team members: \texttt{Taewoong Jang}
% \item Affiliation: \texttt{Superb AI}
% \item Contact: \texttt{krgo@superb-ai.com}
% \item Sponsor affiliation: \texttt{None}
% \item Final score: \texttt{161.086}
% \item Submission link: \texttt{\href{https://github.com/gokyeongryeol/SAIDA}{github repository}}
% \end{itemize}
\subsection{SAIDA}

\subsubsection{Proposed Method}


\noindent\textbf{High-level Idea. }Cross-Domain Few-Shot Object Detection (CD-FSOD) \cite{fu2024cross} presents a formidable challenge in computer vision, requiring models to adapt to novel target distributions with extremely sparse supervision—typically limited to 1, 5, or 10-shot annotations. A critical vulnerability in standard training pipelines for CD-FSOD is the inherent risk of false negatives; when training on such sparse labels without preliminary refinement, the model often incorrectly learns to categorize unannotated objects as background, leading to catastrophic interference during domain transfer.

Synthetic-Augmented Iterative Domain Adaptation (SAIDA) addresses these constraints through a four-phase pipeline, as demonstrated in Fig.~\ref{fig:method8}. By progressing from label-agnostic adaptation to iterative pseudo-labeling and generative data expansion, SAIDA optimizes the latent space for domain-specific distributions and maximizes model precision in data-scarce environments.

\begin{figure}[h]
\centering
\def\figPath{teams/team5_SAIDA/method_figure.png}
\IfFileExists{\figPath}{
  \includegraphics[width=\columnwidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{\columnwidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method\_figure.png} (or .pdf/.jpg) in \texttt{teams2026/team5_SAIDA/} and check filename.
  }}
}
\caption{Overall pipeline of \texttt{SAIDA}}
\label{fig:method8}
\end{figure}

% \noindent\textbf{Method and experimental details}
\subsubsection{Module Details}

% \begin{figure*}[!t]
% \centering
% \IfFileExists{teams2026/team5_SAIDA/method_figure.png}{
%   \includegraphics[width=\textwidth]{method_figure.png}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{\textwidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }
% \caption{Overall pipeline of \texttt{SAIDA}}
% \label{fig:method}
% \end{figure*}



\noindent\textbf{Shot-agnostic domain adaptation.}
The initial phase focuses on adapting the model to the target domain's visual distribution without relying on the provided challenge labels. This ensures the architecture captures the underlying semantics of the new domain before category-specific fine-tuning begins.

\begin{itemize}
    \item Foundation model selection: They utilize ZERO\cite{spbaizero}, a vision foundation model developed by Superb AI. ZERO is a zero-shot/few-shot object detection model specifically engineered for visual grounding tasks and supports both text and visual prompts, making it an ideal candidate for zero-shot domain initialization.
    \item Noun phrase extraction Pipeline: To identify potential objects in the target domain, they employ an ensemble of open-vocabulary detectors—including Grounding DINO\cite{groundingdino}, YOLO-E\cite{yoloe}, and SAM3\cite{sam3}. These models use target category names as text prompts to distinguish objects from the background. The resulting detections are processed by  Qwen3-VL \cite{qwen3vl} to extract descriptive semantic noun phrases, which provide richer context than primitive category labels.
    \item Alignment and reconstruction: The model is optimized using (bounding box, noun phrase) pairs. They employ a dual-loss objective that incorporates both CLIP\cite{clip} and CapPa\cite{cappa} losses without modifying the model architecture of ZERO. This approach ensures global semantic alignment in the embedding space while simultaneously performing conditional reconstruction to stabilize the vision-language projection.
    \item Efficiency via parameter-efficient fine-Tuning: To maintain the predictive performance of the pretrained weights while adapting to new domain semantics, they apply Low-Rank Adaptation (LoRA)\cite{lora} specifically to the prompt encoders. This preserves the generalization capabilities of the foundation model while minimizing the computational footprint of the adaptation.
\end{itemize}




\noindent\textbf{Iterative shot-dependent fine-tuning.}
Following the shot-agnostic adaptation, the methodology transitions to leveraging the provided challenge annotations with a shot-dependent fine-tuning through a iterative process.
\begin{itemize}
    \item Prompt engineering: They utilize human evaluation and feedback from evaluation servers to identify the optimal prompt types for each (dataset, shot) pair. This ensures that the initial pseudo-labels are generated using the most effective semantic cues for the specific domain.
    \item Mathematical threshold optimization: They calculate class-wise score thresholds to optimize the pseudo-labeling process by F-score optimization. By weighing precision higher than recall, they mitigate semantic drift and prevent the propagation of label noise into the training set. As model reliability improves over iterations, they progressively shift the balance from precision to recall, since the risk of introducing noisy pseudo-labels decreases while the benefit of covering more object instances increases.
    \item Label merging strategy: They employ a class-agnostic Non-Maximum Suppression (NMS) to integrate pseudo-labels with Ground-Truth (GT) annotations. In this logic, GT labels are assigned a confidence score of 1.0, ensuring they take priority during the merging process.
    \item Model evolution: This phase facilitates the continual learning of both the prompt encoder finetuned ZERO and the Object365\cite{object365} pretrained Co-DETR\cite{codetr}, with each round refining the quality of the training signals. They follow the default training configurations (e.g., data augmentation, optimizer) provided in the Transformers\cite{transformers} and MMDetection\cite{mmdetection} libraries for ZERO and Co-DETR, respectively\footnote{\href{https://github.com/huggingface/transformers/blob/main/examples/pytorch/object-detection/run_object_detection_no_trainer.py}{ZERO training config}, \href{https://github.com/open-mmlab/mmdetection/blob/main/projects/CO-DETR/configs/codino/co_dino_5scale_swin_l_16xb1_16e_o365tococo.py}{Co-DETR training config}}. For the detailed model architectures, please refer to their technical reports.
\end{itemize}


\noindent\textbf{Diffusion-based data augmentation.}
To circumvent the performance saturation often observed with limited datasets, they expand the training data by a factor of 10 using an image generative model.

\begin{itemize}
    \item Captioning and T2I fine-tuning: Qwen3-VL \cite{qwen3vl} is used to generate high-fidelity captions for the target domain images. These pairs are used to fine-tune Qwen-Image\cite{qwenimage} (via the DiffSynth-Studio library\cite{diffsynth2024}) using LoRA\cite{lora}.
    \item Synthetic scaling: They generate synthetic images using the fine-tuned Qwen-Image\cite{qwenimage} and annotate them with pseudo-labels produced by ZERO\cite{spbaizero} or Co-DETR\cite{codetr} from the previous round. These synthetic samples are incrementally incorporated into subsequent training rounds, improving the model’s robustness to domain shifts and enhancing overall generalization.
\end{itemize}

\noindent\textbf{Final optimization.}
In the final phase, they conduct empirical tuning to maximize discriminative performance.
\begin{itemize}
    \item Curriculum data augmentation: Rather than relying on generative augmentations, they tried image processing-based augmentation techniques. In particular, they employ color augmentations, which is commonly used as strong augmentations in semi-supervised learning, to improve robustness during training \cite{guo2022scale}.
    \item Test-time augmentation: During inference, they employ multi-scale resizing (×0.75, ×1.0, ×1.25) combined with horizontal flipping.
\end{itemize}


% \section{Experimental results}

% \begin{table}[t]
% \centering
% \begin{tabular}{c l}
% \toprule
% \textbf{Round} & \textbf{Newly Introduced Methods} \\
% \midrule
% R0 & Pretrained model \\
% \midrule
% R1 & + Shot-agnostic domain adaptation \\
% \midrule
% R2 & + Shot-dependent fine-tuning \\
% \midrule
% R3 & + Synthetic data expansion ($\times$5) \\
% \midrule
% R4 & + Synthetic data expansion ($\times$5) \\
%    & + Color augmentation \\
%    & + Test-time augmentation \\
% \bottomrule
% \end{tabular}
% \caption{Progressive introduction of methods across rounds.}
% \end{table}

% Table~\ref{tab:results} clearly demonstrates the effectiveness of each component introduced across rounds. Across all shot settings, we observe a monotonic improvement, confirming that each additional component contributes positively.

% Incorporating shot-agnostic domain adaptation on top of the pretrained model leads to larger gains on more challenging domains, while yielding relatively moderate improvements on easier datasets. This indicates that domain adaptation effectively reduces domain discrepancies, particularly for difficult or highly shifted distributions.

% Introducing shot-dependent fine-tuning results in the most significant performance gains, especially under low-shot settings. This highlights that adapting to shot-specific distributions with pseudo-labels is crucial when labeled data is scarce.

% Expanding synthetic data provides consistent and stable improvements across all settings. Although the gains are moderate, they are reliable, indicating improved generalization. This suggests that data scaling complements pseudo-labeling by reducing overfitting and increasing data diversity.

% The final stage further enhances performance through additional synthetic data scaling, image processing-based color augmentation, and test-time augmentation. While the improvements are incremental, they are consistently observed across all benchmarks, validating that strong color augmentations and inference-time ensembling further improve robustness.

% \begin{table}[h]
% \centering
% \begin{tabular}{cccccc}
% \toprule
% & \textbf{Round} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{1-shot}}
% & R0 & \texttt{21.243} & \texttt{52.399} & \texttt{14.011} \\
% & R1 & \texttt{22.319} & \texttt{53.014} & \texttt{18.248} \\
% & R2 & \texttt{25.924} & \texttt{53.544} & \texttt{26.534} \\
% & R3 & \texttt{27.754} & \texttt{56.265} & \texttt{29.386} \\
% & R4 & \textbf{{\texttt{30.488}}} & \textbf{\texttt{56.279}} & \textbf{\texttt{30.924}} \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{5-shot}}
% & R0 & \texttt{22.319} & \texttt{52.399} & \texttt{15.713} \\
% & R1 & \texttt{25.238} & \texttt{53.077} &  \texttt{18.545} \\
% & R2 & \texttt{34.150} & \texttt{56.239} &  \texttt{26.271} \\
% & R3 & \texttt{37.339} & \texttt{56.434} &  \texttt{27.882}\\
% & R4 & \textbf{{\texttt{39.375}}} & \textbf{\texttt{56.796}} & \textbf{\texttt{27.952}} \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{10-shot}}
% & R0 & \texttt{22.319} & \texttt{53.014} & \texttt{13.236} \\
% & R1 & \texttt{25.549} & \texttt{53.911} & \texttt{16.292} \\
% & R2 & \texttt{33.636} & \texttt{51.463} & \texttt{27.568} \\
% & R3 & \texttt{35.367} & \texttt{55.349} & \texttt{28.917} \\
% & R4 & \textbf{{\texttt{37.142}}} & \textbf{\texttt{55.937}} & \textbf{\texttt{30.666}} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets.}
% \label{tab:results}
% \end{table}

% \section{Contribution}

They propose a parameter-efficient domain adaptation approach that preserves pretrained knowledge while mitigating catastrophic forgetting. In addition, they develop an iterative self-improvement procedure that operates without direct human-provided labels, ensuring full compliance with the challenge rules by minimizing human involvement that could be considered unfair or misleading in FSOD settings. Furthermore, beyond exploring image processing-based augmentation policies, they demonstrate that incorporating synthetic data generated by recent diffusion models provides substantial benefits in CD-FSOD scenarios.


% \newpage

% \noindent \textbf{{Other details}}
% \begin{itemize}
% \item Planned submission at NTIRE 2026 workshop: No.
% \item General comments and impressions: Well-motivated, effectively highlighting the challenges of learning under scarce data.
% \item Suggestions for future CD-FSOD challenges: None.
% \item Other comments: None.
% \end{itemize}

% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{references}
% }

% \end{document}


==> ntire26/teams/team7_NUDT-RSIP/affiliation.tex <==
\subsection*{NUDT-RSIP}

\noindent\textit{\textbf{Title: }} NUDT-RSIP\\
\noindent\textit{\textbf{Members: }} \\
Zekang Fan$^{1}$ (\href{mailto:fzk1055279850@qq.com}{fzk1055279850@163.com}),\\
Junjie Liu$^{1}$ (\href{mailto:junjieliucst@163.com}{junjieliucst@163.com})\\
\noindent\textit{\textbf{Affiliations: }} \\
$^1$National University of Defense Technology, China

==> ntire26/teams/team7_NUDT-RSIP/main.tex <==

% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% \let\oldtexttt\texttt
% \renewcommand{\texttt}[1]{\oldtexttt{\hyphenchar\font=\defaulthyphenchar #1}}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\-DDR-}

% \author{Zekang Fan\\
% National University of Defense Technology\\
% Changsha, China, 410073\\
% {\tt\small fzk1055279850@qq.com}
% \and
% Junjie Liu\\
% National University of Defense Technology\\
% Changsha, China, 410073\\
% {\tt\small junjieliucst@163.com}
% }

% \maketitle

% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{NUDT-RSIP} - \texttt{7}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{NUDT-RSIP}
%     \item Team leader (contact): \texttt{\\Zekang Fan}, \texttt{fzk1055279850@qq.com}
%     \item Team members: \texttt{Hailong Yu, Junjie Liu, Tianfang Han, Changyuan Fan, Zihan Tang}
%     \item Method name / nickname: \texttt{DDR}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{\\\url{https://github.com/Catalpa-Hahn/NTIRE2026\_NUDT-RSIP.git}\\\url{https://pan.baidu.com/s/1hY3AxUESGXlUYwV7wIQwAw?pwd=dw1y}}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/Catalpa-Hahn/NTIRE2026_NUDT-RSIP.git}{https://github.com/Catalpa-Hahn/NTIRE2026\_NUDT-RSIP.git}\\
% \noindent Models / weights link: \href{https://pan.baidu.com/s/1hY3AxUESGXlUYwV7wIQwAw?pwd=dw1y}{https://pan.baidu.com/s/1hY3AxUESGXlUYwV7wIQwAw?pwd=dw1y}\\
% \noindent Reproduction instructions (brief): \texttt{bash run.sh}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: \texttt{NUDT-RSIP}
% \item Team leader: \texttt{Zekang Fan}
% \item Affiliation / contact: \texttt{\\National University of Defense Technology, fzk1055279850@qq.com}
% \item Team members: \texttt{Hailong Yu, Junjie Liu, Tianfang Han, Changyuan Fan, Zihan Tang}
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \texttt{DDR}
% \item Final score (if available): \texttt{131.4052}
% \item Submission link: \texttt{https://github.com/Catalpa-Hahn/NTIRE2026\_NUDT-RSIP.git}
% \end{itemize}
\subsection{NUDT-RSIP}
\subsubsection{Method overview}
% (Optional) Add a method figure if you have one.

\begin{figure}[!htbp]
\centering
% 定义图片路径变量，便于维护和修改
\def\figPath{teams/team7_NUDT-RSIP/images/NTIRE-ao.pdf}
\IfFileExists{\figPath}{
  \includegraphics[width=1.\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{fig1.png} (or .pdf/.jpg) in \texttt{teams/team12_J_G_team/images/} and check filename.
  }}
}
\caption{Overall pipeline of \texttt{DDR}.}
\label{fig:method144}
\end{figure}


\noindent \textbf{High-level idea:} As illustrated in Fig.~\ref{fig:method144}, they propose a synergistic strategy integrating data augmentation, model distillation, and two-stage fine-tuning to systematically address data scarcity and domain shift in cross-domain few-shot object detection. At the data level, they employ Domain-RAG to enrich the diversity of the support set and leverage a powerful DINOv3 model to re-label unlabeled data, generating high-quality pseudo-labels to enhance supervision. For the model architecture, they adopt DINOv3-ConvNeXt-Large as the feature extraction backbone combined with an RT-DETR head, balancing strong representational capacity with improved detection accuracy. Finally, a two-stage fine-tuning scheme is designed: the pretrained model is first adapted on Drone Vehicle and URPC2020 datasets, followed by target-specific fine-tuning on the augmented support set. This multi-level framework enables robust generalization in complex cross-domain scenarios under extremely limited annotation budgets.\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} They propose a unified data enhancement paradigm that combines Domain-RAG for support set diversification with DINOv3-driven pseudo-labeling to mitigate annotation sparsity in few-shot learning.
    \item \textbf{Contribution 2:}  They introduce a high-performance DINOv3-ConvNeXt-Large feature extractor with knowledge distillation to transfer robust representations while adapting to novel target domains.
    \item \textbf{Contribution 3:} They design a two-stage progressive fine-tuning strategy that first adapts on Drone Vehicle and URPC2020 datasets before target-specific fine-tuning, effectively bridging the domain gap under limited annotations.
\end{itemize}

\subsubsection{Model architecture}
Describe the backbone, detector head, any added modules, and where they are inserted.
\begin{itemize}
    \item Backbone: DINOv3-ConvNeXt-Large
    \item Detector: RT-DETR
    \item Additional components: Domain-RAG
\end{itemize}



% %%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \begin{thebibliography}{1}

% \bibitem{fu2025cross}Fu, Y., Qiu, X., Ren, B., Fu, Y., Timofte, R., Sebe, N., Yang, M.-H., Gool, L. V., Zhang, K., Nong, Q., Dong, X., Gao, H., Zhou, X., Pan, J., Liu, Y., He, X., Li, J., Sun, Y., Huang, X., … Li, W. (2025). NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results (arXiv:2504.10685). arXiv. https://doi.org/10.48550/arXiv.2504.10685

% \bibitem{}Fu, Y., Wang, Y., Pan, Y., Huai, L., Qiu, X., Shangguan, Z., … Jiang, X. (2025). Cross-domain few-shot object detection via enhanced open-set object detector. European Conference on Computer Vision, 247–264. Springer.

% \bibitem{}Qiu, X., Fu, Y., Jiawei, G., Ren, B., Pan, J., Fu, Y., … Others. (2026). NTIRE 2026 challenge on cross-domain few-shot object detection: methods and results. CVPRW.

% \bibitem{}Siméoni, O., Vo, H. V., Seitzer, M., Baldassarre, F., Oquab, M., Jose, C., Khalidov, V., Szafraniec, M., Yi, S., Ramamonjisoa, M., Massa, F., Haziza, D., Wehrstedt, L., Wang, J., Darcet, T., Moutakanni, T., Sentana, L., Roberts, C., Vedaldi, A., … Bojanowski, P. (2025). DINOv3 (arXiv:2508.10104). arXiv. https://doi.org/10.48550/arXiv.2508.10104

% \bibitem{}Li, Y., Qiu, X., Fu, Y., Chen, J., Qian, T., Zheng, X., Paudel, D. P., Fu, Y., Huang, X., Gool, L. V., \& Jiang, Y.-G. (2025). Domain-RAG: Retrieval-Guided Compositional Image Generation for Cross-Domain Few-Shot Object Detection (arXiv:2506.05872). arXiv. https://doi.org/10.48550/arXiv.2506.05872

% \bibitem{}Zhao, Y., Lv, W., Xu, S., Wei, J., Wang, G., Dang, Q., Liu, Y., \& Chen, J. (2024). DETRs Beat YOLOs on Real-time Object Detection (arXiv:2304.08069). arXiv. https://doi.org/10.48550/arXiv.2304.08069

% \bibitem{}Liu, Z., Mao, H., Wu, C.-Y., Feichtenhofer, C., Darrell, T., \& Xie, S. (2022). A ConvNet for the 2020s (arXiv:2201.03545). arXiv. https://doi.org/10.48550/arXiv.2201.03545

% \end{thebibliography}


% % If you have a .bib file, comment thebibliography above and use:
% % {\small
% % \bibliographystyle{ieee_fullname}
% % \bibliography{egbib}
% % }

% \end{document}


==> ntire26/teams/team8_Intellindust_AI_Lab/affiliation.tex <==
\subsection*{Intellindust AI Lab}
\noindent\textit{\textbf{Title: }} ZAP: Boosting Few-shot Object Detection with Auto-selected Zero-shot Pseudo Labels\\
\noindent\textit{\textbf{Members: }} \\
Xuanlong Yu$^1$ (\href{mailto:yuxuanlong@intellindust.com}{yuxuanlong@intellindust.com}),\\
Youyang Sha$^1$ (\href{mailto:shayouyang@intellindust.com}{shayouyang@intellindust.com}),\\
Longfei Liu$^1$ (\href{mailto:liulongfei@intellindust.com}{liulongfei@intellindust.com}),\\
Di Yang$^2$ (\href{mailto:di.yang@ustc.edu.cn}{di.yang@ustc.edu.cn}),\\
Xi Shen$^1$ (\href{mailto:shenxi@intellindust.com}{shenxi@intellindust.com})\\
\noindent\textit{\textbf{Affiliations: }} \\
$^1$Intellindust AI Lab\\
$^2$Suzhou Institute for Advanced Research, USTC

==> ntire26/teams/team8_Intellindust_AI_Lab/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% %\usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}
% \usepackage{ulem}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\ZAP: Boosting Few-shot Object Detection with \uline{A}uto-selected \uline{Z}ero-shot \uline{P}seudo Labels}

% \author{
%     Xuanlong Yu$^1$ \quad 
%     Youyang Sha$^1$ \quad 
%     Longfei Liu$^1$ \quad 
%     Di Yang$^{2}$ \quad 
%     Xi Shen$^{1}$ \\[6pt] 
%     $^1$Intellindust AI Lab \qquad
%     $^2$Suzhou Institute for Advanced Research, USTC
% }

% \maketitle

% \section{Introduction}




% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% Add CC recipients here (optional).\\
% example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{TEAM\_NAME} - \texttt{TEAM\_ID}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{TEAM\_NAME}
%     \item Team leader (contact): \texttt{NAME}, \texttt{EMAIL}
%     \item Team members: \texttt{MEMBER\_1, MEMBER\_2, ...}
%     \item Method name / nickname: \texttt{METHOD\_NAME}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

\subsection{Intellindust AI Lab}
\subsubsection{Proposed Method}

% (Optional) Add a method figure if you have one.


They generate pseudo-labels for three datasets in a zero-shot manner using Qwen3.5-35B-A3B~\cite{qwen3.5} and SAM3~\cite{carion2026sam}, where only class-name text prompts are provided as input. The overall framework is given in Fig.~\ref{fig:method6}.

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.\linewidth]{teams/team8_Intellindust_AI_Lab/images/pipeline2.pdf}
\caption{Overall pipeline of \texttt{ZEP}.}
\label{fig:method6}
\end{figure}

To automatically select more reliable pseudo-labels for each dataset, they propose a metric termed FSOD-mAP. Specifically, for each dataset, they compute the IoU between pseudo-labels and the few-shot ground-truth boxes (1/5/10-shot). Predictions with IoU $\leq$ 0.3 and matching class labels are filtered out to suppress noisy false positives. They then compute mAP on the remaining predictions, which serves as a proxy for pseudo-label quality. Based on this criterion, they select the pseudo-label source with higher FSOD-mAP (Dataset1 and Dataset2 favor SAM3, while Dataset3 favors Qwen3.5). Additionally, for SAM3-generated pseudo-labels, they further discard predictions with confidence scores lower than 0.8 (Qwen3.5 does not provide confidence scores).

Next, they merge pseudo-labels with the few-shot ground-truth annotations. To avoid redundancy, pseudo-labels that have an IoU greater than 0.8 with ground-truth boxes of the same class are removed.

They explore two strategies for constructing training and validation sets: \textit{Strategy 1}: The merged dataset (pseudo-labels + few-shot annotations) is split into training and validation sets with a ratio of 8:2.
\textit{Strategy 2}: The merged training set is used for training, while pseudo-labels generated on the original test set (without fusion, due to the absence of ground truth) are used as the validation set.

They then fine-tune the two MMGroundingDINO-L~\cite{zhao2024open} models with the Hybrid Ensemble Decoder (HED)~\cite{yu2026acloser}, which is proposed by their team (accepted by CVPR 2026, forthcoming). During inference, they apply test-time augmentation (TTA) with horizontal flipping and Soft-NMS for each model. Finally, predictions from the two models (trained under the two strategies) are combined using Soft-NMS to produce the final results. 
% Results are shown in Table~\ref{tab:results}.


% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & Baseline (Zero-shot)  & \texttt{Open} & \texttt{37.5} & \texttt{52.8} & \texttt{28.3} \\
% & Ours (\texttt{ZEP}) & \texttt{Open} & \texttt{39.6} & \texttt{53.4} & \texttt{44.9} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & Baseline (Zero-shot)  & \texttt{Open} & \texttt{37.5} & \texttt{52.8} & \texttt{28.3} \\
% & Ours (\texttt{ZEP}) & \texttt{Open} & \texttt{43.0} & \texttt{53.6} & \texttt{45.8} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & Baseline (Zero-shot)  & \texttt{Open} & \texttt{37.5} & \texttt{52.8} & \texttt{28.3} \\
% & Ours (\texttt{ZEP}) & \texttt{Open} & \texttt{45.3} & \texttt{53.3} & \texttt{47.4} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Baseline is the zero-shot results given by SAM3 (dataset1 and dataset2) and Qwen3.5-35B-A3B (dataset3).}
% \label{tab:results}
% \end{table}



%%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% \small
% \begin{thebibliography}{1}
% \bibitem{fu2025cross}
% Author(s).
% \newblock Paper title.
% \newblock Conference/Journal, Year. (Placeholder; replace with real references.)
% \end{thebibliography}


% % If you have a .bib file, comment thebibliography above and use:
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> ntire26/teams/team9_FDUROILab_Lenovo/affiliation.tex <==
\subsection*{FDUROILab\_Lenovo}
\noindent\textit{\textbf{Title: }} FDUROILab\_Lenovo\\
\noindent\textit{\textbf{Members: }} \\
Lingyi Hong$^{1}$ (\href{mailto:lyhong22@m.fudan.edu.cn}{lyhong22@m.fudan.edu.cn}),\\
Mingxi Cheng$^{1}$ (\href{mailto:mxchen24@m.fudan.edu.cn}{mxchen24@m.fudan.edu.cn}),\\
Xingqi He$^{1}$,\\
Runze Li$^{2}$ (\href{mailto:lirz7@lenovo.com}{lirz7@lenovo.com}),\\
Xingdong Sheng$^{2}$ (\href{mailto:shengxd1@lenovo.com}{shengxd1@lenovo.com}),\\
Wenqiang Zhang$^{1,3}$ (\href{mailto:wqzhang@fudan.edu.cn}{wqzhang@fudan.edu.cn})\\
\noindent\textit{\textbf{Affiliations: }} \\
$^1$Shanghai Key Lab of Intelligent Information Processing, School of Computer Science, Fudan University, China\\
$^2$Lenovo Research\\
$^3$College of Intelligent Robotics and Advanced Manufacturing, Fudan University, China

==> ntire26/teams/team9_FDUROILab_Lenovo/main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% % \usepackage[review]{cvpr}      % To produce the REVIEW version
% \usepackage{cvpr}              % To produce the CAMERA-READY version
% %\usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage[table]{xcolor} % 用于给表格单元格添加颜色

% % It is strongly recommended to use hyperref, especially for the review version.
% % hyperref with option pagebackref eases the reviewers' job.
% % Please disable hyperref *only* if you encounter grave issues, e.g. with the
% % file validation for the camera-ready version.
% %
% % If you comment hyperref and then uncomment it, you should delete
% % ReviewTempalte.aux before re-running LaTeX.
% % (Or just hit 'q' on the first LaTeX run, let it finish, and you
% %  should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}


% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}




% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\cvprPaperID{*****} % *** Enter the CVPR Paper ID here
% \def\confName{CVPR}
% \def\confYear{2025}


% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{NTIRE 2025 CD-FSOD Challenge Factsheet\\-FDUROILab Lenovo-}

% % \author{Lingyi Hong\\
% % Fudan University\\
% % {\tt\small lyhong22@m.fudan.edu.cn}
% % % For a paper whose authors are all at the same institution,
% % % omit the following lines up until the closing ``}''.
% % % Additional authors and addresses can be added with ``\and'',
% % % just like the second author.
% % % To save space, use either the email address or home page, not both
% % \and
% % Second Author\\
% % Institution2\\
% % {\tt\small secondauthor@i2.org}
% % \and
% % Xinyu Zhou \\
% % Fudan University\\
% % {\tt\small zhouxinyu20@fudan.edu.cn}
% % \and
% % Runze Li \\
% % Lenovo Research \\
% % {\tt\small lirz7@lenovo.com}
% % \and
% % Xingdong Sheng \\
% % Lenovo Research \\
% % {\tt\small shengxd1@lenovo.com}
% % \and
% % Wenqiang Zhang \\
% % Fudan University \\
% % {\tt\small wqzhang@fudan.edu.cn}
% % }


% \author{Lingyi Hong\textsuperscript{\rm 1}~
%         Mingxi Cheng \textsuperscript{\rm 1}~
%         Xingqi He \textsuperscript{\rm 1}~
%         Runze Li\textsuperscript{\rm 2} ~
%         Xingdong Sheng\textsuperscript{\rm 2} ~
%         Wenqiang Zhang\textsuperscript{\rm 1,3}\thanks{Corresponding Author} ~
%         \\
%         \textsuperscript{\rm 1}~Shanghai Key Lab of Intelligent Information Processing, \\School of Computer Science, Fudan University, Shanghai, China\\
%         \textsuperscript{\rm 2}~Lenovo Research\\
%         \textsuperscript{\rm 3}~College of Intelligent Robotics and Advanced Manufacturing, Fudan University, Shanghai, China \\
%         {\tt\small \{lyhong22, mxchen24\}@m.fudan.edu.cn, \{lirz7, shengxd1\}@lenovo.com, wqzhang@fudan.edu.cn}
% }

% \maketitle

% \input{sec/1_intro}
% \input{sec/2_method}

% %%%%%%%%% REFERENCES
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


\subsection{FDUROILab Lenovo}
\subsubsection{Proposed Method}


% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{teams/team9_FDUROILab_Lenovo/figure1.pdf} 
%     \caption{Overview of our efficient tuning and inference.}
%     \label{fig:tuning}
% \end{figure*}



To significantly enhance the model’s adaptability in complex cross-domain scenarios, the team proposes an efficient fine-tuning strategy tailored for the open-vocabulary detection model. Their approach leverages diverse data augmentation techniques to expand the limited training set and improve the model’s ability to recognize novel objects in the target domain using the provided k-shot annotated samples.

\begin{figure}[h]
    \centering
    \def\figPath{teams/team9_FDUROILab_Lenovo/figure1.pdf}
    \IfFileExists{\figPath}{
        \includegraphics[width=\columnwidth]{\figPath}
    }{
        \fbox{\parbox[c][0.22\textheight][c]{\columnwidth}{
        \centering \textbf{Figure Placeholder (Tuning \& Inference)}\\
        Put \texttt{figure1.pdf} (or .png/.jpg) in \texttt{teams/team9_FDUROILab_Lenovo/} and check filename.
        }}
    }
    \caption{Overview of their efficient tuning and inference.}
    \label{fig:tuning}
\end{figure}

Given a k-shot setting, where k represents the number of provided object samples, they employ a structured fine-tuning pipeline, which is shown in Figure~\ref{fig:tuning}. (1) \textbf{Object Cropping and Augmentation.} Using the provided bounding boxes of k-shot examples, they first crop the target objects from the original images. The cropped objects are then subjected to various data augmentation techniques, including flipping, rotation, grayscale conversion, and other transformations, to introduce diversity and improve generalization. (2) \textbf{Object Rescaling and Random Pasting.} They randomly rescale the augmented objects to different sizes and paste these transformed objects onto the original images at different locations. This step simulates new object placements and enhances the model’s robustness to variations in object appearance and context. (3) \textbf{Fine-Tuning with Augmented Data.} They finetune the open-vocabulary detection model with the augmented images. This enables the vision components of the detector to better adapt to objects in the target domain, even with minimal labeled examples. Additionally, the augmented data effectively increases the number of training samples, mitigating the few-shot learning limitation and improving overall detection performance.

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{teams/team9_FDUROILab_Lenovo/figure2.pdf} 
%     \caption{Post Processing.}
%     \label{fig:post}
% \end{figure*}


% \begin{table*}[h] 
%     \centering 
    
%     \caption{Results from Leaderboard}
%     \label{tab:leaderboard}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lcccccccccc} 
%         \toprule 
%         User & final\_score & D1\_1shot & D1\_5shot & D1\_10shot & D2\_1shot & D2\_5shot & D2\_10shot & D3\_1shot & D3\_5shot & D3\_10shot \\
%         \midrule 
%         \rowcolor{gray!20}
%         FDUROILab\_Lenovo (ours) & 217.22 & 	57.04 &	57.15 &	58.08 &	59.23 &	59.23 &	59.23 &	45.23 &	46.17 &	48.77 \\

%         zouyyds & 192.79 & 34.61 & 41.14 & 42.05 & 63.25 & 63.00 & 61.29 & 39.71 & 47.43	& 48.29 \\
%         NJUST-KMG & 191.37 & 35.62 & 47.52 & 46.22 & 60.41 & 60.51 & 61.11 & 40.08 & 42.01 & 44.54 \\
        
%         \bottomrule 
%     \end{tabular}
%     }
% \end{table*}


Since their approach utilizes the open-vocabulary detection model, which fundamentally relies on vision-language alignment, it requires access to accurate target category labels during inference, as shown in Figure~\ref{fig:tuning}. To obtain these context-rich labels, they utilize Qwen3-VL~\cite{bai2025qwen3} to generate descriptive textual representations of the target categories. The retrieved target labels from Qwen3-VL are then used as textual input to guide the detection process. Finally, they adopt the detection model to identify and classify objects in the test images based on these enhanced text-based prompts.


Although modern vision-language detectors possess strong generalization capabilities, their performance on the challenging cross-domain test set remains suboptimal in certain cases. Upon further analysis, they found that while the detector can successfully localize most objects, its primary weakness lies in classification errors rather than detection failures. This indicates that the detector still struggles with fine-grained classification when adapting to objects in a new domain. To address this issue, they introduce Qwen3-VL as an auxiliary classifier to refine the final predictions, which is illustrated in Figure~\ref{fig:post}.




Specifically, for each test image, they construct a multimodal prompt comprising the target scene and a set of representative example images for all candidate categories. By leveraging these example images as visual prompts, they instruct Qwen3-VL to describe the objects present in the scene and output a refined list of categories that are likely to appear. After that, they refine the output of the detection model using one of two strategies: (1) \textbf{Filtering.} Remove objects that are classified incorrectly by the detector and are not listed by Qwen3-VL. (2) \textbf{Reclassification.} Assign all detected objects to one of the categories predicted by Qwen3-VL, ensuring consistency between the detected bounding boxes and the high-level scene understanding of the multimodal model. The choice between these two strategies depends on the specific test dataset, as detailed in the Implementation Details. By leveraging Qwen3-VL and visual prompting as a post-processing step, they effectively correct classification errors and enhance the model’s performance on unseen domains, leading to more accurate and reliable object detection results.

\begin{figure}[h]
    \centering
    \def\figPath{teams/team9_FDUROILab_Lenovo/figure2.pdf}
    \IfFileExists{\figPath}{
        \includegraphics[width=\columnwidth]{\figPath}
    }{
        \fbox{\parbox[c][0.22\textheight][c]{\columnwidth}{
        \centering \textbf{Figure Placeholder (Post Processing)}\\
        Put \texttt{figure2.pdf} (or .png/.jpg) in \texttt{teams/team9_FDUROILab_Lenovo/} and check filename.
        }}
    }
    \caption{Post Processing.}
    \label{fig:post}
\end{figure}

\subsubsection{Training Details}

They use the open-vocabulary detection model as the baseline detection model. They utilize Qwen3-VL-235B-A22B~\cite{bai2025qwen3} as their MLLM for label generation and post-processing. Their fine-tuning experiments are conducted on 8 NVIDIA RTX 3090 GPUs, with a batch size of 8 and a base learning rate of 1e-6. During the optimization process, the \texttt{text\_model} is completely frozen, and an \texttt{lr\_mult} of 0.01 is applied to it. They experiment with different numbers of training iterations across datasets and few-shot settings. For dataset1 and dataset3, they fine-tune the model for 30, 50, and 100 batches under 1-shot, 5-shot, and 10-shot settings. For dataset2, no fine-tuning is performed.

To maximize classification accuracy, they adopt dataset-specific post-processing strategies. For dataset1, they reclassify all detected objects into one of the categories predicted by Qwen3-VL. For dataset3, they filter out any detected objects that do not belong to the MLLM-predicted categories. For dataset2, since it contains only a single object category, they do not perform additional classification. However, they apply a specific filtering step: they eliminate overly large detection boxes, which are likely incorrect, as objects in dataset2 are generally small. Besides, they also apply Non-Maximum Suppression (NMS) to suppress redundant or overlapping bounding boxes across all datasets. These dataset-specific strategies ensure that their model achieves optimal performance across different domain shifts and few-shot settings.

% \section{Results}

% We show the results from the official Challenge Leaderboard in Table~\ref{tab:leaderboard}.

% \section{Conclusion}

% In this paper, we tackle cross-domain few-shot object detection (CD-FSOD) by proposing an efficient fine-tuning strategy based on the open-vocabulary detection framework, coupled with a Qwen3-VL-assisted post-processing method. Our approach enhances the model's adaptability to new domains through strategic data augmentation, object transformation, and parameter-efficient tuning, while MLLM-based post-processing significantly improves classification accuracy. Experimental results demonstrate the effectiveness and robustness of our method in few-shot settings.









 

==> ntire26/teams/team9_FDUROILab_Lenovo/sec/1_intro.tex <==
\section{Introduction}

Cross-domain few-shot object detection (CDFSOD)~\cite{fu2025cross,fu2025ntire} is a challenging task that aims to detect specified object categories in a new target domain using only a few labeled examples (e.g., 1-shot, 5-shot, or 10-shot), which differ significantly from the source training set. Unlike traditional object detection, CDFSOD requires models to identify and classify objects beyond the training set while handling severe domain shifts effectively. Compared to standard open-vocabulary detection, CDFSOD presents an additional challenge due to the substantial distribution discrepancies between the novel target domain and the original source domain, which often leads to severe performance degradation.

To address these challenges, we propose an efficient fine-tuning and adaptation approach built upon the robust open-vocabulary detection model. By applying strategic transformations to the highly limited support samples for data augmentation, we significantly enhance the adaptation capability of the detection model to the unseen target domains. Furthermore, we introduce a novel post-processing method leveraging multimodal large language models (MLLMs) to refine the predictions and achieve more precise classification, effectively bridging the domain gap. Our approach aims to maximize the Mean Average Precision (mAP) in cross-domain scenarios with minimal supervision, ensuring superior adaptability and robust detection performance on the unseen test sets.

==> ntire26/teams/team9_FDUROILab_Lenovo/sec/2_method.tex <==
\section{Team Details}
\begin{itemize}
\item Team name: FDUROILab\_Lenovo                    
\item Team leader name: Lingyi Hong                   
\item Team leader email: lyhong22@m.fudan.edu.cn
\item Team members: Mingxi Cheng, Xingqi He, Runze Li, Xingdong Sheng, Wenqiang Zhang
\item Affiliation: Fudan University, Lenovo Research
\item Best scoring entries of the team during the test phase: 217.2
\item Code, pre-trained model, and factsheet download command/link: \href{https://github.com/omnipotent13/FDUROILab\_Lenovo\_2026\_CDFSOD\_Challenge}{github}
\end{itemize}

\section{Code Submission}
\noindent Code link / repository: \href{https://github.com/omnipotent13/FDUROILab\_Lenovo\_2026\_CDFSOD\_Challenge}{github}\\
\noindent Models / weights link: \href{https://huggingface.co/MaggotKing/2026_CDFSOD_FDUROILab_Lenovo}{MaggotKing/2026\_CDFSOD\_FDUROILab\_Lenovo}\\
\noindent Reproduction instructions (brief): You can easily follow the provided README to reproduce our results.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figure1.pdf} 
    \caption{Overview of our efficient tuning and inference.}
    \label{fig:tuning}
\end{figure*}

\section{Method}

In this section, we firstly introduce our approach to enhancing cross-domain few-shot object detection (CD-FSOD) through efficient fine-tuning based on the vision-language open-vocabulary framework. Then, we describe a robust post-processing strategy utilizing a Multimodal Large Language Model (MLLM). 

\subsection{Efficient Tuning}

To significantly enhance the model’s adaptability in complex cross-domain scenarios, we propose an efficient fine-tuning strategy tailored for the open-vocabulary detection model. Our approach leverages diverse data augmentation techniques to expand the limited training set and improve the model’s ability to recognize novel objects in the target domain using the provided k-shot annotated samples.

Given a k-shot setting, where k represents the number of provided object samples, we employ a structured fine-tuning pipeline, which is shown in Figure~\ref{fig:tuning}. (1) \textbf{Object Cropping and Augmentation.} Using the provided bounding boxes of k-shot examples, we first crop the target objects from the original images. The cropped objects are then subjected to various data augmentation techniques, including flipping, rotation, grayscale conversion, and other transformations, to introduce diversity and improve generalization. (2) \textbf{Object Rescaling and Random Pasting.} We randomly rescale the augmented objects to different sizes and paste these transformed objects onto the original images at different locations. This step simulates new object placements and enhances the model’s robustness to variations in object appearance and context. (3) \textbf{Fine-Tuning with Augmented Data.} We finetune the open-vocabulary detection model with the augmented images. This enables the vision components of the detector to better adapt to objects in the target domain, even with minimal labeled examples. Additionally, the augmented data effectively increases the number of training samples, mitigating the few-shot learning limitation and improving overall detection performance.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figure2.pdf} 
    \caption{Post Processing.}
    \label{fig:post}
\end{figure*}

\begin{table*}[h] 
    \centering 
    
    \caption{Results from Leaderboard}
    \label{tab:leaderboard}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccc} 
        \toprule 
        User & final\_score & D1\_1shot & D1\_5shot & D1\_10shot & D2\_1shot & D2\_5shot & D2\_10shot & D3\_1shot & D3\_5shot & D3\_10shot \\
        \midrule 
        \rowcolor{gray!20}
        FDUROILab\_Lenovo (ours) & 217.22 & 	57.04 &	57.15 &	58.08 &	59.23 &	59.23 &	59.23 &	45.23 &	46.17 &	48.77 \\

        zouyyds & 192.79 & 34.61 & 41.14 & 42.05 & 63.25 & 63.00 & 61.29 & 39.71 & 47.43	& 48.29 \\
        NJUST-KMG & 191.37 & 35.62 & 47.52 & 46.22 & 60.41 & 60.51 & 61.11 & 40.08 & 42.01 & 44.54 \\
        
        \bottomrule 
    \end{tabular}
    }
\end{table*}

\subsection{Inference}

Since our approach utilizes the open-vocabulary detection model, which fundamentally relies on vision-language alignment, it requires access to accurate target category labels during inference, as shown in Figure~\ref{fig:tuning}. To obtain these context-rich labels, we utilize Qwen3-VL~\cite{bai2025qwen3} to generate descriptive textual representations of the target categories. The retrieved target labels from Qwen3-VL are then used as textual input to guide the detection process. Finally, we adopt the detection model to identify and classify objects in the test images based on these enhanced text-based prompts.

\subsection{Post-Process}

Although modern vision-language detectors possess strong generalization capabilities, their performance on the challenging cross-domain test set remains suboptimal in certain cases. Upon further analysis, we found that while the detector can successfully localize most objects, its primary weakness lies in classification errors rather than detection failures. This indicates that the detector still struggles with fine-grained classification when adapting to objects in a new domain. To address this issue, we introduce Qwen3-VL as an auxiliary classifier to refine the final predictions, which is illustrated in Figure~\ref{fig:post}.

Specifically, for each test image, we construct a multimodal prompt comprising the target scene and a set of representative example images for all candidate categories. By leveraging these example images as visual prompts, we instruct Qwen3-VL to describe the objects present in the scene and output a refined list of categories that are likely to appear. After that, we refine the output of the detection model using one of two strategies: (1) \textbf{Filtering.} Remove objects that are classified incorrectly by the detector and are not listed by Qwen3-VL. (2) \textbf{Reclassification.} Assign all detected objects to one of the categories predicted by Qwen3-VL, ensuring consistency between the detected bounding boxes and the high-level scene understanding of the multimodal model. The choice between these two strategies depends on the specific test dataset, as detailed in the Implementation Details. By leveraging Qwen3-VL and visual prompting as a post-processing step, we effectively correct classification errors and enhance the model’s performance on unseen domains, leading to more accurate and reliable object detection results.

\subsection{Remark}

Our method strictly adheres to the k-shot setting, using only the provided k-shot labeled samples for fine-tuning. We do not incorporate any external detection datasets, additional bounding box annotations, or test set images during training. All improvements to the model are achieved solely through the given few-shot examples and permitted pretrained resources, ensuring full compliance with the competition’s constraints.

\subsection{Implementation Details}

We use the open-vocabulary detection model as our baseline detection model. We utilize Qwen3-VL-235B-A22B~\cite{bai2025qwen3} as our MLLM for label generation and post-processing. Our fine-tuning experiments are conducted on 8 NVIDIA RTX 3090 GPUs, with a batch size of 8 and a base learning rate of 1e-6. During the optimization process, the \texttt{text\_model} is completely frozen, and an \texttt{lr\_mult} of 0.01 is applied to it. We experiment with different numbers of training iterations across datasets and few-shot settings. For dataset1 and dataset3, we fine-tune the model for 30, 50, and 100 batches under 1-shot, 5-shot, and 10-shot settings. For dataset2, we do not perform any fine-tuning. 

To maximize classification accuracy, we adopt dataset-specific post-processing strategies. For dataset1, we reclassify all detected objects into one of the categories predicted by Qwen3-VL. For dataset3, we filter out any detected objects that do not belong to the MLLM-predicted categories. For dataset2, since it contains only a single object category, we do not perform additional classification. However, we apply a specific filtering step: we eliminate overly large detection boxes, which are likely incorrect, as objects in dataset2 are generally small. Besides, we also apply Non-Maximum Suppression (NMS) to suppress redundant or overlapping bounding boxes across all datasets. These dataset-specific strategies ensure that our model achieves optimal performance across different domain shifts and few-shot settings.

\section{Results}

We show the results from the official Challenge Leaderboard in Table~\ref{tab:leaderboard}.

\section{Conclusion}

In this paper, we tackle cross-domain few-shot object detection (CD-FSOD) by proposing an efficient fine-tuning strategy based on the open-vocabulary detection framework, coupled with a Qwen3-VL-assisted post-processing method. Our approach enhances the model's adaptability to new domains through strategic data augmentation, object transformation, and parameter-efficient tuning, while MLLM-based post-processing significantly improves classification accuracy. Experimental results demonstrate the effectiveness and robustness of our method in few-shot settings.









 



==> teams/team00_Example/affiliation.tex <==
\subsection*{Example}
\noindent\textit{\textbf{Title: }}Cross-Domain Few-Shot Object Detection via Enhanced Open-Set Object Detector\\
\noindent\textit{\textbf{Members: }} \\
Yuqian Fu$^1$ (\href{mailto:yuqian.fu@insait.ai}{yuqian.fu@insait.ai}),\\
Yu Wang$^2$, \\
Yixuan Pan$^3$, \\
Xingyu Qiu$^2$, \\
$^1$ INSAIT \\
$^2$ Fudan University  \\
$^3$ Southeast University\\



==> teams/team00_Example/main.tex <==
\subsection{Example}
\subsubsection{Proposed Method}
We propsose a novel CD-ViTO method for the CD-FSOD, under the close-set setting, which only takes COCO as source data and transfer the model to novel target. 
As in Fig.~\ref{fig:framework}, we build our CD-ViTO upon one open-set detector (DE-ViT) and finetune our method using few labeled instances of target domain. Modules in blue are inherited from DE-ViT while modules in orange are proposed by us. New improvements include learnable instance features, instance reweighting, domain prompter, and finetuning;  

\begin{figure}[h]
\vspace{-0.1in}
\centering	{\includegraphics[width=1.\linewidth]{teams/team00_Example/framework.jpg}}
\vspace{-0.1in}
\caption{(a) Overall framework of CD-ViTO. \label{fig:framework} 
}
\vspace{-0.15in}
\end{figure}

Specifically, given $S$ and $q$ as input, we perform the same steps as DE-ViT to obtain instance features $F_{ins} =\{F_{ins}^{ob}, F_{ins}^{bg}\}$, region proposals $R_{q}$, visual features $F_{q}$, and ROI features $F_{q_{roi}}$.
But different from directly averaging $F_{ins}^{ob}$ to obtain class prototypes $F_{pro}^{ob}$ for objects, we first utilize our $M_{LIF}$ to make the precalculated $F_{ins}$ learnable and adapt them by performing the disentangled detection tasks i.e., the localization task supervised by $\mathcal{L}_{loc}$ and the classification task supervised by $\mathcal{L}_{cls}$. 
we apply our $M_{LR}$ to reweight the weights of object instances features $F_{ins}^{ob}$. Generally, $M_{LR}$ is expected to assign higher values to the high-quality instances with slight IB. In this way, the high-quality instances could contribute more to its class prototype. The $M_{LR}$ is inserted after the $M_{LIF}$ and is optimized use the same $\mathcal{L}_{loc}$, $\mathcal{L}_{cls}$.
In addition, to make the model more robust to the changing styles, our proposed $M_{DP}$ is applied to synthesize several virtual "domains" $F_{domain}$. The goal of the $M_{DP}$ is to introduce such domain perturbations and force our features to be consistent with different domains. To ensure the diversity of the introduced domains and constrain the domains would not affect the semantics of features, an extra loss $\mathcal{L}_{dp}$ is introduced. The $M_{DP}$ is build upon the object prototypes $F_{pro}^{ob}$ and the $\mathcal{L}_{dp}$ works with the $\mathcal{L}_{loc}$ and $\mathcal{L}_{cls}$ together.

As for finetuning, we finetune the top two modules i.e., the $M_{DET}$ and $M_{CLS}$. 
via the object function $\mathcal{L}$ as:
\begin{equation}\label{eq:loss}
\mathcal{L}  = \mathcal{L}_{loc} + \mathcal{L}_{cls} + \mathcal{L}_{dp}.
\end{equation}


\noindent \textbf{Learnable Instance Features $M_{LIF}$.}
% The implementation of our learnable instance features $M_{LIF}$ is quiet easy and efficient. 
Given the precalculated instance features $F_{ins} \in \mathcal{R}^{(N \times K + N_{bg}) \times D}$, where $N$, $K$, $N_{bg}$, $D$ represents the number of object classes, the number of shots, the number of background instances, and the dimension of visual features, $M_{LIF}$ defines a new learnable matrix $F_{ins}^{lea}$ with the same size of $F_{ins}$ and use the $F_{ins}$ for initialization. 

\noindent \textbf{Instance Reweighting Module $M_{IR}$.}
Our $M_{IR}$ is proposed to reweight the instances enabling high-quality object instances e.g., objects with slight IB contribute more to the class prototype. 
% The architecture of $M_{IR}$ is shown in Fig.~\ref{fig:framework}(b). 
Given the learnable instance features $F_{ins}^{lea}$ from $M_{LIF}$, we first obtain the object instance features from  $F_{ins}^{lea}$ and denote it as $F_{ins}^{0} \in \mathcal{R}^{N \times K \times D}$. Our $M_{IR}$ has two paths connected in a residual way. 
More specifically, the lower path feeds the $F_{ins}^{0}$ into an MLP module to get the weighted score which is further used to perform the weighted sum on the initial $F_{ins}^{0}$ resulting in the deformed prototypes $F_{ins}^{att} \in \mathcal{R}^{N \times D}$. The upper path performs the average operation on $F_{ins}^{0}$ getting $F_{ins}^{avg} \in \mathcal{R}^{N \times D}$. The final object prototypes $F_{pro}^{ob}$ are represented as $\alpha fc(F_{ins}^{att}) + (1-\alpha)F_{ins}^{avg}$, where the $fc(\cdot)$ denotes a fully connected layer and $\alpha$ is a hyperparameter.  



\noindent \textbf{Domain Prompter $M_{DP}$.}

Given $F_{domain}$ and $F_{pro}^{ob}$, we first propose the domain diversity loss $\mathcal{L}_{domain}$ to force the different domains e.g., $f^{d_{i}}$ and $f^{d_j}$ to be far from each other. Secondly, for a prototype $f_{p_{i}}$ in $F_{pro}^{ob}$, we randomly perturbs it with two various domains $f^{d_{k}}$ and $f^{d_{m}}$ sampled from $F_{domain}$ forming two perturbed prototypes $f_{p_{i}}^{d_{k}}, f_{p_{i}}^{d_{m}}$. The perturbation is done by adding the features e.g., $f_{p_{i}}^{d_{k}} = f_{p_{i}} +f^{d_{k}}$. 
The domain $f^{d_{m}}$ is also added to other object prototypes forming $f_{p_{j}}^{d_{m}}$, where $j = 1, \ldots, N$. 
We constrain that $f_{p_{i}}^{d_{k}}$ and $f_{p_{i}}^{d_{m}}$ should be close to each other while being distant from perturbed prototypes generated from different class prototypes.
This constitutes our prototype consistency loss $\mathcal{L}_{proto}$.  Both the $\mathcal{L}_{domain}$ and $\mathcal{L}_{proto}$ are implemented by the InfoNCE loss.

\subsubsection{Training Details}
we adopt the "pretrain, finetune, and test" pipeline. 
In the case of our CD-ViTO, the base DE-ViT model pretrained on COCO is taken, then the $M_{DET}$, $M_{CLS}$, $M_{LIF}$, $M_{IR}$, and $M_{DP}$ are tuned on novel support images $S$ using the loss as in Eq.~\ref{eq:loss}.
The hyperparameter $N_{bg}$, $\alpha$ ratio of instance reweighting module, $\tau$ temperature for $\mathcal{L}_{proto}$, $\tau$ temperature for $\mathcal{L}_{domain}$  are set as 530, 0.7, 2, 0.1 for all the target datasets. While the value $N_{dom}$ means the number of virtual domains depending on the number of target classes $N$, specifically, we have $N_{dom} = 2*N$.  The hyperparameter Top-K ($K$) in DE-ViT is set as 5. For datasets with number of classes $N$ less than 5, we have $K=N$. We tune the trainable parameters on 1-shot around 80 epochs, and on 5/10-shot around 40 epochs. The SGD with the learning rate as 0.002 is used as the optimizer. Experiments are performed on four RTX3090 GPUs.



==> teams/team11_AIRCAS_MILab/ori.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE
% % \usepackage[review]{cvpr}
% \usepackage{cvpr}
% % \usepackage[pagenumbers]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage[shortlabels]{enumitem}
% \usepackage{multirow}
% \usepackage{rotating}

% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}
% \Crefname{figure}{Figure}{Figures}
% \crefname{figure}{Fig.}{Figs.}

% %%%%%%%%% PAPER ID
% \def\cvprPaperID{*****}
% \def\confName{CVPR}
% \def\confYear{2026}

% \begin{document}

% %%%%%%%%% TITLE
% \title{NTIRE 2026 CD-FSOD Challenge Factsheet\\Semantic-Filtered Domain-RAG and Auto-Tuned GroundingDINO}

% \author{
% Zhenzhao Xing \quad Dandan Zhao \quad Hanzhe Xia \quad Dongdong Lu \quad Zhe Zhang\\
% AIRCAS MILab\\
% {\tt\small xingzhenzhao25@mails.ucas.ac.cn}
% }

% \maketitle

% \section{Introduction}

% This factsheet presents our submission to the NTIRE 2026 Cross-Domain Few-Shot Object Detection (CD-FSOD) Challenge. The challenge targets an extremely data-scarce setting, where the target domains are substantially different from the source distribution and only a very limited number of annotated samples are available for each novel class. Under this setting, detector stability, data quality, and task-specific adaptation become more important than simply increasing training complexity.

% Our solution treats the challenge as nine independent few-shot detection tasks, corresponding to three target datasets under 1-shot, 5-shot, and 10-shot settings. Instead of training a single unified model across all domains and all shot configurations, we fine-tune a dedicated detector for each dataset-shot pair. This design avoids cross-task interference and makes it easier to control class definitions, hyperparameters, checkpoints, and post-processing strategies in a reproducible way.

% The detector is built on GroundingDINO with a Swin-B backbone. Our main effort is devoted to stable cross-domain few-shot adaptation rather than heavy architectural modification. Specifically, the full pipeline combines: (1) task-specific annotation preparation, (2) Domain-RAG based data expansion, (3) semantic filtering for generated backgrounds, (4) automatic configuration generation for GroundingDINO, and (5) dataset-specific post-processing during inference. We also explored a pseudo-label refinement stage, but found that direct inference from the first-stage augmented model was often more reliable under extremely low-shot conditions.

% The provided factsheet, source codes, trained models, and final prediction files are intended to support reproducibility and transparent evaluation. In the final submission, we will provide the corresponding download links and package the factsheet both as a compiled PDF and as a ZIP archive containing the \texttt{.tex} source files.

% \section{Email Final Submission Guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here if needed.\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{AIRCAS MILab} - \texttt{TEAM\_ID}\\

% To obtain the \texttt{TEAM\_ID}, please register in the official Google Sheet and fill in the Team Name, Contact Person, and Contact Email in the first available row.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{AIRCAS MILab}
%     \item Team leader (contact): \texttt{Zhenzhao Xing}, \texttt{xingzhenzhao25@mails.ucas.ac.cn}
%     \item Team members: \texttt{Dandan Zhao (zhaodandan@aitech.edu.cn), Hanzhe Xia (xiahanzhe25@163.com), Dongdong Lu (ludd@aircas.ac.cn), Zhe Zhang (zhangzhe01@aircas.ac.cn)}
%     \item Username on the NTIRE 2026 CodaLab/CodaBench Competition Platform: \texttt{[TO BE FILLED]}
%     \item Method name / nickname: \texttt{SF-DomainRAG + Auto-Tuned GroundingDINO}
%     \item Download methods for the factsheet, code, and pre-trained models: \texttt{[TO BE FILLED]}
% \end{enumerate}

% \noindent The factsheet should be submitted as a compiled PDF together with a ZIP archive containing the \texttt{.tex} source files.

% \section{Code Submission}

% \noindent Code link / repository: \texttt{[TO BE FILLED]}\\
% \noindent Models / weights link: \texttt{[https://pan.baidu.com/s/1kINv-SkBmmM8goOnIfBERA?pwd=utbe]}\\
% \noindent Reproduction instructions (brief): \texttt{Prepare semantically filtered Domain-RAG augmented annotations, automatically generate GroundingDINO configurations for all nine dataset-shot tasks, fine-tune task-specific models, and export json predictions with dataset-specific post-processing.}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}[leftmargin=1.2em]
% \item Team name: \texttt{AIRCAS MILab}
% \item Team leader: \texttt{Zhenzhao Xing}
% \item Affiliation / contact: \texttt{AIRCAS MILab, xingzhenzhao25@mails.ucas.ac.cn}
% \item Team members: \texttt{Zhenzhao Xing (xingzhenzhao25@mails.ucas.ac.cn), Dandan Zhao (zhaodandan@aitech.edu.cn), Hanzhe Xia (xiahanzhe25@163.com), Dongdong Lu (ludd@aircas.ac.cn), Zhe Zhang (zhangzhe01@aircas.ac.cn)}
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \texttt{SF-DomainRAG + Auto-Tuned GroundingDINO}
% \item Final score : \texttt{[150.6085]}
% \item Submission link: \texttt{[TO BE FILLED]}
% \end{itemize}
\subsection{AIRCAS MILab}

\subsubsection{Proposed Method}

% \begin{figure*}[t]
% \centering
% \IfFileExists{teams2026/team11_AIRCAS MILab/method_figure.pdf}{
%   \includegraphics[width=0.95\textwidth]{method_figure.pdf}
% }{
%   \IfFileExists{method_figure.png}{
%     \includegraphics[width=0.95\textwidth]{method_figure.png}
%   }{
%     \IfFileExists{method_figure.jpg}{
%       \includegraphics[width=0.95\textwidth]{method_figure.jpg}
%     }{
%       \fbox{\parbox[c][0.23\textheight][c]{0.95\textwidth}{
%       \centering \textbf{Method Figure Placeholder}\\[4pt]
%       Put \texttt{method\_figure.pdf} (or \texttt{.png}/\texttt{.jpg}) in the same folder and update the filename if needed.
%       }}
%     }
%   }
% }
% \caption{Overall pipeline of our method. Each dataset-shot pair is treated as an independent few-shot task. The support annotations are first expanded with semantically filtered Domain-RAG generated samples, then used to automatically build task-specific GroundingDINO configurations, and finally the detector outputs are filtered with dataset-specific post-processing for submission.}
% \label{fig:method}
% % \end{figure*}
% \begin{figure*}[t]
% \centering
% % 定义统一的基础路径变量，解决多层判断的路径不一致问题
% \def\figBasePath{teams2026/team11_AIRCAS MILab/}
% % 依次检查PDF/PNG/JPG格式，且所有检查/加载路径统一
% \IfFileExists{\figBasePath method_figure.pdf}{
%   \includegraphics[width=0.95\textwidth]{\figBasePath method_figure.pdf}
% }{
%   \IfFileExists{\figBasePath method_figure.png}{
%     \includegraphics[width=0.95\textwidth]{\figBasePath method_figure.png}
%   }{
%     \IfFileExists{\figBasePath method_figure.jpg}{
%       \includegraphics[width=0.95\textwidth]{\figBasePath method_figure.jpg}
%     }{
%       \fbox{\parbox[c][0.23\textheight][c]{0.95\textwidth}{
%       \centering \textbf{Method Figure Placeholder}\\[4pt]
%       Put \texttt{method\_figure.pdf} (or \texttt{.png}/\texttt{.jpg}) in \texttt{teams2026/team11_AIRCAS MILab/} and update the filename if needed.
%       }}
%     }
%   }
% }


\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，便于维护和排查
\def\figPath{teams2026/team11_AIRCAS MILab/method_figure.pdf}
% 增加文件存在性检查，避免图片缺失时报错，同时给出清晰提示
\IfFileExists{\figPath}{
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{}\\
  Put \texttt{} (or .png/.jpg) in the \texttt{images/} folder (relative to main .tex file) and check filename.
  }}
}



\caption{Overall pipeline of our method. Each dataset-shot pair is treated as an independent few-shot task. The support annotations are first expanded with semantically filtered Domain-RAG generated samples, then used to automatically build task-specific GroundingDINO configurations, and finally the detector outputs are filtered with dataset-specific post-processing for submission.}
\label{fig:method11}
\end{figure}


\noindent \textbf{High-level idea:}
Our solution addresses the challenge as nine independent few-shot object detection tasks, corresponding to three target datasets under 1-shot, 5-shot, and 10-shot settings. We adopt GroundingDINO with a Swin-B backbone as the base detector and fine-tune it separately for each dataset-shot pair instead of merging all tasks into a single training set. To alleviate the severe lack of supervision in the few-shot regime, we expand the original support annotations with Domain-RAG generated samples. A lightweight semantic filtering step is introduced before the generated data are merged back into the training set, so that only generated backgrounds that remain semantically compatible with the foreground object are preserved. In addition, we build an automatic configuration generation and parameter tuning pipeline for GroundingDINO, which allows us to manage all nine task-specific settings consistently and reproducibly. During inference, final submission json files are produced with dataset-specific confidence filtering, NMS, and top-\emph{k} control.

\noindent \textbf{Key contributions:}
\begin{itemize}[leftmargin=1.2em]
    \item \textbf{Contribution 1:} We introduce semantic filtering for Domain-RAG generated backgrounds, which reduces semantically mismatched augmentation noise before few-shot detector training.
    \item \textbf{Contribution 2:} We develop an automatic GroundingDINO configuration generation and parameter tuning pipeline for all nine dataset-shot tasks, including data paths, class reconstruction, training hyperparameters, checkpoint handling, and inference settings.
    \item \textbf{Contribution 3:} We employ fully task-specific training and dataset-specific inference post-processing instead of a single unified setting, which improves stability under cross-domain and extremely low-shot conditions.
\end{itemize}

\noindent\textbf{Model architecture}

The detector is based on GroundingDINO and initialized from an official pre-trained checkpoint. We use the Swin-B version as the visual backbone and keep the detector architecture itself largely unchanged. Rather than introducing a heavy architectural modification, we focus on improving the data pipeline and the task adaptation process. In particular, the class definitions are reconstructed automatically from the target few-shot COCO annotations, and the detector head is adapted to the corresponding task. This design keeps the main model stable while allowing robust adaptation to the challenge setting.

\begin{itemize}[leftmargin=1.2em]
    \item Backbone: \texttt{Swin-B}
    \item Detector: \texttt{GroundingDINO}
    \item Additional components: \texttt{Semantic filtering for Domain-RAG augmentation, automatic config generation, and dataset-specific post-processing}
\end{itemize}

\subsubsection{Training details}

The training pipeline is organized around nine independent tasks: dataset1, dataset2, and dataset3 under 1-shot, 5-shot, and 10-shot settings. We do not mix different datasets or different shot settings into a single training set, because their visual domains and supervision scales are clearly different. Each task is therefore trained independently with its own COCO annotation file and its own GroundingDINO configuration.

The original support annotations are first converted into task-specific COCO training files. We then expand them with Domain-RAG generated samples. However, the generated samples are not used blindly. During background generation, some outputs are visually diverse but semantically inconsistent with the foreground object or scene context. To reduce this type of noise, we apply a semantic filtering stage and only retain generated results that remain compatible with the original object semantics. The selected generated images are then copied into the corresponding training directory and merged into the few-shot COCO annotations of the same task.

This produces augmented training files such as \texttt{1\_shot\_domainrag\_aug.json}, \texttt{5\_shot\_domainrag\_aug.json}, and \texttt{10\_shot\_domainrag\_aug.json}. The same principle is applied throughout the pipeline: augmented samples are only merged back into the original dataset-shot task from which they are derived. This prevents cross-dataset contamination and preserves the integrity of the few-shot setting.

GroundingDINO is fine-tuned with AdamW. The learning rate and epoch number are adjusted according to the shot setting and the target dataset. Because the official test annotation file does not contain bounding-box ground truth, we disable the validation stage during training and save checkpoints directly. This avoids meaningless validation loops and reduces unnecessary computation. In practice, this design is more suitable for the challenge setup than forcing a conventional validation protocol on unlabeled test annotations.

We also explored a second-stage pseudo-label re-training scheme. The idea was to use the first-stage detector to predict high-confidence boxes on unlabeled training images, merge them into the augmented annotations, and fine-tune again. While this strategy can recover some missed instances, we observed that in extremely low-shot conditions pseudo-label noise may easily lead to overfitting. Therefore, our final submission relies primarily on the first-stage augmented model and carefully tuned test-time filtering.

\begin{itemize}[leftmargin=1.2em]
    \item Training data: \texttt{dataset1 / dataset2 / dataset3, each with separate 1-shot, 5-shot, and 10-shot task-specific COCO annotations}
    \item Few-shot setting: \texttt{1-shot, 5-shot, and 10-shot; all nine tasks trained independently}
    \item Optimization: \texttt{GroundingDINO fine-tuning with AdamW, task-specific learning rate and epoch settings}
    \item Augmentations: \texttt{Domain-RAG generated data with semantic filtering before annotation merging}
    \item Hardware / runtime: \texttt{Single-GPU training and inference pipeline; exact hardware information can be filled in by the team}
\end{itemize}

\noindent\textbf{Inference details}

Inference is carried out separately for each dataset and each shot setting. The final json results are exported directly from selected GroundingDINO checkpoints. Since no official validation set with bounding-box labels is provided, we support explicit checkpoint and epoch selection during testing. This allows us to compare different checkpoints from the same training run and choose a more reliable model for submission.

We apply dataset-specific post-processing instead of using a single global setting for all domains. In particular, the confidence threshold, NMS IoU threshold, and per-image top-\emph{k} filtering are adjusted separately for dataset1, dataset2, and dataset3. This is important because the three target domains have different background complexity, object scale distributions, and false-positive patterns. In addition, we include image-id alignment and json schema normalization in the export pipeline to ensure that the submission files strictly match the evaluation format required by the challenge.

\begin{itemize}[leftmargin=1.2em]
    \item Test-time settings: \texttt{GroundingDINO export with task-specific checkpoint selection and dataset-specific post-processing}
    \item Ensemble / TTA: \texttt{Not used in the final submission}
    \item Any post-processing: \texttt{Confidence thresholding, per-class NMS, image-id alignment, and per-image top-k filtering}
\end{itemize}

% \subsection{Experimental results}

% Our experiments mainly compare two training strategies: the first-stage model trained on semantically filtered Domain-RAG augmented data, and the second-stage model further refined with pseudo labels. We observe that pseudo-label re-training is not consistently beneficial under the extremely low-shot setting. In several cases, the first-stage augmented model generalizes better than the second-stage model, suggesting that supervision quality is more critical than supervision quantity when the annotation budget is extremely limited.

% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{c l c c c c}
% \toprule
% \textbf{Shot} & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{1-shot}
% & Baseline / Reference & Open & -- & -- & -- \\
% & Ours (SF-DomainRAG + Auto-Tuned GDINO) & Open & 21.264 & 30.8204 & 34.1407 \\
% \midrule
% \multirow{2}{*}{5-shot}
% & Baseline / Reference & Open & -- & -- & -- \\
% & Ours (SF-DomainRAG + Auto-Tuned GDINO) & Open & 57.1144 & 55.3462 & 58.2842 \\
% \midrule
% \multirow{2}{*}{10-shot}
% & Baseline / Reference & Open & -- & -- & -- \\
% & Ours (SF-DomainRAG + Auto-Tuned GDINO) & Open & 18.3613 & 59.6604 & 41.1944 \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1-shot, 5-shot, and 10-shot settings on the three target datasets.}
% \label{tab:results}
% \end{table*}

% \subsection{Ablation and analysis (optional)}

% \begin{itemize}[leftmargin=1.2em]
%     \item Ablation 1: \texttt{Removing the semantic filtering step from Domain-RAG background selection reduces the quality of augmented training samples and makes the few-shot training process less stable.}
%     \item Ablation 2: \texttt{Replacing the automatic GroundingDINO config generation with manual configuration increases the risk of class-mapping errors, wrong annotation paths, and inconsistent parameter settings across the nine tasks.}
%     \item Failure cases: \texttt{Common failure cases include small objects in cluttered backgrounds, confusion between visually similar categories, and overfitting caused by noisy pseudo labels in extremely low-shot conditions.}
% \end{itemize}

% \section{Other details}

% \begin{itemize}[leftmargin=1.2em]
% \item Planned submission of a solution description paper at the NTIRE 2026 workshop: \texttt{Yes}
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{This challenge is well designed to reflect a realistic and difficult cross-domain few-shot detection setting. It clearly exposes the trade-off between strong pre-trained detectors, data augmentation, and the risk of overfitting under very limited supervision.}
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{Providing an official validation split or a small labeled development set would make checkpoint selection and ablation analysis more reliable, especially in the current setting where public test annotations do not provide ground-truth boxes.}
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{A major practical difficulty is that pseudo-label refinement does not always improve performance in an extreme few-shot setting. Better validation support or more explicit development protocols would help distinguish genuine model improvement from pseudo-label overfitting.}
% \end{itemize}

% %%%%%%%%% REFERENCES
% {\small
% \begin{thebibliography}{1}

% \bibitem{fu2025cross}
% Fu, Y., Qiu, X., Ren, B., Fu, Y., Timofte, R., Sebe, N., Yang, M.-H., Van Gool, L., et al.
% \newblock NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.
% \newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, pages 1048--1069, 2025.

% \end{thebibliography}
% }

% \end{document}

==> teams/team12_J_G_team/ori.tex <==
% \subsection{J\_G\_team}
% \subsubsection{Proposed Method}
% % (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams2026/team12_J_G_team/images/fig1.png}{
%   \includegraphics[width=0.95\linewidth]{images/fig1.png}
% }{
%   \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.pdf} (or .png/.jpg) in the same folder and update filename.
%   }}
% }
% \caption{Overall pipeline of Negative Prompting for Few-Shot Object Detection.}
% \label{fig:method}
% \end{figure}
\subsection{J\_G\_team}
\subsubsection{Proposed Method}
% (Optional) Add a method figure if you have one.
\begin{figure}[!htbp]
\centering
% 定义图片路径变量，便于维护和修改
\def\figPath{teams2026/team12_J_G_team/images/fig1.png}
\IfFileExists{\figPath}{
  % 加载和检查使用相同的完整路径，避免路径不一致问题
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  % 占位框：保持原样式，提示用户正确放置图片
  \fbox{\parbox[c][0.22\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{fig1.png} (or .pdf/.jpg) in \texttt{teams2026/team12_J_G_team/images/} and check filename.
  }}
}
\caption{Overall pipeline of Negative Prompting for Few-Shot Object Detection.}
\label{fig:method12}
\end{figure}

\noindent \textbf{High-level idea:} We propose a few-shot object detection method based on FSOD-VFM\cite{feng2025fsodvfm} with two key improvements. First, we incorporate negative sample features generated by randomly shifting and scaling positive bounding boxes, providing the model with additional background context. Second, we replace static class prototypes with query-adaptive cross-attention prototypes, allowing support features to be dynamically weighted according to each query proposal. These two strategies improve the model’s ability to discriminate between foreground and background, and enable it to adapt to intra-class variation, leading to more accurate detection.\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} We introduce negative sample features as additional guidance, helping the model distinguish foreground from background.
    \item \textbf{Contribution 2:} We propose cross-attention prototypes that dynamically adapt to each query proposal, improving matching precision.
\end{itemize}

\noindent \textbf{Model architecture}
\begin{itemize}
    \item \textbf{Detector:} Universal Proposal Network\cite{jiang2024chatrextamingmultimodalllm} is used to generate category‑agnostic bounding box proposals for candidate objects.
    \item \textbf{Mask extraction module:} SAM2 is employed to produce accurate object masks for support annotations, aiding robust feature extraction.
    \item \textbf{Visual Feature Extractor:} We use C-RADIOv4-H as visual feature extractor for whole image.
\end{itemize}

\subsubsection{Training details}
This method is training-free and does not require any task-specific finetuning.

\noindent \textbf{Inference details}
\begin{itemize}
    \item Test-time settings: During preprocessing, C-RADIOv4 resizes all input images so that the longer side is 1260. For all proposals generated by UPN, we select top 100 boxes per image ranked by confidence.
\end{itemize}

% \subsection{Experimental results}
% Experimental results is shown in Table.\ref{tab:results}.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% &  FSOD-VFM & \texttt{(Open)} & \texttt{26.93} & \texttt{58.84} & \texttt{17.28} \\
% & Ours & \texttt{(Open)} & \texttt{26.71} & \texttt{57.99} & \texttt{18.01} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & FSOD-VFM & \texttt{(Open)} & \texttt{38.21} & \texttt{58.70} & \texttt{25.80} \\
% & Ours & \texttt{(Open)} & \texttt{38.46} & \texttt{57.94} & \texttt{26.77} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & FSOD-VFM & \texttt{(Open)} & \texttt{35.03} & \texttt{58.21} & \texttt{27.31} \\
% & Ours & \texttt{(Open)} & \texttt{34.85} & \texttt{57.50} & \texttt{28.86} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Replace placeholders with official numbers.}
% \label{tab:results}
% \end{table}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: No.
% \item General comments and impressions of the NTIRE 2026 challenge: This challenge provides a valuable benchmark for evaluating few-shot object detection under cross-domain scenarios. The task setup is meaningful and reflects practical challenges in real-world applications.
% \item Suggestions for future CD-FSOD challenges: Future editions of the challenge could explore more diverse domain shifts or introduce additional subtracks focusing on efficiency.
% \end{itemize}

%%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> teams/team13_WRC/ori.tex <==
\subsection{WRC}
\subsubsection{Proposed Method}

% \section{Introduction}

% This factsheet template is meant to structure the description of the contributions made by each participating team in the NTIRE 2026 challenge on Cross-Domain Few-Shot Object Detection. 

% Ideally, all the aspects enumerated below should be addressed.
% The provided information, the codes/executables, and the achieved performance on the testing data are used to decide the awardees of the NTIRE 2026 challenge. 

% Reproducibility is a must and needs to be checked for the final test results in order to qualify for the NTIRE awards. 

% The main winners will be decided based on overall performance and a number of awards will go to novel, interesting solutions and solutions that stand up as the best. Please check the competition webpage and forums for more details.

% The winners, the awardees, and the top ranking teams will be invited to co-author the NTIRE 2026 challenge report and to submit papers with their solutions to the NTIRE 2026 workshop. Detailed descriptions are much appreciated.


% The factsheet, source codes/executables e.g., \href{https://github.com/ohMargin/NTIRE2026_CDFSOD}{NTIRE2026\_CDFSOD}\cite{fu2025cross} , trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.


% \noindent The factsheet, source codes/executables, and trained models should be sent to \textbf{all of the NTIRE 2026 challenge organizers} by email.

% \section{Email final submission guide}

% \noindent \textbf{To:}\\
% {xyqiu24@m.fudan.edu.cn}\\
% {yuqian.fu.ai@gmail.com}\\
% {jwgeng25@m.fudan.edu.cn}\\
% {bin.ren.mondo@gmail.com}\\
% {jiancheng.pan.plus@gmail.com}\\
% {zongwei.wu@uni-wuerzburg.de}\\
% {howard.haotang@gmail.com}\\
% {yanweifu@fudan.edu.cn}\\
% {radu.timofte@uni-wuerzburg.de}\\
% {niculae.sebe@unitn.it}\\
% {mohamed.elhoseiny@kaust.edu.sa}\\

% \noindent \textbf{CC:}\\
% % Add CC recipients here (optional).\\
% % example@domain.com\\

% \noindent \textbf{Title:} NTIRE 2026 CD-FSOD Challenge - \texttt{WRC} - \texttt{13}\\

% To get your TEAM\_ID, please register at
% \href{https://docs.google.com/spreadsheets/d/1xfFfhO3D9MGYn0E7nHiL5iI5ttQJu-6ftGTmlbdKC3k/edit?usp=sharing}{Google Sheet}.
% Please fill in your Team Name, Contact Person, and Contact Email in the first empty row from the top of the sheet.

% \noindent Body contents should include:
% \begin{enumerate}[a)]
%     \item Team name: \texttt{WRC}
%     \item Team leader (contact): \texttt{Liwei Zhou}, \texttt{zhouliwei123@nudt.edu.cn}
%     \item Team members: \texttt{Liwei Zhou, Bei Dou, Tao Wu}
%     \item Method name / nickname: \texttt{MQ-Det}
%     \item Code, pre-trained model, and factsheet download command/link: \texttt{LINK / COMMAND}
% \end{enumerate}

% \noindent Factsheet must be a compiled PDF file together with a ZIP containing the \texttt{.tex} source files.

% \section{Code Submission}
% \noindent Code link / repository: \href{https://github.com/your_repo}{https://github.com/ZLW-123-123/MQ-Det-main.git}\\
% \noindent Models / weights link: \url{https://pan.baidu.com/s/18qNyIaUNHYJlZRxPONuCVQ?pwd=n4yd}\\
% \noindent Reproduction instructions (brief): \texttt{bash extract.sh, bash stage2.sh, bash inference.sh}

% \section{Factsheet Information}

% \subsection{Team details}
% \begin{itemize}
% \item Team name: \texttt{WRC}
% \item Team leader: \texttt{Liwei Zhou}
% \item Affiliation / contact: \texttt{College of Intelligence Science and Technology, National University of Defense Technology,  zhouliwei123@nudt.edu.cn}
% \item Team members: \texttt{Liwei Zhou, Bei Dou, Tao Wu}
% \item Sponsor affiliation (if any): \texttt{None}
% \item Method name / nickname: \texttt{MQ-Det}
% \item Final score (if available): \texttt{139.7438}
% \item Submission link: \url{https://www.codabench.org/profiles/user/zhouliwei21/}
% \end{itemize}

% \subsection{Method overview}
% (Optional) Add a method figure if you have one.
% \begin{figure}[!htbp]
% \centering
% \IfFileExists{teams2026/team13_WRC/images/method_figure.png}{  
%   \includegraphics[width=0.95\linewidth]{images/method_figure.png}  
% }{
%   \fbox{\parbox[c][0.8\textheight][c]{0.95\linewidth}{
%   \centering \textbf{Method Figure Placeholder}\\
%   Put \texttt{method\_figure.png} (or .png/.jpg) in the \texttt{images/} folder and update filename.  
%   }}
% }
% \caption{Overall pipeline of Multimodal Query-based Object Detection.}

% \label{fig:method}
% \end{figure}
\begin{figure}[!htbp]
\centering
% 定义统一的图片路径变量，解决路径不一致问题
\def\figPath{teams2026/team13_WRC/images/method_figure.png}
\IfFileExists{\figPath}{
  % 加载路径与检查路径完全一致，保留原宽度设置
  \includegraphics[width=0.95\linewidth]{\figPath}
}{
  % 优化占位提示，明确图片应放置的正确路径，保留原高度比例
  \fbox{\parbox[c][0.8\textheight][c]{0.95\linewidth}{
  \centering \textbf{Method Figure Placeholder}\\
  Put \texttt{method\_figure.png} (or .png/.jpg) in \texttt{teams2026/team13_WRC/images/} folder and check filename.
  }}
}
\caption{Overall pipeline of Multimodal Query-based Object Detection.}
\label{fig:method13}
\end{figure}

\noindent \textbf{High-level idea:}Based on an image-text multimodal detector\cite{groundingdino2024}, this method first constructs a full-level multi-scale visual query library, and performs instantiation and cascaded refinement guided by text semantics on the retrieved visual features. It then embeds the refined visual queries into the deep layers of the frozen text encoder via a gated adaptive fusion mechanism, achieving efficient cross-modal alignment of visual and textual features. Subsequent joint image-text fine-tuning is carried out: the visual backbone network and the shallow layers of the text encoder are frozen to preserve the basic representation capability; learnable continuous prompt parameters are introduced into the text branch, and LoRA low-rank adaptation is added to the cross-attention layer for visual-text fusion. To address the partially unlabeled instances existing in the few-shot dataset, the EMA (Exponential Moving Average) Mean Teacher\cite{meanteacher2017} is incorporated to generate pseudo-labels, thereby enhancing the effect of model fine-tuning. Only the parameters of the fusion module are fine-tuned to improve the performance of few-shot object detection.\\
\noindent \textbf{Key contributions:}
\begin{itemize}
    \item \textbf{Contribution 1:} A vision-enhanced text branch is constructed, which bridges the modal gap of pure text in characterizing fine-grained visual features and enables efficient cross-modal alignment of visual-text features via the establishment of a visual query library, cascaded refinement of retrieved features and gated adaptive fusion.
    \item \textbf{Contribution 2:} A lightweight joint image-text fine-tuning strategy is designed: the visual backbone and shallow layers of the text encoder are frozen, learnable prompt parameters are introduced into the text branch, LoRA adaptation is applied to the cross-attention layer for visual-text fusion, and only the fusion module is fine-tuned to boost few-shot detection performance and mitigate overfitting.
\end{itemize}

\noindent \textbf{Model architecture}
Describe the backbone, detector head, any added modules, and where they are inserted.
\begin{itemize}
    \item Backbone: \texttt{(Swin-T, BERT-base-uncased)}
    \item Detector: \texttt{(Deformable DETR)}
    \item Additional components: \texttt{(Vision Query Bank, Gated Cross-Attention, CoOp, LoRA)}
\end{itemize}

\subsubsection{Training details}
Provide training settings sufficient for reproduction.
\begin{itemize}
    \item Training data: \texttt{(coco17)}
    \item Few-shot setting: \texttt{(1/5/10-shot,challenge-provided fixed support sets)}
    \item Optimization: \texttt{(AdamW, 1e-4, WarmupMultiStepLR, 1, 20)}
    \item Augmentations: \texttt{(Multi-scale Resize, Random Horizontal Flip, Normalization)}
    \item Hardware / runtime: \texttt{(A100, 1 GPU, 3 hours)}
\end{itemize}

\noindent \textbf{Inference details}
Explain inference-time details that affect performance.
\begin{itemize}
    \item Test-time settings: \texttt{(Scale: Short edge 800, Long edge max 1333, score threshold: 0.05, Max Detections: 900 )}
    \item Ensemble / TTA: \texttt{(None)}
    \item Any post-processing: \texttt{(None)}
\end{itemize}

% \subsection{Experimental results}
% Fill in your results. Replace dataset names with official ones used in the challenge.

% \begin{table}[t]\scriptsize
% \centering
% \begin{tabular}{clcccc}
% \toprule
% & \textbf{Method} & \textbf{Setting} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{1-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{12.8} & \texttt{8.0} & \texttt{15.8} \\
% & Ours (\texttt{MQ-Det}) & \texttt{(Close)} & \texttt{15.6} & \texttt{53.2} & \texttt{21.9} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{5-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{22.7} & \texttt{19.8} & \texttt{29.1} \\
% & Ours (\texttt{MQ-Det}) & \texttt{(Close)} & \texttt{31.4} & \texttt{54.7} & \texttt{33.3} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{10-shot}}
% & Baseline / Reference & \texttt{(Close)} & \texttt{21.8} & \texttt{16.9} & \texttt{32.6} \\
% & Ours (\texttt{MQ-Det}) & \texttt{(Close)} & \texttt{27.6} & \texttt{54.2} & \texttt{36.4} \\
% \bottomrule
% \end{tabular}
% \caption{Results under 1/5/10-shot settings on three target datasets. Replace placeholders with official numbers.}
% \label{tab:results}
% \end{table}

% \noindent \textbf{Ablation and analysis (optional)}
% \begin{itemize}
%     \item Failure cases: \texttt{Without the pseudo-label generation module, due to a large number of unannotated instances in Dataset 2, the 5-shot and 10-shot scores of Dataset 2 drop to 17.9 and 18.1, respectively. The performance of Dataset 1 also decreases, resulting in a total score of only 109. However, the pseudo-label generation method currently used is overly simplistic and still introduces some incorrect labels.}
% \end{itemize}

% \section{Other details}
% \begin{itemize}
% \item Planned submission of a solution description paper at NTIRE 2026 workshop: \texttt{No}.
% \item General comments and impressions of the NTIRE 2026 challenge: \texttt{NTIRE 2026 is a highly valuable challenge in computer vision. It provides dedicated datasets, reliable baseline models, and standardized evaluation protocols for cross-domain few-shot object detection, offering a clear research direction and a fair comparison platform. It effectively guides participants to continuously improve their methods and promotes the advancement of related technologies}.
% \item Suggestions for future CD-FSOD challenges (e.g., new subtracks, new metrics): \texttt{The evaluation is limited by using only mAP, as practical detection tasks do not demand high IoU and only require approximate box placement. Thus, the scoring should focus more on detection correctness instead of high-IoU-based mAP}.
% \item Other comments: encountered difficulties, fairness, proposed evaluation methods, etc.: \texttt{The datasets are stored on Google Drive for download, which frequently causes access limitations for users in China}.
% \end{itemize}

% %%%%%%%%% REFERENCES (self-contained, compilable placeholder)
% {\small
% \begin{thebibliography}{1}

% \bibitem{fu2025cross}
% Fu, Y., Qiu, et al.
% \newblock NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results.
% \newblock 2025 IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (CVPRW), 2025.

% \bibitem{groundingdino2024}
% Liu, Shilong, Zeng, Xingyi, et al.
% \newblock Grounding DINO: Marrying DINO with Grounded Pre-training for Open-Set Object Detection.
% \newblock \textit{18th European Conference on Computer Vision (ECCV 2024)}, 2025.

% \bibitem{meanteacher2017}
% Tarvainen, Antti, Valpola, Harri, et al.
% \newblock Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results.
% \newblock \textit{NIPS'17: Proceedings of the 31st International Conference on Neural Information Processing Systems}, 2017.
% \end{thebibliography}
% }

% % If you have a .bib file, comment thebibliography above and use:
% % {\small
% % \bibliographystyle{ieee_fullname}
% % \bibliography{egbib}
% % }

% \end{document}


==> teams/team9_FDUROILab_Lenovo/sec/1_intro.tex <==
\section{Introduction}

Cross-domain few-shot object detection (CDFSOD)~\cite{fu2025cross,fu2025ntire} is a challenging task that aims to detect specified object categories in a new target domain using only a few labeled examples (e.g., 1-shot, 5-shot, or 10-shot), which differ significantly from the source training set. Unlike traditional object detection, CDFSOD requires models to identify and classify objects beyond the training set while handling severe domain shifts effectively. Compared to standard open-vocabulary detection, CDFSOD presents an additional challenge due to the substantial distribution discrepancies between the novel target domain and the original source domain, which often leads to severe performance degradation.

To address these challenges, we propose an efficient fine-tuning and adaptation approach built upon the robust open-vocabulary detection model. By applying strategic transformations to the highly limited support samples for data augmentation, we significantly enhance the adaptation capability of the detection model to the unseen target domains. Furthermore, we introduce a novel post-processing method leveraging multimodal large language models (MLLMs) to refine the predictions and achieve more precise classification, effectively bridging the domain gap. Our approach aims to maximize the Mean Average Precision (mAP) in cross-domain scenarios with minimal supervision, ensuring superior adaptability and robust detection performance on the unseen test sets.

==> teams/team9_FDUROILab_Lenovo/sec/2_method.tex <==
\section{Team Details}
\begin{itemize}
\item Team name: FDUROILab\_Lenovo                    
\item Team leader name: Lingyi Hong                   
\item Team leader email: lyhong22@m.fudan.edu.cn
\item Team members: Mingxi Cheng, Xingqi He, Runze Li, Xingdong Sheng, Wenqiang Zhang
\item Affiliation: Fudan University, Lenovo Research
\item Best scoring entries of the team during the test phase: 217.2
\item Code, pre-trained model, and factsheet download command/link: \href{https://github.com/omnipotent13/FDUROILab\_Lenovo\_2026\_CDFSOD\_Challenge}{github}
\end{itemize}

\section{Code Submission}
\noindent Code link / repository: \href{https://github.com/omnipotent13/FDUROILab\_Lenovo\_2026\_CDFSOD\_Challenge}{github}\\
\noindent Models / weights link: \href{https://huggingface.co/MaggotKing/2026_CDFSOD_FDUROILab_Lenovo}{MaggotKing/2026\_CDFSOD\_FDUROILab\_Lenovo}\\
\noindent Reproduction instructions (brief): You can easily follow the provided README to reproduce our results.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figure1.pdf} 
    \caption{Overview of our efficient tuning and inference.}
    \label{fig:tuning}
\end{figure*}

\section{Method}

In this section, we firstly introduce our approach to enhancing cross-domain few-shot object detection (CD-FSOD) through efficient fine-tuning based on the vision-language open-vocabulary framework. Then, we describe a robust post-processing strategy utilizing a Multimodal Large Language Model (MLLM). 

\subsection{Efficient Tuning}

To significantly enhance the model’s adaptability in complex cross-domain scenarios, we propose an efficient fine-tuning strategy tailored for the open-vocabulary detection model. Our approach leverages diverse data augmentation techniques to expand the limited training set and improve the model’s ability to recognize novel objects in the target domain using the provided k-shot annotated samples.

Given a k-shot setting, where k represents the number of provided object samples, we employ a structured fine-tuning pipeline, which is shown in Figure~\ref{fig:tuning}. (1) \textbf{Object Cropping and Augmentation.} Using the provided bounding boxes of k-shot examples, we first crop the target objects from the original images. The cropped objects are then subjected to various data augmentation techniques, including flipping, rotation, grayscale conversion, and other transformations, to introduce diversity and improve generalization. (2) \textbf{Object Rescaling and Random Pasting.} We randomly rescale the augmented objects to different sizes and paste these transformed objects onto the original images at different locations. This step simulates new object placements and enhances the model’s robustness to variations in object appearance and context. (3) \textbf{Fine-Tuning with Augmented Data.} We finetune the open-vocabulary detection model with the augmented images. This enables the vision components of the detector to better adapt to objects in the target domain, even with minimal labeled examples. Additionally, the augmented data effectively increases the number of training samples, mitigating the few-shot learning limitation and improving overall detection performance.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figure2.pdf} 
    \caption{Post Processing.}
    \label{fig:post}
\end{figure*}

\begin{table*}[h] 
    \centering 
    
    \caption{Results from Leaderboard}
    \label{tab:leaderboard}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccc} 
        \toprule 
        User & final\_score & D1\_1shot & D1\_5shot & D1\_10shot & D2\_1shot & D2\_5shot & D2\_10shot & D3\_1shot & D3\_5shot & D3\_10shot \\
        \midrule 
        \rowcolor{gray!20}
        FDUROILab\_Lenovo (ours) & 217.22 & 	57.04 &	57.15 &	58.08 &	59.23 &	59.23 &	59.23 &	45.23 &	46.17 &	48.77 \\

        zouyyds & 192.79 & 34.61 & 41.14 & 42.05 & 63.25 & 63.00 & 61.29 & 39.71 & 47.43	& 48.29 \\
        NJUST-KMG & 191.37 & 35.62 & 47.52 & 46.22 & 60.41 & 60.51 & 61.11 & 40.08 & 42.01 & 44.54 \\
        
        \bottomrule 
    \end{tabular}
    }
\end{table*}

\subsection{Inference}

Since our approach utilizes the open-vocabulary detection model, which fundamentally relies on vision-language alignment, it requires access to accurate target category labels during inference, as shown in Figure~\ref{fig:tuning}. To obtain these context-rich labels, we utilize Qwen3-VL~\cite{bai2025qwen3} to generate descriptive textual representations of the target categories. The retrieved target labels from Qwen3-VL are then used as textual input to guide the detection process. Finally, we adopt the detection model to identify and classify objects in the test images based on these enhanced text-based prompts.

\subsection{Post-Process}

Although modern vision-language detectors possess strong generalization capabilities, their performance on the challenging cross-domain test set remains suboptimal in certain cases. Upon further analysis, we found that while the detector can successfully localize most objects, its primary weakness lies in classification errors rather than detection failures. This indicates that the detector still struggles with fine-grained classification when adapting to objects in a new domain. To address this issue, we introduce Qwen3-VL as an auxiliary classifier to refine the final predictions, which is illustrated in Figure~\ref{fig:post}.

Specifically, for each test image, we construct a multimodal prompt comprising the target scene and a set of representative example images for all candidate categories. By leveraging these example images as visual prompts, we instruct Qwen3-VL to describe the objects present in the scene and output a refined list of categories that are likely to appear. After that, we refine the output of the detection model using one of two strategies: (1) \textbf{Filtering.} Remove objects that are classified incorrectly by the detector and are not listed by Qwen3-VL. (2) \textbf{Reclassification.} Assign all detected objects to one of the categories predicted by Qwen3-VL, ensuring consistency between the detected bounding boxes and the high-level scene understanding of the multimodal model. The choice between these two strategies depends on the specific test dataset, as detailed in the Implementation Details. By leveraging Qwen3-VL and visual prompting as a post-processing step, we effectively correct classification errors and enhance the model’s performance on unseen domains, leading to more accurate and reliable object detection results.

\subsection{Remark}

Our method strictly adheres to the k-shot setting, using only the provided k-shot labeled samples for fine-tuning. We do not incorporate any external detection datasets, additional bounding box annotations, or test set images during training. All improvements to the model are achieved solely through the given few-shot examples and permitted pretrained resources, ensuring full compliance with the competition’s constraints.

\subsection{Implementation Details}

We use the open-vocabulary detection model as our baseline detection model. We utilize Qwen3-VL-235B-A22B~\cite{bai2025qwen3} as our MLLM for label generation and post-processing. Our fine-tuning experiments are conducted on 8 NVIDIA RTX 3090 GPUs, with a batch size of 8 and a base learning rate of 1e-6. During the optimization process, the \texttt{text\_model} is completely frozen, and an \texttt{lr\_mult} of 0.01 is applied to it. We experiment with different numbers of training iterations across datasets and few-shot settings. For dataset1 and dataset3, we fine-tune the model for 30, 50, and 100 batches under 1-shot, 5-shot, and 10-shot settings. For dataset2, we do not perform any fine-tuning. 

To maximize classification accuracy, we adopt dataset-specific post-processing strategies. For dataset1, we reclassify all detected objects into one of the categories predicted by Qwen3-VL. For dataset3, we filter out any detected objects that do not belong to the MLLM-predicted categories. For dataset2, since it contains only a single object category, we do not perform additional classification. However, we apply a specific filtering step: we eliminate overly large detection boxes, which are likely incorrect, as objects in dataset2 are generally small. Besides, we also apply Non-Maximum Suppression (NMS) to suppress redundant or overlapping bounding boxes across all datasets. These dataset-specific strategies ensure that our model achieves optimal performance across different domain shifts and few-shot settings.

\section{Results}

We show the results from the official Challenge Leaderboard in Table~\ref{tab:leaderboard}.

\section{Conclusion}

In this paper, we tackle cross-domain few-shot object detection (CD-FSOD) by proposing an efficient fine-tuning strategy based on the open-vocabulary detection framework, coupled with a Qwen3-VL-assisted post-processing method. Our approach enhances the model's adaptability to new domains through strategic data augmentation, object transformation, and parameter-efficient tuning, while MLLM-based post-processing significantly improves classification accuracy. Experimental results demonstrate the effectiveness and robustness of our method in few-shot settings.









 


